iBall: Augmenting Basketball Videos with Gaze-moderated Embedded Visualizations

We present iBall, a basketball video-watching system that leverages gaze-moderated embedded visualizations to facilitate game understanding and engagement of casual fans. Video broadcasting and online video platforms make watching basketball games increasingly accessible. Yet, for new or casual fans, watching basketball videos is often confusing due to their limited basketball knowledge and the lack of accessible, on-demand information to resolve their confusion. To assist casual fans in watching basketball videos, we compared the game-watching behaviors of casual and die-hard fans in a formative study and developed iBall based on the fndings. iBall embeds visualizations into basketball videos using a computer vision pipeline, and automatically adapts the visualizations based on the game context and users' gaze, helping casual fans appreciate basketball games without being overwhelmed. We confrmed the usefulness, usability, and engagement of iBall in a study with 16 casual fans, and further collected feedback from 8 die-hard fans.

==> tex/_deprecated/1-intro_v0.tex <==
\section{Introduction}

% - basketball is good
TV broadcasting and live streams 
have significantly expanded access to live sports games 
and continued to attract new fans to watch sports games
over the past decades.
For example,
basketball, one of the most popular team sports,
has attracted more than 2 billions fans worldwide~\cite{}.
In the last year, 
the average viewers per NBA game across ABC~\footnote{}, ESPN~\footnote{}, 
and TNT~\footnote{} has increased by 19\% compared to the 2020-21 season~\cite{}.

% the NBA league averaged 1.6 million viewers per game across 
% up 19\% from the 2020-21 season~\cite{}. 
% Additionally, 
% with the proliferation of social media platforms such as Twitter and TikTok,
% NBA videos viewership has seen a growth in the last year
% with 910 millions new views compared to the 2020-21 season~\cite{}.
% Generally speaking, sports videos and live streams have gradually become the mainstream medium to watch sports
% and, due to their accessibility, continue to attract new fans to watch sports games.

% - basketball is hard to understand, high entry barrier, unfriendly for casual fans
However, team sports, such as basketball, usually involve complex rules, norms, tactics, and in-game decisions that can be hard to understand for new fans.
For example, in basketball games, the five players on the offense need to play collaboratively and make numerous in-game decisions within a few seconds to make a field goal.
These in-game decisions are made based on a large amount of situated information,
such as the players' positions, their abilities, the score, and the game clock.
While experienced fans usually can read this information from the game videos, new and casual fans lack sufficient knowledge to interpret such information.
Consequently, without knowing these details,
casual fans can easily get confused and overwhelmed when watching basketball games and cannot appreciate games at the same deep level of understanding as experienced fans.

%% need more in-game data and explanations to help them understand what's going on
Unfortunately, the mainstream TV broadcasting and live streams
fall short in providing sufficient information for casual fans to understand basketball games.
After decades of development, 
scoreboards and commentaries remain the major methods for casual fans to obtain data when watching live games on TV.
%% not controllable
The data provided by these methods lack not only controllability but also diversity,
which can hardly fulfill the individual needs of the casual fans~\cite{}.
%% data is separated
On the other hand,
thanks to the advances in sensing and computer vision (CV) techniques,
live data such as game events and player positions
are becoming increasingly available in each NBA game.
These data, together with other historical stats of the players, can significantly facilitate the casual fans' understanding and engagement of NBA games.
Currently, however, these extra data are stored and presented in webpages (e.g., ESPN~\cite{}), % separated from the game videos,
distracting the fans from the game videos to separated windows.
% forcing the fans to look up the data in separated windows and 
Thus, finding a way to enable seamless access to extra data when watching live games could greatly benefit casual fans in their understanding of and engagement with games.

Embedded visualizations provide a promising opportunity to improve casual fans' game watching experience.
By directly displaying data in the actual physical scene, 
embedded visualizations allow audiences 
to consume situated data within its physical context.
Audiences can thus access extra data 
without getting distracted from the game videos.
Given such benefits,
various commercial products (e.g., Viz Libero~\cite{} and Piero~\cite{}) 
and research systems (e.g., VisCommentator~\cite{} and Sporthesia~\cite{})
leverage embedded visualizations and video effects (e.g., pause and slow motion) 
to augment sports videos.
However, all these systems focus on post-game analysis
and cannot be used for live game watching scenarios,
where the visualizations must be lightweight and videos cannot be paused.
An exception is CourtVision~\cite{}, a live basketball game watching system 
that allows users to inspect in-game stats of each player through embedded visualizations.
However, it only uses simple, non-interactive text labels and progress bars to show the data.
Recently, researchers have started to explore the design space of embedded visualizations in live game watching scenarios~\cite{}.
However, the researchers mainly investigated visualizations in abstracted scenarios (e.g., 3D simulated sports games~\cite{},  moving charts on white background~\cite{}).
Little is known about how embedded visualizations can facilitate watching experiences
in real live sports videos.

In this work, we aim to develop a personalized basketball viewing system to improve casual fans' game watching experiences.
To understand the current practices, pain points, and requirements of casual fans in watching live basketball games,
we conducted a formative study with 16 participants (8 casual and 8 die-hard fans).
We involved the die-hard fans as a reference 
to be able to identify the pain points that are particular to casual fans and to further inform the design of our system.
We adopted a contextual query~\cite{hartson2012ux},
to observe fans watching basketball games in a live setting 
and record their think-aloud and gaze data.
Findings reveal that casual fans are confused about \cmo{xxx}.

Based on our findings, we developed \system{}, a basketball game viewing system that features gaze-moderated embedded visualizations.
\system{} uses embedded visualizations to \cmo{a) direct users attention to the key players, b) present situated data for understanding in-game decisions, and c) adaptively adjust visualizations based on the user's gaze.}


% In this study, we aim to fill this gap by exploring the design space of embedded visualizations for live sports in-game data analysis. 
% We adopted a user-centered design approach throughout the study to answer three questions: 



% with embedded visualizations 
% We propose to leverage leverage live gaze as implicit feedback from the audiences to personalized the embedded visualizations.


==> tex/_deprecated/1-intro_v1.tex <==
\section{Introduction}

% - basketball is good
TV broadcasting and live streams 
have significantly expanded access to live sports games 
and continued to attract new sports fan %s to watch sports games
over the past decades.
For example,
in basketball, one of the most popular team sports,
the average viewers per NBA game across ABC~\cite{}, ESPN~\cite{}, and TNT~\cite{} has
increased to 1.6 million in the last year, 
up 19\% from the 2020-21 season~\cite{}.
These new fans usually lack sufficient knowledge to fully understand basketball games that involve complex teamwork and in-game decisions.
These in-game decisions are made based on rules, norms, tactics, 
and a large amount of situated information,
such as the players' positions, their abilities, the score, and the game clock.
While experienced fans can read this information from the game videos, 
new and casual fans lack enough knowledge to interpret such information.
Consequently, without knowing these details,
casual fans can easily get confused when watching basketball games 
and thus cannot appreciate games at the same deep level of understanding and engagement as experienced fans.


%% need more in-game data and explanations to help them understand what's going on
However, the mainstream TV broadcasting and live streams
fall short in providing sufficient information for new and casual fans to understand basketball games.
After decades of development, 
TV broadcasting and live streams are still using 
scoreboards and commentaries as the primary methods to provide data for the audiences.
A recent study revealed that the data provided by these methods lack controllability and diversity
and can hardly fulfill the individual needs of the fans~\cite{}.
%% data is separated
On the other hand,
thanks to the advances in sensing and computer vision (CV) techniques,
live data such as game events and player positions
are becoming increasingly available in each NBA game.
These data, together with other historical stats of the players, 
can significantly facilitate the casual fans' understanding and engagement of the games.
However, these extra data are stored and presented in webpages (e.g., ESPN~\cite{}), % separated from the game videos,
distracting the fans from the game videos to separated windows. 
\cmo{another issue is that they don't know what to look up}
Thus, 
finding a way to enable seamless access to extra data 
when watching live games can greatly benefit casual fans 
in their understanding and engagement of basketball games.

%%%%%%%%%%%%%%%% research questions %%%%%%%%%%%%%%%%
Embedded visualizations provide a promising opportunity to improve casual fans' game watching experience.
By directly displaying data in the actual physical scene, 
embedded visualizations allow audiences 
to consume situated data within its physical context.
Audiences can thus access extra data 
without getting distracted from the game videos.
Given such benefits,
various commercial products (e.g., Viz Libero~\cite{} and Piero~\cite{}) 
and research systems (e.g., VisCommentator~\cite{} and Sporthesia~\cite{})
leverage embedded visualizations and video effects (e.g., pause and slow motion) 
to augment sports videos.
However, all these systems focus on post-game analysis
and cannot be used for live game watching scenarios,
where the visualizations must be lightweight and videos cannot be paused.
An exception is CourtVision~\cite{},
a live basketball game watching system developed by Second Spectrum~\cite{}
that allows users to inspect in-game stats of players through embedded visualizations.
However, it only uses simple, non-interactive text labels and progress bars to show the data.
Recently, 
researchers have started to explore the design space of embedded visualizations for live games
but mainly using abstracted settings 
(e.g., 3D simulated sports games~\cite{}, moving charts on white background~\cite{}).
Little is known about 
the designs and key techniques to enable interactive embedded visualizations in live sports videos
and how they can facilitate game understanding and engagement.

In this work, 
we aim to fill this gap by 
investigating 
the design and implementation of interactive embedded visualizations in live basketball videos
to improve casual fans' watching experiences.
To understand the practices, pain points, and requirements of casual fans in watching live basketball games,
we conducted a formative study with 16 participants (8 casual and 8 die-hard fans).
We involved the die-hard fans as a reference 
to identify the pain points that are particular to casual fans.
% and to further inform the design of our system.
% We adopted a contextual query~\cite{hartson2012ux},
% to observe fans watching basketball games in a live setting 
% and record their think-aloud and gaze data.
% Findings reveal that casual fans are confused about \cmo{xxx}.
Informed by the findings (detail in Sec.3), 
we develop \system{}, 
a basketball game viewing system that features gaze-moderated embedded visualizations,
by tackling two main challenges:
First, embedding visualizations into actual scenes is recognized as a grand challenge for situated visualizations~\cite{}, 
especially for basketball as the players overlaps heavily
and the camera moves rapidly.
However, to the best of our knowledge,
there is no publicly available solutions to achieve embedded visualizations for basketball videos.
We contribute an open-sourced CV pipeline to process the video for 
embedding visualizations into basketball videos,
which provides a stepstone for future research in embedded visualizations in complex, dynamic scenarios.
Second, how to design embedded visualizations that 
seamlessly present extra data in basketball games 
without distracting and overwhelming audiences remains an open question.
Different audiences can have individual game and data literacy

Visual design to direct users attention and present situated data for understanding in-game decisions without overwhelming.
Third, gaze-interactions
to adaptively adjust visualizations based on the user's own interests.


==> tex/_deprecated/1-intro_v3.tex <==
\section{Introduction}
% - basketball is good
TV broadcasting and live streams 
have significantly expanded access to live sports games 
and continued to attract new sports fan %s to watch sports games
over the past decades.
For example,
in basketball, one of the most popular team sports,
the average viewers per NBA game across ABC~\cite{ABC}, ESPN~\cite{ESPN}, and TNT~\cite{TNT} has
increased to 1.6 million in the last year, 
up 19\% from the 2020-21 season~\cite{NBAUp}.
These new fans usually cannot
fully understand basketball games that involve complex teamwork and in-game decisions.
These in-game decisions are made based on rules, norms, tactics, 
and large amounts of situated information,
such as the players' positions and abilities, the score, and the game clock.
Unlike experienced fans,
% While experienced fans can read this information from the game videos, 
new and casual fans often lack sufficient knowledge to read this information from the game videos.
As our formative study will show,
without knowing these details,
casual fans can easily get confused when watching basketball games 
and cannot appreciate games at the same deep level of understanding and engagement as experienced fans.

%% need more in-game data and explanations to help them understand what's going on
However, mainstream TV broadcasting and live streams
fall short in providing enough information for new and casual fans to understand basketball games.
After decades of development, 
TV and live streams are still using 
scoreboards and commentaries as the primary methods to provide data for the audiences.
A recent study revealed that the data provided by these methods lack controllability and diversity
and can hardly fulfill the individual needs of the fans~\cite{}.

%% data is separated
On the other hand,
thanks to the advances in sensing and computer vision (CV) techniques,
live data such as game events and player positions
are becoming increasingly available in each NBA game.
These data, together with other historical stats of the players, 
can significantly facilitate the casual fans' understanding and engagement of the games.
However, these extra data are stored and presented in webpages (e.g., ESPN~\cite{}), % separated from the game videos,
distracting the fans from the game videos to separated windows. 
Thus, 
finding a way to enable seamless access to extra data 
when watching live games can greatly benefit casual fans 
in their understanding and engagement of basketball games.

%%%%%%%%%%%%%%% In this work, we aim to fill this gap by %%%%%%%%%

%%%%%%%%%%%%%%%% research questions %%%%%%%%%%%%%%%%
Embedded visualizations provide a promising opportunity to improve casual fans' game watching experience.
By directly displaying data in the actual physical scene, 
embedded visualizations allow audiences 
to consume situated data within its physical context.
Audiences can thus access extra data 
without getting distracted from the game videos.
Given such benefits,
various commercial products (e.g., Viz Libero~\cite{} and Piero~\cite{}) 
and research systems (e.g., VisCommentator~\cite{} and Sporthesia~\cite{})
leverage embedded visualizations and video effects (e.g., pause and slow motion) 
to augment sports videos.
However, all these systems focus on post-game analysis
and cannot be used for live game watching scenarios,
where the visualizations must be lightweight and videos cannot be paused.
An exception is CourtVision~\cite{},
a live basketball game watching system developed by Second Spectrum~\cite{}
that allows users to inspect in-game stats of players through embedded visualizations.
However, it only uses simple, non-interactive text labels and progress bars to show the data.
Recently, 
researchers have started to explore the design space of embedded visualizations for live games
but mainly using abstracted settings 
(e.g., 3D simulated sports games~\cite{}, moving charts on white background~\cite{}).
Little is known about 
the designs and key techniques to enable interactive embedded visualizations in live sports videos
and how they can facilitate game understanding and engagement.

In this work, 
we aim to fill this gap by 
investigating 
the design and implementation of interactive embedded visualizations in live basketball videos
to improve casual fans' watching experiences.
To understand the practices, pain points, and requirements of casual fans in watching live basketball games,
we conducted a formative study with 16 participants (8 casual and 8 die-hard fans).
We involved the die-hard fans as a reference 
to identify the pain points that are particular to casual fans.
Findings revealed that XXX.
Yet, 

% We found that the
% animations and transitions of unit visualizations in such content tightly correspond with the content and structure of
% the underlying story, which conforms with previous literature on principles of effective visual communication with
% animations. Yet, ensuring such congruence requires tedious back and forth between the visual and the narrative during
% the prototyping, editing, composition, and iteration of the content.


Informed by the findings, 
we develop \system{}, 
a basketball game viewing system that features gaze-moderated embedded visualizations
by tackling two main challenges:
First, embedding visualizations into actual scenes is recognized as a grand challenge for situated visualizations~\cite{}, 
especially for basketball as the players overlaps heavily
and the camera moves rapidly.
However, to the best of our knowledge,
there is no publicly available solutions to achieve embedded visualizations for basketball videos.
We contribute an open-sourced CV pipeline to process the video for 
embedding visualizations into basketball videos,
providing a stepstone for future research in embedded visualizations in complex, dynamic scenarios.
Second, how to design embedded visualizations in basketball videos that
are informative but not overwhelming for individual (\cmo{or each?}) audiences remains an open question.
% seamlessly present extra data without overwhelming 
The game literacy, data needs, and personal interests 
can vary from audience to audience, 
leading to a great demand of personalized visualizations
in game watching.
We leverage an eye-tracker to track the user's attention
and design a set of gaze-moderate interactive embedded visualizations
that dynamically adapt the visualizations,
as well as the video scene, 
to highlight the user's interested content
and suppress others.
\cmo{where is casual fans? where is educating them to watch the game?}
To evaluate \system{},
we conducted a comparative user study with 16 casual fans.
\cmo{Findings and results.}

In summary,
our contribution is threefold:
1) a CV solution, 2) a set up gaze-moderate embedded visualizations,
3) a user study.

% Users were able to generate distinct game insights with each embedded visualization 
% and to utilize to personalize their in-game analysis in our simulated basketball game videos.

==> tex/_deprecated/1-intro_v4.tex <==
\section{Introduction}
% - basketball is good
TV broadcasting and live streams 
have significantly expanded access to live sports games 
and continued to attract new sports fan %s to watch sports games
over the past decades.
For example,
in basketball, one of the most popular team sports,
the average viewers per NBA game across ABC~\cite{ABC}, ESPN~\cite{ESPN}, and TNT~\cite{TNT} has
increased to 1.6 million in the last year, 
up 19\% from the 2020-21 season~\cite{NBAUp}.
These new fans usually cannot
fully understand basketball games that involve complex teamwork and in-game decisions.
These in-game decisions are made based on rules, norms, tactics, 
and large amounts of situated information,
such as the players' positions and abilities, the score, and the game clock.
Unlike experienced fans,
% While experienced fans can read this information from the game videos, 
new and casual fans often lack sufficient knowledge to read this information from the game videos.
As our formative study will show,
without knowing these details,
casual fans can easily get confused when watching basketball games 
and cannot appreciate games at the same deep level of understanding and engagement as experienced fans.

%% need more in-game data and explanations to help them understand what's going on
However, TV broadcasting and live streams
fall short in providing enough information for new and casual fans to understand basketball games.
After decades of development, 
TV and live streams are still using 
scoreboards and commentaries as the primary methods to provide data for the audiences.
A recent study revealed that the data provided by these methods lack controllability and diversity
and can hardly fulfill the individual needs of the fans~\cite{}.
%% data is separated
On the other hand,
thanks to the advances in sensing and computer vision (CV) techniques,
live data such as game events and player positions
are becoming increasingly available in each NBA game.
These data, together with other historical stats of the players, 
can significantly facilitate the casual fans' understanding and engagement of the games.
Yet, these extra data are stored and presented in webpages (e.g., ESPN~\cite{}), % separated from the game videos,
distracting the fans from the game videos to separated windows. 
Thus, 
finding a way to enable seamless access to extra data 
when watching live games can greatly benefit casual fans 
in their understanding and engagement of basketball games.

%%%%%%%%%%%%%%%% research motivations %%%%%%%%%%%%%%%%
In this work, 
we aim to fill 


Embedded visualizations provide a promising opportunity to fulfill casual fans' in-game data needs.
By directly displaying data in the actual scenes, 
embedded visualizations allow audiences 
to consume situated data within its physical context without being distracted from the game videos.
% Audiences can thus access extra data 
% without getting distracted from the game videos.
Given such benefits,
various commercial products~\cite{vizrt, piero}
% (e.g., Viz Libero~\cite{} and Piero~\cite{}) 
and research systems~\cite{VisCommentator, chen2022sporthesia}
% (e.g., VisCommentator~\cite{} and Sporthesia~\cite{})
leverage embedded visualizations 
to augment sports videos.
However, all these systems focus on post-game analysis
and cannot be used for live game watching scenarios,
where the visualizations must be lightweight and videos cannot be paused.
An exception is CourtVision~\cite{courtvision} developed by Second Spectrum~\cite{secondspectrum},
which targets live game watching scenarios 
but only uses simple, non-interactive text labels and progress bars to show data.
Recently, 
researchers have started to explore the design space of embedded visualizations for live games
but mainly using abstracted settings 
(e.g., 3D simulated sports games~\cite{}, moving charts on white background~\cite{}).
Little is known about 
the key techniques and visual and interaction designs
to enable interactive embedded visualizations in live sports videos
and how they can facilitate game understanding and engagement.

%%%%%%%%%%%%%%% In this work, we aim to fill this gap by %%%%%%%%%
In this work, 
we aim to fill this gap by 
investigating 
the design and implementation of interactive embedded visualizations in live basketball videos
to improve casual fans' watching experiences.
To understand the practices, pain points, and requirements of casual fans in watching live basketball games,
we conducted a formative study with 16 participants (8 casual and 8 die-hard fans).
We involved the die-hard fans as a reference 
to identify the pain points that are particular to casual fans.
Findings revealed that casual fans 
Yet, 

% We found that the
% animations and transitions of unit visualizations in such content tightly correspond with the content and structure of
% the underlying story, which conforms with previous literature on principles of effective visual communication with
% animations. Yet, ensuring such congruence requires tedious back and forth between the visual and the narrative during
% the prototyping, editing, composition, and iteration of the content.


Informed by the findings, 
we develop \system{}, 
a basketball game viewing system that features gaze-moderated embedded visualizations
by tackling two main challenges:
First, embedding visualizations into actual scenes is recognized as a grand challenge for situated visualizations~\cite{}, 
especially for basketball as the players overlaps heavily
and the camera moves rapidly.
However, to the best of our knowledge,
there is no publicly available solutions to achieve embedded visualizations for basketball videos.
We contribute an open-sourced CV pipeline to process the video for 
embedding visualizations into basketball videos,
providing a stepstone for future research in embedded visualizations in complex, dynamic scenarios.
Second, how to design embedded visualizations in basketball videos that
are informative but not overwhelming for individual (\cmo{or each?}) audiences remains an open question.
% seamlessly present extra data without overwhelming 
The game literacy, data needs, and personal interests 
can vary from audience to audience, 
leading to a great demand of personalized visualizations
in game watching.
We leverage an eye-tracker to track the user's attention
and design a set of gaze-moderate interactive embedded visualizations
that dynamically adapt the visualizations,
as well as the video scene, 
to highlight the user's interested content
and suppress others.
\cmo{where is casual fans? where is educating them to watch the game?}
To evaluate \system{},
we conducted a comparative user study with 16 casual fans.
\cmo{Findings and results.}

In summary,
our contribution is threefold:
1) a CV solution, 2) a set up gaze-moderate embedded visualizations,
3) a user study.

% Users were able to generate distinct game insights with each embedded visualization 
% and to utilize to personalize their in-game analysis in our simulated basketball game videos.

==> tex/_deprecated/1-intro_v5.tex <==
\section{Introduction}
% - basketball is good
Basketball, as one of the most popular team sports,
has continually attracted new fans
over the past decades due to the proliferation of TV broadcasting and live streams.
In NBA league alone,
the average viewers per game across ABC~\cite{ABC}, ESPN~\cite{ESPN}, and TNT~\cite{TNT} has
increased to 1.6 million in the last year, 
up 19\% from the 2020-21 season~\cite{NBAUp}.
Unlike experienced fans,
these new and casual fans often lack sufficient knowledge to fully understand basketball games,
which involve complex teamwork and in-game decisions
that are made based on rules, norms, tactics, 
and large amounts of situated information,
such as the players' positions, abilities, and roles.
% As our formative study will show,
Without knowing these details,
casual fans 
can easily get confused when watching basketball games 
and cannot appreciate games at the same deep level of understanding and engagement as experienced fans.


However, mainstream TV broadcasting and live streams
fall short in providing enough information for casual fans to understand basketball games.
After decades of development, 
TV and live streams are still using 
scoreboards and commentaries as the primary methods to provide data for the audiences.
A recent study revealed that the data provided by these methods lack controllability and diversity
and can hardly fulfill the individual needs of the fans~\cite{}.
On the other hand,
thanks to the advances in sensing and computer vision (CV) techniques,
live data such as game events and player positions
are becoming increasingly available in each NBA game.
These data, together with other historical stats of the players, 
can significantly facilitate the casual fans' understanding and engagement of the games.
Yet, these extra data are stored and presented in webpages (e.g., ESPN~\cite{}), % separated from the game videos,
distracting the fans from the game videos to separated windows. 
Thus, 
finding a way to enable seamless access to extra data 
when watching live games can greatly benefit casual fans 
in their understanding and engagement of basketball games.

Embedded visualizations provide a promising opportunity to fulfill casual fans' in-game data needs.
By directly displaying data in the actual scenes, 
embedded visualizations allow audiences 
to consume situated data within its physical context without being distracted from the game videos.
Given such benefits,
various commercial products~\cite{vizrt, courtvision}
and research systems~\cite{VisCommentator, chen2022sporthesia}
leverage embedded visualizations 
to augment sports videos.
However, these systems either focus on post-game analysis, rather than live game watching, scenarios,
or only uses simple, non-interactive text labels and progress bars to show data.
% and cannot be used for live game watching scenarios,
% where the visualizations must be lightweight and videos cannot be paused.
% An exception is CourtVision~\cite{courtvision} developed by Second Spectrum~\cite{secondspectrum},
% which targets live game watching scenarios 
% but only uses simple, non-interactive text labels and progress bars to show data.
Recently, 
researchers have started to explore the design space of embedded visualizations for live games
but mainly using abstracted settings 
(e.g., 3D simulated sports games~\cite{lin2022the}, moving charts on white background~\cite{yao2022visualization}).
Little is known about 
how to design and achieve 
interactive embedded visualizations in live sports videos
and how they can facilitate game understanding and engagement.


The goal of this work is to facilitate casual fans' understanding and engagement 
in watching basketball game videos through interactive embedded visualizations.
To understand the particular practices, pain points, and requirements of casual fans
in watching basketball game videos,
a formative study with 8 casual and 8 die-hard fans was conducted.
% revealed that
% unlike die-hard fans, casual fans are confuse
% about the key players and their in-game decisions from time to time,
% and almost never proactively seek extra information to resolve their confusions in watching basketball videos.
Informed by the study, 
we present \system{}, 
a basketball game viewing system 
that assists casual fans in watching live game videos
by automatically highlighting key players
and visualizing their performance
through gaze-moderated embedded visualizations.
Two main challenges are tackled in developing \system{}:
First, 
embedding visualizations into actual scenes 
is recognized as a grand challenge~\cite{DBLP:conf/chi/EnsBCESWPABDDGH21},
% for situated visualizations~\cite{}, 
especially for basketball wherein the players overlaps heavily
and the camera moves rapidly.
We contribute an open-sourced CV pipeline to process team sports videos for 
embedding visualizations into the videos,
providing a stepstone for future research in embedded visualizations in complex, dynamic scenarios.
Second, 
it remains unclear how to design embedded visualizations that
are informative but not overwhelming for individual audiences,
who may have various game literacy, data needs, and personal interests.
We leverage an eye-tracker to track the user's attention
and design a set of gaze-moderated embedded visualizations
that dynamically adapt the visualizations,
as well as the video scene, 
to highlight the user's interested content
and suppress others.

To evaluate \system{},
we conducted a user study with 16 casual fans
to compare the game watching experiences 
between raw video (\texttt{RAW}), video + embedded visualizations (\texttt{AUG}), 
and video + gaze-moderated embedded visualizations (\texttt{FULL}).
Participants spoken highly of our system,
ranked \texttt{FULL} as the best, 
and confirmed that our embedded visualizations and gaze interactions
are useful, usable, and engaging.
We further discus our observations and design implications obtained from our study for future research inspiration.

In summary,
our contributions include
1) an open-source CV pipeline to process team sports videos for embedding visualizations, 
2) a set of gaze-moderated embedded visualizations for live basketball game videos,
3) a user study that assess our system and provides 
insightful feedback of using embedded visualizations in live team sports videos.


% seamlessly present extra data without overwhelming 
% leading to a great demand of personalized visualizations
% in game watching.
% \cmo{where is casual fans? where is educating them to watch the game?}
% which players they should focus on and 
% To understand the practices, pain points, and requirements of casual fans in watching live basketball games,
% we conducted a formative study with 16 participants (8 casual and 8 die-hard fans).
% We involved the die-hard fans as a reference 
% to identify the pain points that are particular to casual fans.
% Findings revealed that casual fans 
% Yet, 

%%%%%%%%%%%%%%% In this work, we aim to fill this gap by %%%%%%%%%
% In this work, 
% we aim to fill this gap by 
% investigating 
% the design and implementation of interactive embedded visualizations in live basketball videos
% to improve casual fans' watching experiences.
% To understand the practices, pain points, and requirements of casual fans in watching live basketball games,
% we conducted a formative study with 16 participants (8 casual and 8 die-hard fans).
% We involved the die-hard fans as a reference 
% to identify the pain points that are particular to casual fans.
% Findings revealed that casual fans 
% Yet, 

% We found that the
% animations and transitions of unit visualizations in such content tightly correspond with the content and structure of
% the underlying story, which conforms with previous literature on principles of effective visual communication with
% animations. Yet, ensuring such congruence requires tedious back and forth between the visual and the narrative during
% the prototyping, editing, composition, and iteration of the content.
% Users were able to generate distinct game insights with each embedded visualization 
% and to utilize to personalize their in-game analysis in our simulated basketball game videos.

==> tex/_deprecated/1-intro_v6.tex <==
\section{Introduction}
% - basketball is good
Basketball, one of the most popular team sports,
has continually attracted new fans
over the past decades due to the proliferation of TV broadcasting and live streams.
In the NBA league alone,
the average number of viewers per game across major US networks has increased to 
%%ABC~\cite{ABC}, ESPN~\cite{ESPN}, and TNT~\cite{TNT} 
1.6 million in the last year, 
up 19\% from the 2020-21 season~\cite{NBAUp}.
Unlike experienced fans,
these new and casual fans often lack sufficient knowledge to fully understand basketball games,
which involves complex teamwork and in-game decisions
that are made based on rules, norms, tactics, 
and large amounts of situated information,
such as the players' positions, abilities, and roles.
As our formative study will show,
without knowing these details,
casual fans 
can easily get confused when watching basketball games 
and cannot appreciate games at the same deep level of understanding and engagement as experienced fans.

Mainstream TV broadcasting and live streams
fall short in providing enough information for casual fans to understand basketball games.
After decades of development, 
TV and live streams are still using 
scoreboards and commentaries as the primary methods to provide data for their audience.
A recent study revealed that the data provided by these methods lack controllability and diversity
and can hardly fulfill the individual needs of fans~\cite{lin2022the}.
On the other hand,
thanks to the advances in sensing and computer vision (CV) techniques,
live data such as game events and player positions
are becoming increasingly available for NBA games.
These data, together with other historical player stats, 
could significantly facilitate game understanding and engagement in casual fans.
Yet, these extra data are stored and presented on webpages (e.g., ESPN~\cite{}), % separated from the game videos,
distracting fans from the game videos to separated windows. 
Thus, 
finding a way to enable seamless access to extra data 
when watching live games would greatly benefit casual fans 
in their understanding and engagement of basketball games.

Embedded visualizations provide a promising opportunity to fulfill casual fans' in-game data needs.
By directly displaying data in the actual scenes, 
embedded visualizations allow audiences 
to consume situated data within its physical context without being distracted from the game video.
Given such benefits,
various commercial products~\cite{vizrt, courtvision}
and research systems~\cite{VisCommentator, chen2022sporthesia}
leverage embedded visualizations 
to augment sports videos.
However, these systems either focus on post-game analysis rather than live game-watching scenarios,
or only use simple, non-interactive text labels and progress bars to show data.
% and cannot be used for live game watching scenarios,
% where the visualizations must be lightweight and videos cannot be paused.
% An exception is CourtVision~\cite{courtvision} developed by Second Spectrum~\cite{secondspectrum},
% which targets live game watching scenarios 
% but only uses simple, non-interactive text labels and progress bars to show data.
Recently, 
researchers have started to explore the design space of embedded visualizations for live games
but mainly use abstracted settings 
(e.g., 3D simulated sports games~\cite{lin2022the}, moving charts on white background~\cite{yao2022visualization}).
Little is known about 
how to design and implement 
interactive embedded visualizations in live sports videos
and how they can facilitate game understanding and engagement for novice and casual fans.

In this work,
we aim to fill this gap 
by developing interactive embedded visualizations in live basketball videos
to facilitate casual fans' understanding and engagement.
% in watching basketball game videos through interactive embedded visualizations.
To understand the particular practices, pain points, and requirements of casual fans
in watching basketball game videos, we conducted
a formative study with 8 casual and 8 die-hard fans.
% revealed that
% unlike die-hard fans, casual fans are confuse
% about the key players and their in-game decisions from time to time,
% and almost never proactively seek extra information to resolve their confusions in watching basketball videos.
Informed by the study, 
we developed \system{} (\autoref{fig:teaser}), 
a basketball game viewing system 
that assists casual fans in watching live game videos
by automatically highlighting key players
and visualizing their performance
through gaze-moderated embedded visualizations.
We tackle two main challenges to develop \system{}:
First, 
embedding visualizations into actual scenes 
is recognized as a grand challenge~\cite{DBLP:conf/chi/EnsBCESWPABDDGH21},
% for situated visualizations~\cite{}, 
especially for basketball where players overlap heavily
and the camera moves rapidly.
We contribute an open-sourced CV pipeline to process team sports videos for 
embedding visualizations into these videos,
providing a stepping stone for future research in embedded visualizations in complex, dynamic scenarios.
Second, 
it remains unclear how to design embedded visualizations that
are informative but not overwhelming for individual audiences,
who may have various levels of game literacy, data needs, and personal interests.
We leverage an eye-tracker to track the user's attention
and design a set of gaze-moderated embedded visualizations
that dynamically adapt the visualizations,
as well as the video scene, 
to highlight the content the user is interested in,
and to suppress others.

To evaluate \system{},
we conducted a user study with 16 casual fans
to compare the game-watching experiences 
between raw video (\texttt{RAW}), video + embedded visualizations (\texttt{AUG}), 
and video + gaze-moderated embedded visualizations (\texttt{FULL}).
Participants spoke highly of our system,
ranked \texttt{FULL} as the best, 
and confirmed that our embedded visualizations and gaze interactions
are useful, usable, and engaging.
We further discuss our observations and design implications obtained from our study for future research inspiration.

In summary,
our contributions include
1) an open-source CV pipeline to process team sports videos for embedding visualizations, 
2) a set of gaze-moderated embedded visualizations for live basketball game videos,
3) a user study that assesses our system and provides 
insightful feedback on using embedded visualizations in live team sports videos.

==> tex/_deprecated/1-intro_v7.tex <==
\section{Introduction}
% - basketball is good
Basketball, one of the most popular team sports,
has continually attracted new fans
over the past decades due to the proliferation of \cmo{video broadcasting and online video platforms}.
In the NBA league alone,
the average number of viewers per game across major US networks has increased to 
1.6 million in the last year, 
up 19\% from the 2020-21 season~\cite{NBAUp}.
Today, watching basketball games is not just a personal hobby
but a social activity that connects people, 
increases solidarity, 
and boosts social capital. 
% Additionally, it even endorses diversity, inclusion, unity, and teamwork~\cite{}.

However, as our formative study will show,
new or casual fans often get confused
when watching basketball videos,
and cannot appreciate games at the same deep level of understanding and engagement as experienced fans.
Basketball games often involve complex teamwork and in-game decisions
that are made based on rules, tactics, 
and large amounts of situated information,
such as the players' positions, abilities, and roles.
Unlike experienced fans, 
casual fans lack sufficient basketball knowledge 
to extract and interpret this information from game videos.
Yet, existing methods 
fall short of supporting fans to access extra information when watching the games:
Mainstream \cmo{broadcasting videos}
cannot provide on-demand data 
to fulfill fans' individual needs~\cite{lin2022the};
online webpages (e.g., ESPN~\cite{ESPN}) provide rich historical and game data
but distract fans from the game videos by showing information in separate windows.
Thus,
finding a way to enable seamless access to extra data 
when watching basketball games would particularly benefit casual fans 
in their understanding and engagement of games.

Embedded visualizations provide a promising opportunity
to allow audiences 
to access extra data 
without being distracted from the game video
by directly displaying data in the actual scenes.
% to enable seamless access to extra data 
% when watching basketball videos.
% , 
% embedded visualizations 
Given such benefits,
various commercial products~\cite{vizrt, courtvision}
and research systems~\cite{VisCommentator, chen2022sporthesia}
leverage embedded visualizations 
to augment sports videos.
However, these systems either 
focus on post-game analysis rather than game-watching scenarios,
or only use simple, non-interactive text labels and progress bars to show data.
Recently, 
researchers have started to explore the design space of embedded visualizations for \cmo{game-watching scenarios}
but used low-fidelity simulated environments
(e.g., 3D simulated sports games~\cite{lin2022the}, moving charts on white backgrounds~\cite{yao2022visualization}).
% rather than real game videos.
Little is known about 
how to design and implement 
interactive embedded visualizations in real sports videos
and how they can facilitate game understanding and increase engagement of fans when watching games.

In this work,
we aim to fill this gap by developing interactive embedded visualizations
to assist casual fans in watching basketball game videos.
To understand the particular practices, pain points, and solutions of casual fans
in watching basketball game videos, 
we compared the game-watching behaviors of 8 casual and 8 die-hard fans
in a formative study.
Findings revealed that casual fans are confused
about key players and their in-game decisions from time to time,
and almost never proactively seek extra information to resolve their confusion during or after the game.
Informed by the study, 
we developed \system{} (\autoref{fig:teaser}), 
a basketball game viewing system 
that %assists casual fans in watching live game videos
automatically highlights key players
and visualizes their performance
through gaze-moderated embedded visualizations.

We developed \system{} by tackling two main challenges.
First, 
embedding visualizations into actual scenes 
is recognized as a grand challenge~\cite{DBLP:conf/chi/EnsBCESWPABDDGH21},
especially for basketball, where players overlap heavily
and the camera moves rapidly.
We contribute a CV pipeline based on open-source components to process team sports videos for 
embedding visualizations into these videos,
providing a stepping stone for future research in embedded visualizations.
Second, 
it remains unclear how to design embedded visualizations that
are informative but not overwhelming for individual audiences,
who may have various levels of game literacy, data needs, and personal interests.
We leverage an eye-tracker to track the user's attention
and design a set of gaze-moderated embedded visualizations
that dynamically adapt the visualizations
%, as well as the video scene, 
to highlight the content the user is interested in
and to suppress others.
To evaluate \system{},
we conducted a user study with 16 casual fans
to compare the game-watching experiences 
between raw video (\RAW{}), 
video + embedded visualizations (\AUG{}), 
and video + gaze-moderated embedded visualizations (\FULL{}).
Participants spoke highly of our system,
ranked \FULL{} as the best, 
and confirmed that our embedded visualizations and gaze interactions
are useful, usable, and engaging.
We further discuss our observations and design implications learned from the study for future research inspiration.

In summary,
through developing \system{},
we make the following four main contributions:
1) a formative study that identifies the pain points of casual fans in watching basketball videos
and solicits plausible solutions from die-hard fans,
2) an open-source CV pipeline to process team sports videos for embedding visualizations, 
3) a set of gaze-moderated embedded visualizations for basketball game videos,
4) a user study that assesses our system and provides 
insightful feedback on using gaze-moderated embedded visualizations in live team sports videos.
Finally, we will open source our system at \cmo{\url{https://anonymous-before-published.github.io}}.

==> tex/_deprecated/1-intro_v8.tex <==
\section{Introduction}
% - basketball is good
Basketball, one of the most popular team sports,
has continually attracted new fans
over the past decades due to the proliferation of \cmo{video broadcasting and online video platforms}.
% In the NBA league alone,
% the average number of viewers per game across major US networks has increased to 
% 1.6 million in the last year, 
% up 19\% from the 2020-21 season~\cite{NBAUp}.
% Today, watching basketball games is not just a personal hobby
% but a social activity that connects people, 
% increases solidarity, 
% and boosts social capital. 
% Additionally, it even endorses diversity, inclusion, unity, and teamwork~\cite{}.
However, as our formative study will show,
unlike experienced fans, 
new or casual fans often get confused
when watching basketball videos.
\cmo{
This is because they 
lack sufficient basketball knowledge 
to understand the players' complex teamwork and in-game decisions,
and existing methods 
fall short of providing extra information to solve their confusion:\jb{I would use . not :}}
% and cannot appreciate games at the same deep level of understanding and engagement as experienced fans.
% Basketball games often involve complex teamwork and in-game decisions
% that are made based on large amounts of situated information,
% such as the players' positions, abilities, and roles.
% Unlike experienced fans, 
% casual fans 
% to extract and interpret this information from game videos.
% supporting fans to access extra information when watching the games:
Mainstream \cmo{broadcasting videos}
cannot provide on-demand data 
to fulfill fans' individual needs~\cite{lin2022the};
online webpages (e.g., ESPN~\cite{ESPN}) provide rich historical data
but distract fans from the game videos by showing information in separate windows.
Thus,
finding a way to enable seamless access to extra data 
when watching basketball games would particularly benefit casual fans 
in their understanding and engagement of games.

Embedded visualizations provide a promising opportunity
to allow audiences 
to access extra data 
without being distracted from the game video
by directly displaying data in the actual scenes.
Given such benefits,
various commercial products~\cite{vizrt, courtvision}
and research systems~\cite{VisCommentator, chen2022sporthesia}
leverage embedded visualizations 
to augment sports videos.
However, these systems either 
focus on post-game analysis rather than game-watching scenarios,
or only use simple, non-interactive text labels and progress bars to show data.
Recently, 
researchers have started to explore the design space of embedded visualizations for \cmo{game-watching scenarios}
but used low-fidelity simulated environments
(e.g., 3D simulated sports games~\cite{lin2022the}, moving charts on white backgrounds~\cite{yao2022visualization}).
% rather than real game videos.
Little is known about 
how to design and implement 
interactive embedded visualizations in real sports videos
and how they can facilitate game understanding and increase engagement of fans when watching games.

In this work,
we aim to fill this gap by developing interactive embedded visualizations
to assist casual fans in watching basketball game videos.
To understand the particular practices, pain points, and solutions of casual fans
in watching basketball game videos, 
we compared the game-watching behaviors of 8 casual and 8 die-hard fans
in a formative study.
Findings revealed that casual fans are confused
about key players and their in-game decisions from time to time,
and almost never proactively seek extra information to resolve their confusion during or after the game.
Informed by the study, 
we developed \system{} (\autoref{fig:teaser}), 
a basketball game viewing system 
that %assists casual fans in watching live game videos
automatically highlights key players
and visualizes their performance
through gaze-moderated embedded visualizations.

We developed \system{} by tackling two main challenges.
First, 
embedding visualizations into actual scenes 
is recognized as a grand challenge~\cite{DBLP:conf/chi/EnsBCESWPABDDGH21},
especially for basketball, where players overlap heavily
and the camera moves rapidly.
To tackle this challenge,
we contribute a CV pipeline that \cmo{pre-processes} team sports videos
for embedding visualizations.
\cmo{We also conducted a quantitative evaluation of our pipeline 
and provide guidelines on extending the pipeline to process live videos in the future.}
% for embedding visualizations into .
% providing a stepping stone for future research in embedded visualizations.
Second, 
it remains unclear how to design embedded visualizations that
are informative but not overwhelming for individual audiences,
who may have various levels of game literacy, data needs, and personal interests.
% We leverage an eye-tracker to track the user's attention
We design a set of gaze-moderated embedded visualizations
that leverage the user's gaze---\cmo{a fast, implicit, and expressive input source}---to adaptively 
present the data the user is interested in
and suppress others.
To evaluate \system{},
we conducted a user study with 16 casual fans
to compare the game-watching experiences 
between raw video (\RAW{}), 
video + embedded visualizations (\AUG{}), 
and video + gaze-moderated embedded visualizations (\FULL{}).
Participants spoke highly of our system,
ranked \FULL{} as the best, 
and confirmed that our embedded visualizations and gaze interactions
are useful, usable, and engaging.
We further discuss our observations and design implications learned from the study for future research inspiration.

In summary,
through developing \system{},
we make the following four main contributions:
1) a formative study that identifies the pain points of casual fans in watching basketball videos
and solicits plausible solutions from die-hard fans,
2) an open-source CV pipeline to process team sports videos for embedding visualizations, 
3) a set of gaze-moderated embedded visualizations for basketball game videos,
4) a user study that assesses our system and provides 
insightful feedback on using gaze-moderated embedded visualizations in live \jb{do we keep the word live?} team sports videos.
Finally, we will open source our system at \cmo{\url{https://anonymous-before-published.github.io}}.

==> tex/_deprecated/2-related.tex <==
\section{Related Work}

\subsection{Personalized Game Viewing Systems}
Visualization has long been used in sports to present data~\cite{},
including box scores~\cite{}, tracking data~\cite{}, and meta data~\cite{}.
These visualizations can roughly be divided into two categories:
for post-game analysis purpose
and for in-game informing purpose.
This work mainly focuses on in-game i


Sports, by nature, are highly competitive and usually involve complex in-game decision making.
To better understand, analyze, and appreciate players' in-game decisions,
spectators often look for additional information when watching a sports game~\cite{}.
While modern sports TV broadcasts provide extra information 
through scoreboards and commentaries,
the information needs of individual spectators may vary greatly,
leading to a great demand for personalized game view systems.
Thus, 
researchers from Computer Graphics and HCI have explored interactive systems
to augment game watching experiences with personalized information.
ARSpectator~\cite{}, for example, presents a concept design of using mobile AR to enhance the experience of live sport events.
Gamebot~\cite{} uses a conversational interface that allows users to request data visualizations in watching NBA games through asking questions.
Aside from research projects, only a few commercial products support personalized content.
A representative example is CourtVision~\cite{courtvision}, 
a mobile app developed by Second Spectrum~\cite{secondspectrum}, which provides three modes to allow inspectors to review different basketball in-game data through simple embedded visualizations (e.g., text labels, progress bars).
Compared to traditional sports, most E-Sports are actually ahead in providing personalized game viewing experiences.
MOBA games, such as Defense of the Ancients2~\cite{dota} (Dota2) and League of Legends~\cite{lol} (LoL),
allow audiences to interact with the systems to inspect the in-game data (\emph{e.g.}, points over time) of players or the teams.
Nevertheless, these systems either display the data in separated panels or require audiences to explicitly interact with the system to request the data, inevitably distracting audiences' attention away from the game.
In contrast, we propose to use embedded visualizations implicitly triggered by gaze to merge the extra data into the game video, providing an intuitive, seamless, and engaging watching experience.

\subsection{Visual Analytics for Sports}
Data analytics has long been used in sports to measure players' performance and develop winning tactics~\cite{}.
To facilitate the analysis of sports data,
numerous visual analytics systems have been developed
for stakeholders such as coaches, analysts, and fans.
These visualizations, according to the review of Perin et al.~\cite{PerinVSSWC18},
mainly focus on three kinds of sports data, i.e., 
box score data, metadata, and tracking data.
%% box score
Box score data, due to its cheap and easy acquisition,
has been widely investigated in visualization research.
For example,
based on a comprehensive formative study,
Fu and Stasko~\cite{DBLP:conf/chi/FuS22} developed NBA GameViz and LineupViz, 
two interactive visualization systems, to help NBA journalists in writing data-driven stories.
iTTVis~\cite{} and TenniVis~\cite{} use several coordinated views 
to support the analysis of score data of table tennis and tennis, respectively.
%% tracking
With the rapid development of sensing and CV techniques,
an increasingly amount of 
visualizations systems are being developed for tracking data.
% due to its increasingly availability.
SoccerStories~\cite{SoccerStories}, for example,
focuses on tracking data collected in soccer games
and provides visualizations including in-court trajectories, heatmaps, and text embedded icons.
In basketball,
BKViz~\cite{BKViz} is an early example
of using visualizations of both box score and tracking data
to ease the analysis of play sequences.
Tracking data has also been used to train machine learning models
that automatically predict game results~\cite{skinner2015method} 
and evaluate player performance~\cite{cervone2014pointwise, DBLP:conf/kdd/SiciliaPG19}.
Outside the research community, a number of metrics and models have been developed by basketball analysts and introduced in books such as \emph{Basketball on Paper}~\cite{} and \emph{Sports Analytics-Spatial Tracking}~\cite{} to evaluate and predict players' performance based on tracking data.
Recently, due to the proliferation of consumer-grade Virtual Reality (VR) devices,
researchers have explored using immersive visualizations to present tracking data in simulated courts~\cite{ShuttleSpace, TIVEE}.
% For example, 
% ShuttleSpace~\cite{ShuttleSpace} and TIVEE~\cite{TIVEE}, two VR-based visual analytics systems for badmiton,
% enable users to explore a large scale of shuttle trajectories from first and third-person views in the court.
% Users can also use VR controllers to interact with the tracking data by using embodied interactions, such as performing a stroke to select the targeted trajectories.
Different from traditional desktop systems,
these immersive systems can visualize tracking data in a simulated 3D court
so that users can not only see but also experience the data,
thereby increasing spatial understanding and peripheral awareness~\cite{marriott2018immersive,lin2020sportsxr}.
Lastly, 
% metadata has been gaining relatively less traction.
% sports meta-data
% , such as physical characteristics of players,
% can be visualized together with box-score and tracking data to provide context details beyond a specific game.
only little research has been done on visualizations for meta-data.
A typical example comes from Vuillemot and Perin~\cite{DBLP:journals/cga/VuillemotP16},
who used a visualization of tournament brackets with direct manipulations to support tournament prediction.

While these visualization systems have successfully showcased their usefulness in analyzing sports data,
they all target sports analysts %in post-game analysis. 
and are designed for post-game analysis.
Visualizations designed for casual fans in live game scenarios can be significantly different than those existing works 
as casual fans often lack sufficient knowledge about the games 
and the games are usually fast-paced and intense.
Only a few studies explore visualizations for live game scenarios.
For instance, 
Zhi et al.~\cite{DBLP:conf/chi/ZhiLSM19} use simple visualizations (\emph{e.g.}, line charts)
to show in-game box scores of basketball games.
Lin et al.~\cite{} have investigated embedded visualizations to support experienced fans in their in-game analysis.
The above works, however, all target experienced basketball fans who have rich basketball knowledge and actively seek data when watching the games.
By contrast, we aim to help casual fans, who are new to basketball and often do not even know what type of data they need to understand a game, by using personalized embedded visualizations.

% We also aim to augment basketball viewing experiences using embedded visualizations
% but target casual fans,
% use real broadcasting videos,
% and provide gaze-based interactions.
% and can hardly be used for live game scenarios.
% in-game scenarios.
% To show data in a live game,
% the visualizations must be lightweight and not distracting
% since sports games are usually 
% However, only a few methods explore visualizations for in-game analysis.
%  augmenting basketball watching experiences with 
% They targeted experienced fans and
% used 3D simulated basketball games, instead of videos, as a design probe
% to explore the effectiveness of various embedded visualizations.


\subsection{Embedded Visualizations in Sports Videos}
An embedded visualization blends data into its physical context (\emph{e.g.}, a basketball court) to 
% reduce the context switching and 
facilitate the understanding of the data.
As such, embedded visualizations have been widely used for sports data, which is inherently associated with its physical context.
Early works mainly embedded the data into static court diagrams.
Examples such as CourtVision~\cite{goldsberry2012courtvision} (basketball), StatCast Dashboard~\cite{DBLP:journals/cga/LageOCCDS16} (baseball),
and SnapShot~\cite{DBLP:journals/tvcg/PileggiSBS12} (ice hockey) use density maps to show sports events, usually shots, 
on the court diagrams to depict the performance of a player or a team.
Sacha et al.~\cite{DBLP:journals/cgf/SachaASSKAJ17} introduced an interactive visualization technique
that allows users 
to adjust the level of abstraction of the moving trajectories of soccer players.
Stein et al.~\cite{DBLP:journals/cga/SteinJBSSGCK16} 
animated the movement of soccer players on the court diagram
and dynamically visualized the interaction space of each player.
In recent years, progress in CV and image processing
has gradually shifted research interest from embedding visualizations into court diagrams to directly embedding visualizations into sports videos.
For example, Stein et al.~\cite{DBLP:journals/tvcg/SteinJLBZGSAGK18, DBLP:conf/bdva/SteinBHSNSGKJ18} developed a method to automatically extract and visualize data from and in soccer videos.
Chen et al.~\cite{VisCommentator} explored the design of augmented sports videos
and introduced VisCommentator to ease the augmentation of racket-based sports videos.
They further developed Sporthesia~\cite{} to enable users
to create augmented videos for racket-based sports by directly using textual comments.
Nevertheless, 
these works mainly target experts for analytic and authoring purposes
and do not fulfill general audiences' needs in live game watching scenarios.
More recently, 
Yao et al.~\cite{} proposed the notion of \emph{visualization in motion}
to depicts visualizations that are relatively moving to the viewer
and summarized a design space and a research agenda for it.
Embedded visualizations in sports videos also fall into this category.
Lin et al.~\cite{} presented a design framework 
for designing embedded visualizations 
to facilitate the in-game analysis when watching basketball games.
We design our embedded visualizations based on prior work
but particularly focus on the concrete goal of helping casual fans, who lack sufficient basketball knowledge, to better understand basketball games without overwhelming them.
\cmo{where to emphasize actual games?}



\subsection{Gaze-based Interactions}
%% maybe need more works from Andreas Bulling: https://www.perceptualui.org/publications/
There is a long history of interest in leveraging gaze for interactions 
due to its efficiency, expressiveness, and applicability in hands-free scenarios~\cite{DBLP:journals/tochi/MengesKS19, majaranta2014eye, DBLP:journals/pervasive/BullingG10}.
Extensive research has been conducted to develop gaze-based interactions that \emph{explicitly} or \emph{implicitly} leverage gaze to interact with digital contents for different application domains, such as classroom teaching~\cite{gazeclassroom, DBLP:journals/mta/AsteriadisTKK09},
remote collaborations~\cite{DBLP:journals/pacmhci/KuttTRMSKP20, DBLP:journals/tvcg/BeckKKF13}, and biomedical image analysis~\cite{karargyris2021creation, corredor2017training}.
In this work, we focus on implicit methods
and refer readers to a more comprehensive review~\cite{majaranta2014eye} for further reading.

%% what is implicit gaze interactions
Implicit gaze-based systems use gaze as an implicit input source, usually in combination with other input modalities,
to facilitate interactions~\cite{DBLP:conf/chi/FeitWTPKKM17, majaranta2014eye}.
Given that reliable eye trackers are now affordable enough to be integrated into desktop and laptop computers,
researchers have leveraged implicit gaze interactions to support a variety of day-to-day activities.
%% gaze for annotations
For example, 
% since gaze can reflect users' understanding of the content during reading,
researchers have recorded users' gaze to generate content annotations automatically.
Cheng et al.~\cite{DBLP:conf/chi/ChengSSYD15} have introduced a system that automatically generates
annotations of a paper from a user's gaze in reading the paper.
Templier et al.~\cite{DBLP:conf/chi/TemplierBH16} have proposed a gaze-based image annotation approach 
for volumetric microscopy images, where the user annotations are subsequently used for segmenting neuronal fibers.
% gaze for authoring
Gaze has also been used for content creation.
By collecting and analyzing audiences' gaze on raw footages,
Jain et al.~\cite{retargeting1} presented an algorithm that
uses pan, cut, and zoom operations
to convert an edited video to a device with different aspect ratio (so called \emph{retargeting}).
Their method was improved by Rachavarapu et al.~\cite{retargeting2}
to reduce its computational cost.
Similarly,
Moorthy et al.~\cite{shotselection} have exploited gaze data to select shots from monocular video recordings and generate virtual camera movements, \emph{e.g.}, pan, tilt, and zoom.
%% gaze-based remote collaboration
Moreover, there has been a growing trend in implicitly leveraging gaze movement to facilitate
remote collaboration.
Eye-Write~\cite{DBLP:conf/chi/KuttLHP19}, for example, 
allows co-authors to see their partners' gaze within a text editor,
thereby improving the collaboration quality.
GazeChat et al.~\cite{gazechat} uses webcam to track users' gaze and generates gaze-aware 3D profile photos,
increasing the sense of presences during teleconferences.
%% gaze-adaptive content
The most relevant to our endeavor 
are attempts at adapting viewing contents based on users' gaze.
A typical example is a gaze-contingent display,
explored in the early 2000s~\cite{DBLP:journals/cbsn/DuchowskiCM04},
which shows a higher resolution on the area where the user is focusing on.
%In recent years, researchers has utilized gaze to adapt more contents.
Other examples include 
Nguyen and Liu's work~\cite{DBLP:conf/chi/NguyenL16} on adjusting the video playback speed while a user is watching lecture videos based on the user's gaze.
Kwok et al.~\cite{DBLP:conf/chi/KwokKSAR19} have developed a tourist guide that directs a user's gaze to highlighted features in a panorama and adapts the audio introductions accordingly.
Kurzhals et al.~\cite{gazecaption} have proposed a gaze-adaptive system that dynamically adjusts video captions' placement to optimize the viewing experience.
We also aim to use gaze to adjust video content but focus on augmented sports videos.

% Displaying Teacher’s Gaze in a MOOC: Effects on Students’ Video Navigation Patterns
% Towards Measuring and Inferring User Interest from Gaze

In the visualization field, research related to gaze mainly focuses on visualizing gaze-data~\cite{sotaVisGaze, DBLP:journals/tvcg/KurzhalsHHBEW16} and analyzing users' gaze in viewing visualizations~\cite{DBLP:journals/tvcg/BorkinBKBYBPO16, DBLP:conf/uist/BylinskiiKOAMPD17}.
Only a few works~\cite{DBLP:journals/cgf/OkoeAJ14, DBLP:conf/fmt/SilvaSSEF16, DBLP:conf/etra/SilvaSVSEF18, DBLP:conf/iui/ShaoSES17} have explored leveraging gaze to interact with visualization systems.
Silva et al.~\cite{DBLP:conf/etra/SilvaBJRWRS19} have systematically reviewed eye tracking support for visual analytics systems, identified research challenges and summarized a roadmap to broaden the use of eye tracking for visualization systems.
We draw on this line of research and, to the best of our knowledge, are the first to explore gaze-aware embedded visualizations to improve the sports watching experience.


\subsection{Computer Vision for Embedded Visualizations}
Recent years have witnessed remarkable advancement in CV techniques based on deep learning.
Researchers have achieved unprecedented success in a broad range of tasks including
object detection~\cite{}, object tracking~\cite{}, pose estimation~\cite{}, and segmentation~\cite{}.
Thanks to these progress,
more and more data is available to be extracted from videos~\cite{},
opening new opportunities for sports analytics.
For example, 
% SoccerNet~\cite{} is a large-scale soccer video dataset that supports various tasks including action spotting, camera calibration, player re-identification and tracking. 
the positions of the players and the ball~\cite{}, as well as other tracking data~\cite{}, in each NBA game are extracted and shared online.
We refer the reader to Shih~\cite{shih2017survey} for a comprehensive survey on content-aware video analysis for sports.
Besides extracting data from videos,
these new CV techniques make registering, or embedding, 
visualizations into the video scenes easier,
which is recognized as a grand challenge in situated visualization~\cite{}.
To embed a visualization of a player into the video scene,
one usually needs to detect~\cite{}, % (bounding box), 
track~\cite{}, % (identify), 
and segment~\cite{} %, (mask) 
the player from the video, 
estimate her/his pose~\cite{},
calibrate the camera~\cite{},
and sometimes reconstruct the 3D scene~\cite{}.
% using the video as the major input.
Prior works~\cite{} applied a simplified CV pipeline 
to process racket-based sports videos,
in which the players are separated and the camera is mostly static.
However, it is much difficult to embed visualizations into team sports, especially basketball, videos
since the players overlap heavily and the camera moves rapidly.
While commercial systems~\cite{} can achieve good embedding results,
% to the best of our knowledge, 
there is no publicly available CV solution 
for embedding visualizations into basketball videos.
The lack of such a CV solution inevitably hinders the research of embedded visualizations in complex, dynamic scenarios, such as team sports.
In this work,
we explore this issue 
and contribute a CV solution that consists of several modular components
to process basketball videos
for embedding visualizations.

% In this work,
% we composite multiple state-of-the-art machine learning models~\cite{ttnet, bodypiex2, he2016}
% to extract the data from table tennis videos, % with a fixed camera angle.
% such as ball and players' position, actions, events, and key strokes.
% 1) object level includes the data of video objects in each frame,
% 2) event level contains the actions of objects,
% and 3) conclusion level 
% embedded visualizations in sports videos:
%% rendering
% tracking identity
% overlapping
% He summarized the state-of-the-art techniques to parse sports videos
% from a low-semantic to a high-semantic level:
% 1) object level techniques extract the key objects in the video, 
% 2) event level recognizes the action of the key object, 
% and 3) conclusion level generates the semantic summarization of the video.
% Besides models tailored to sports videos,
% researchers have also developed models~\cite{nguyen2016} to detect and segment humans from general images and videos.
% A particular challenge in table tennis is that
% the ball is small (15 pixels on average~\cite{ttnet}) 
% and move fast (\emph{e.g.}, $30$ $m/s$).
% To tackle this challenge, Voeikov et al.~\cite{ttnet}
% proposed TTNet, a convolution-based neural network,
% to detects the ball in a high-resolution video.
% Besides, TTNet can further segments the ball 
% and detect ball events such as bounces and net hits.

==> tex/_deprecated/2-related_v2.tex <==
\section{Related Work}
We review prior work on personalized game viewing systems,
embedded visualizations in sports videos,
computer vision for embedded visualizations,
and applications of gaze interactions.

\subsection{Personalized Game Viewing Systems}
Visualization has long been used in sports to present data~\cite{PerinVSSWC18},
including box scores~\cite{DBLP:conf/chi/FuS22}, tracking data~\cite{SoccerStories, BKViz, ShuttleSpace, TIVEE}, and meta data~\cite{DBLP:journals/cga/VuillemotP16}.
Sports visualizations are mainly used for post-game analysis or for in-game informing purposes.
This work mainly focuses on the latter.

Sports games usually involve complex in-game decision-making.
To better understand, analyze, and appreciate players' in-game decisions,
spectators often look for additional information when watching a sports game~\cite{lin2022the}.
To fulfill individual spectators' information needs, prior research has 
explored the design of interactive game-watching systems.
ARSpectator~\cite{DBLP:conf/siggrapha/ZollmannLLLB19}, for example, presents a concept design of using mobile AR to enhance the experience of live sports events.
Gamebot~\cite{DBLP:conf/chi/ZhiM20} uses a conversational interface to help users request data visualizations in watching NBA games. % by asking questions.
GameViews~\cite{DBLP:conf/chi/ZhiLSM19} uses simple visualizations (\emph{e.g.}, line charts)
to show in-game box scores of basketball games.
Omnioculars~\cite{lin2022the} uses interactive embedded visualizations to support in-game analysis of basketball games.
%Aside from research projects, 
%a few commercial products for traditional sports also support personalized content.
%For instance,
CourtVision~\cite{courtvision} is a commercial product that
allows inspectors to review basketball in-game data through simple, non-interactive embedded visualizations (e.g., text labels, progress bars).
% Recently, 
% Nixon et al.~\cite{nixon2022data} presented a survey about selecting TV content based on personal preference.
Compared to traditional sports, 
most E-Sports already provide a personalized game viewing experience by default.
% actually ahead in providing personalized game viewing experiences.
MOBA games, such as Defense of the Ancients2~\cite{dota} (Dota2) and League of Legends~\cite{lol} (LoL),
allow spectators to interact with the systems to inspect in-game data (\emph{e.g.}, points over time) of players or teams.
Nevertheless, these systems either display the data in separated panels 
or require viewers to explicitly interact with the system to request the data, 
inevitably distracting viewers from the game.
In contrast, we propose to use embedded visualizations and gaze interactions
to present extra data in game videos,
providing an intuitive, seamless, and engaging watching experience.

\subsection{Embedded Visualizations in Sports Videos}
% Embedded visualizations 
% facilitate the understanding of data
% by showing the data into its physical context (\emph{e.g.}, a basketball court).
% Subsequently,
Embedded visualizations have been widely used for sports data
due to their ability to show the data into its physical context (\emph{e.g.}, a basketball court).
% which is inherently associated with its physical context.
Early works mainly embedded the data into static court diagrams.
Examples such as CourtVision~\cite{goldsberry2012courtvision} (basketball), 
StatCast Dashboard~\cite{DBLP:journals/cga/LageOCCDS16} (baseball),
and SnapShot~\cite{DBLP:journals/tvcg/PileggiSBS12} (ice hockey) 
display density maps on top of court diagrams to show sports events, 
such as successful shots. %, to depict the performance of a player or a team.
Recent progress in CV
now allows embedding visualizations directly into sports videos instead of just court diagrams.
For example, Stein et al.~\cite{DBLP:journals/tvcg/SteinJLBZGSAGK18, DBLP:conf/bdva/SteinBHSNSGKJ18} 
developed a method to automatically extract and visualize data from and in soccer videos.
Chen et al.~\cite{VisCommentator, chen2022sporthesia} explored the design of augmented sports videos
and introduce fast prototyping tools to help users create augmented videos for racket-based sports
by using direct manipulation and textual comments.
However,
these works mainly target experts for analytic and authoring purposes.
% and do not fulfill the needs of a general audience in live game-watching scenarios.
More recently, 
researchers have started to explore embedded visualizations in live game-watching scenarios.
Yao et al.~\cite{yao2022visualization} proposed the notion of \emph{visualization in motion}
to depict visualizations that are moving relative to the viewer
and summarized a design space for it.
% Embedded visualizations in sports videos also fall into this category.
Lin et al.~\cite{lin2022the} presented a design framework 
for embedded visualizations to facilitate in-game analysis when watching basketball games.
Yet, all the above works only evaluated visualizations in simulated scenarios 
(e.g., moving charts on white backgrounds, 3D virtual sports games).
We design our embedded visualizations based on these prior works
but particularly target live basketball videos,
with the aim to understand how embedded visualizations can improve casual fans' game-watching experience.

\subsection{Computer Vision for Embedded Visualizations}
Recent years have shown remarkable advances in CV techniques based on deep learning.
Researchers have achieved unprecedented success in a broad range of tasks including
object detection~\cite{yolox2021, liu2021Swin}, 
object tracking~\cite{aharon2022bot, zhang2022bytetrack}, 
pose estimation~\cite{xu2022vitpose}, 
and segmentation~\cite{chen2022vitadapter}.
Thanks to this progress,
more and more data can be extracted from videos (e.g., \cite{DBLP:conf/cvpr/DeliegeCGSDNGMD21, DBLP:conf/cvpr/RamanathanHAG0F16, DBLP:journals/corr/KayCSZHVVGBNSZ17, DBLP:conf/cvpr/GuSRVPLVTRSSM18}),
opening new opportunities for sports analytics.
For example, 
the positions of the players and the ball~\cite{sportvu}, as well as other tracking data~\cite{nbashotcharts, nbastats}, 
of each NBA game are extracted and shared online.
We refer the reader to Shih~\cite{shih2017survey} for a comprehensive survey on content-aware video analysis for sports.
%Besides extracting data from videos,
Furthermore, these new CV techniques ease the embedding
of visualizations into the video scenes,
which is recognized as a grand challenge in situated visualization~\cite{DBLP:conf/chi/EnsBCESWPABDDGH21}.
Embedding visualizations into sports videos
requires a CV pipeline completing tasks such as
detecting, % (bounding box), 
tracking, % (identify), 
and segmenting %, (mask) 
the players from the video, 
estimating their pose,
calibrating the camera~\cite{DBLP:journals/pami/Zhang00},
and sometimes reconstructing the 3D scene~\cite{DBLP:journals/cacm/MildenhallSTBRN22}.
% using the video as the major input.
Prior works~\cite{VisCommentator, chen2022sporthesia, DBLP:journals/tvcg/SteinJLBZGSAGK18} applied a simplified CV pipeline 
to process racket-based sports videos,
in which the players are separated, and the camera is mostly static.
However, it is much more difficult to embed visualizations into team sports videos (especially basketball)
since players overlap heavily and the camera typically moves rapidly.
While commercial systems~\cite{courtvision} can achieve good embedding results,
% to the best of our knowledge, 
there is no publicly available CV solution 
for embedding visualizations into basketball videos.
The lack of such a solution inevitably hinders the research of embedded visualizations in complex, dynamic scenarios, such as team sports.
In this work,
we explore this issue 
and contribute a CV pipeline that consists of open-sourced modular components
to process team sports videos for embedding visualizations.

\subsection{Applications of Gaze Interactions}
%% maybe need more works from Andreas Bulling: https://www.perceptualui.org/publications/
There is a long history of interest in leveraging gaze for interactions 
due to its efficiency, expressiveness, and applicability in hands-free scenarios~\cite{DBLP:journals/tochi/MengesKS19, majaranta2014eye, DBLP:journals/pervasive/BullingG10}.
%Extensive research has been conducted to develop 
Gaze interactions either \emph{explicitly} or \emph{implicitly} leverage gaze to interact with digital contents. 
% Different application domains include classroom teaching~\cite{gazeclassroom, DBLP:journals/mta/AsteriadisTKK09},
% remote collaborations~\cite{DBLP:journals/pacmhci/KuttTRMSKP20, DBLP:journals/tvcg/BeckKKF13}, and biomedical image analysis~\cite{karargyris2021creation, corredor2017training}.
In this work, we focus on implicit methods
and refer readers to a more comprehensive review~\cite{majaranta2014eye} for further reading.

%% what is implicit gaze interactions
Implicit gaze-based systems use gaze as an implicit input source, 
usually in combination with other input modalities,
to facilitate interactions~\cite{DBLP:conf/chi/FeitWTPKKM17, majaranta2014eye}.
Given that reliable eye trackers are now affordable enough to be integrated into desktop and laptop computers,
researchers have leveraged implicit gaze interactions to support a variety of applications,
such content annotation~\cite{DBLP:conf/chi/ChengSSYD15, DBLP:conf/chi/TemplierBH16},
video editing~\cite{retargeting1, retargeting2, shotselection},
and remote collaborations~\cite{DBLP:conf/chi/KuttLHP19, gazechat}.
The most relevant to our endeavor 
are attempts at adapting viewing content based on users' gaze.
%A typical example is a 
The gaze-contingent display~\cite{DBLP:journals/cbsn/DuchowskiCM04}, for example,
shows a higher resolution on the area the user is focusing on.
Other examples include adjusting the playback speed of lecture videos based on the user's gaze~\cite{DBLP:conf/chi/NguyenL16}, or a tourist guide that directs a user's gaze to highlighted features in a panorama and adapts the audio introductions accordingly~\cite{DBLP:conf/chi/KwokKSAR19}.
Kurzhals et al.~\cite{gazecaption} have proposed a gaze-adaptive system that dynamically adjusts video captions' placement to optimize the viewing experience.
We also aim to use gaze to adjust video content but focus on augmented sports videos.

In the visualization field, research related to gaze mainly focuses on visualizing gaze-data~\cite{sotaVisGaze, DBLP:journals/tvcg/KurzhalsHHBEW16} and analyzing users' gaze in viewing visualizations~\cite{DBLP:journals/tvcg/BorkinBKBYBPO16, DBLP:conf/uist/BylinskiiKOAMPD17}.
Only a few works~\cite{DBLP:journals/cgf/OkoeAJ14, DBLP:conf/fmt/SilvaSSEF16, DBLP:conf/etra/SilvaSVSEF18, DBLP:conf/iui/ShaoSES17} have explored leveraging gaze to interact with visualization systems.
Silva et al.~\cite{DBLP:conf/etra/SilvaBJRWRS19} give a systematic review on eye tracking for visual analytics systems and current challenges.
%, identified research challenges and summarized a roadmap to broaden the use of eye tracking for visualization systems.
We draw on this line of research and, to the best of our knowledge, are the first to explore gaze-aware embedded visualizations to improve the sports-watching experience.


==> tex/_deprecated/3-formative_v1.tex <==
\section{Formative Study with Basketball Fans}

To understand the practices, pain points, and requirements of casual fans in watching live basketball videos,
a formative study was conducted.

\subsection{Study Setup}

\paragraph{Participants.}
We recruited participants using university mailing lists and forums, 
and used a prescreening survey (\cmo{in supplemental material}) to select participants 
based on their fandom level, game watching frequency, and basketball knowledge. 
In total we recruited 8 casual fans (P1-P8; M=3, F=5; Age: 18 - 35),
who only knew \quot{basic rules of basketball} and watched \quot{1 - 10 games per year}.
To better identify the pain points specific to casual fans, 
we further recruited 8 die-hard fans (P9 - P16; M=8; Age: 18 - 55), who knew \quot{basketball tactics and pros and cons of specific players} and watched \quot{at least 1 game per week}. No female die-hard fan responded to us.
All participants had normal vision or wore contact lenses or glasses to correct to normal vision.

{\renewcommand{\arraystretch}{1.3}% for the vertical padding
\begin{table}[h]
\begin{threeparttable}
    \centering
    \caption{Context information of the two game videos in the formative study.}
    \begin{tabular}{c c c c c c c c}
    % \toprule
     & \textbf{Date} & \textbf{Teams} & \textbf{Quarter} & \textbf{Scores} & \textbf{Game Clock (m:ss)} & \textbf{Video Duration (m:ss)} \\ \midrule
    %% -----
    \textbf{G1} & 2015.12.25 & GSW vs. CLE\tnote{*} & 4 & 67 : 71 & 7:00 & 9:02\\ \hline
    \textbf{G2} & 2015.12.22 & OKC vs. LAC\tnote{*} & 4 & 83 : 89 & 6:11 & 9:30\\
	\bottomrule
    \end{tabular}
    \label{tab:study1_games}
    %%% ---- 
	\begin{tablenotes}\footnotesize
    \item[*] GSW (Golden State Warriors), CLE (Cleveland Cavaliers), OKC (Oklahoma City Thunder), and LAC (Los Angeles Clippers)
    \end{tablenotes}
\end{threeparttable}
\end{table}
}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig_31_study_setup.pdf}
    \caption{a) Formative study setup. 
    b) In the review session, the participant's gaze is visualized in purple and overlaid on the video.}
    \label{fig:study_setup}
\end{figure}

\paragraph{Procedure.}
We started each session by introducing our research motivation and study protocol.
The experimenter then conducted a semi-structured interview with each participant, focusing on their current practices, pain points, and solutions in watching live basketball games.
Next, we followed the format of \emph{contextual query}~\cite{hartson2012ux}
to asked participants to watch two game videos of an NBA regular-season (\autoref{tab:study1_games})
on a 24-inch monitor. %, each last for about 9 minutes.
These two games were rated as top-30 games of the season 
and have been watched millions of times.
Before watching the games, 
the experimenter asked participants to pretend watching the game in a real-world scenario 
and encouraged them to think-aloud as much as possible.
We collected think-aloud and gaze data during the game watching process.
To collect the gaze data, we used Eyeware Beam~\cite{Eyeware},
a commercial software that leverages Apple's TrueDepth camera~\cite{TrueDepth}
to track the participant's head and gaze.
The participants sat approximately 60cm from the screen
and were asked to adjusted their chair prior to watching the videos (\autoref{fig:study_setup}a).
The system was then calibrated and the participants
were allowed to move their head freely after the calibration.
We used a TrueDepth camera based tracker as 
it provided sufficient accuracy~\cite{DBLP:conf/hci/GreinacherV20} 
for inspecting what video objects the participants were looking at during watching the game,
while requiring much less budget compared to proficient eye-trackers (e.g., Pupil Core~\footnote{https://pupil-labs.com/products/core}, > \$3K).
However, proficient eye-trackers are required 
if the research needs to analyze more fine-grained gaze data (e.g., saccades, fixation).

After watching each game video,
we asked participants to re-watch the game with their gaze data overlaid (\autoref{fig:study_setup}b)
and to elaborate their confusion, data needs, insights, and excitement they had 
when watching the game for the first time.
Participants could pause the video in the review session.
Each participant was compensated with a \$20 giftcard for their time (1 hour).

\paragraph{Analysis.}
Interviews and think-alouds were audio-recorded, 
transcribed, 
and analyzed using a reflexive thematic analysis~\cite{}.
Three authors coded independently on the transcriptions to form sets of plausible codes
and iteratively refined the codes to converge on a single coding schema,
focusing on the poor watching experience in watching the games.
Disagreements were resolved through discussions.
Moreover,
three authors analyzed the gaze data
by manually annotating
the video object each participant 
was looking at when watching the games.
The categories of objects (\autoref{tab:study1_gaze} header) 
were generated both inductively (i.e., bottom-up, based on the data) 
and deductively (i.e., top-down, based on prior knowledge).
A participant was considered as looking at an object only when his/her gaze
rested on the object for at least 0.25 second (fixation duration~\cite{}). 
The duration when the participant moved his/her gaze to the object
was also annotated as looking at the object.

% {\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{table}[h]
    \centering
    % \vspace{-0.5mm}
    \caption{The gaze distribution in seconds.}
    \label{tab:study1_gaze}
    % \vspace{-0.5em}
    \begin{tabular}{c | c| c c c c c c c c c}
    \toprule

    \multicolumn{1}{c}{}  & \textbf{Fans} & \textbf{Player w/ ball} & \textbf{Player w/o ball} & \textbf{Referee} & \textbf{Basket} & \textbf{Score} & \textbf{Time} &\textbf{Ball} &\textbf{Others} &\textbf{Total}\\ \midrule
    %% -----
    \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{G1}}} & \textbf{Casual} & 254.39 & 141.10 & 4.74 & 27.32 & 23.65 & 9.98 & 3.66 & 75.55 & 540.39 \\ \cline{2-11} 
     & \textbf{Die-hard} & 212.54 & 180.48 & 4.68 & 28.25 & 28.13 & 9.05 & 7.42 & 68.89 & 539.44\\ \hline
    \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{G2}}} & \textbf{Casual}   & 221.63 & 115.41 & 4.80 & 30.01 & 37.54 & 14.33 & 2.78 & 134.36 & 560.86\\ \cline{2-11} 
     & \textbf{Die-hard} & 199.70 & 144.38 & 4.80 & 23.52 & 27.74 & 8.53 & 4.49 & 149.32 & 562.48 
 \\
	\bottomrule
\end{tabular}
\end{table}
% }

\subsection{Findings and Discussions}

%% Practices of Watching Live Basketball Games
All casual fans we interviewed
watched \quot{1 - 10 games per year}, mostly \quot{the important games, such as semi-finals or finals.} (P1-P8) 
Overall, they were not familiar with basketball games and the NBA, 
stating that they \quot{only knew the basic rules} of basketball
and \quot{the names of some superstars}, such as \quot{James} and \quot{Curry}. 
While they were not fans of particular teams or players, 
they did prefer some teams due to some personal connections. 
For example, 
most of the participants supported the team of their city 
(e.g., Boston Celtics); 
one participant particularly felt connected to Stanley since he was her high school's alumni. 
As for the game watching medium, 
all casual fans reported that they only watch live NBA games on TV,
usually with their die-hard fan friends at home or at bars.
In comparison, 
the die-hard fans we interviewed watched basketball games much more frequently, either with friends or alone. 
They had a rich knowledge about basketball (e.g., tactics), 
knew almost all NBA players, 
and even their strengths and shortcomings. 
TV was also the main way for die-hard fans to watch live basketball games.
Overall, for casual fans, watching live basketball games is a leisure activity, such as watching a movie or hiking, 
but it is a more serious hobby for die-hard fans. 

\subsubsection{\textbf{Casual Fans' Confusion in Watching Live Basketball Games}}

\noindent
In terms of the watching experience, 
all 16 participants confirmed that 
they were confused from time to time when watching basketball games 
and that they would like to seek extra information, other than the data provided by the scoreboard and commentaries.
Some confusion is common in both casual and die-hard fans, 
such as questions like \quot{who get a foul?} and \quot{which team called the timeout?}
These questions can usually be resolved easily by \quot{watching a replay of the game} (P5, P11) or simply by \quot{searching Google.} (P12)
However, we did identify some confusing aspects specific to casual fans 
that cannot be easily resolved by the current live streaming techniques, 
and which lead to a poor watching experience:

% \vspace{-4mm}
\paragraph{C1: Casual fans are confused about which players they should focus on.}
\label{para:C1}
In a basketball game, 
the importance of players varies 
based on their skills, roles, and positions. 
% Focusing more on the key players can 
\cmo{one more sentence to explain the necessity of focusing on key players?}
However, 
it is challenging for casual fans to identify the key players from the 10 moving players. 
Casual fans described that they did not understand the players' roles, 
the purpose of their movements, and their expected actions. 
Thus, casual fans often did not know whom to focus on when watching a game and felt that the players were just \quot{10 moving objects.} (P6)

The casual fans' inability to identify key players was also reflected in the participants' gaze patterns.
In our study, we found that casual fans spent more time on the player with the ball, 
while die-hard fans allocated more attention on other players (\autoref{tab:study1_gaze}). 
When we asked the reasons in the review session,
most of the casual fans explained that they focused on the player with the ball 
since they \quot{do not know who else I should look at.} (P1)
As a result, 
casual fans often missed important off-ball movements and felt that the ball \quot{is magically passed to a player who is empty.} (P1) 
Moreover, we also noticed some rapid zigzag movement in the gaze of casual fans between the player with the ball and other players, 
revealing their attempts to watch other players without the ball.
P6, for example, explained that she was trying to look for the player whom the ball would be passed to, 
while keeping an eye on the player with the ball.
However, she had to \quot{scan through the players one-by-one}
and felt such kind of scanning was \quot{exhausting} due to the heavy cognitive load.
Differently, 
die-hard fans scanned through the players much more effectively and predicatively, 
and often could directly identify the key player who, for example, would get the ball at the next pass. 

% explained that she was trying to look for the player whom the ball would be passed to but 
% Meanwhile, she was “worry about losing the ball.” 
% In our study, we observed several bahaviours that indicated poor watching experience due to the inability of identifying key players: 
% Since casual fans cannot identify other key players, 
% According to the gaze data, the casual fans spent X and X secs on the ballholder and others in average, while the die-hard fans spent X and X secs on each of them (Table. []). 

% Some casual fans (PX - X) attempted to inspect other players instead of only focusing on the ballholder. However, since they cannot efficiently identify the key players, they usually have to scan the players one-by-one, while keeping an eye on the ballholder, leading to a huge cognitive load. 
% In summary, since the casual fans cannot identify the key players, they either tended to focus more on the ballholder but failed to notice important off-ball movements, or attempted to inspect the off-ball movements but suffered from high cognitive loads.

\paragraph{C2: Casual fans are confused about the in-game decisions of players.}
\label{para:C2}
Even when casual fans focused on a specific player,
they usually could not understand the in-game decisions of the player. 
As a highly tactical and competitive sport, 
a basketball game includes numerous in-game decisions made by the players 
based on 
% the specific situation that involves 
situated factors such as the players’ abilities, positions, and shooting touches. 
However, these factors were mostly unknown or hard to interpret from the videos 
for casual fans, 
who only \quot{know the basic rules of basketball.}
Thus, casual fans could hardly understand the in-game decisions of the players.

Without understanding the in-game decisions of the players, 
casual fans could not appreciate and enjoy the game at the same deep level 
as die-hard fans 
and had difficulties to \quot{keep pace with other experienced spectators.} (P6)
This was also revealed in the study.
While we particularly encouraged the participants to think-aloud in the study,
most of the casual fans rarely provided meaningful comments when watching the two videos.
The most frequent verbal feedback from casual fans were interjections, e.g., \quot{Oops}, \quot{Wooooow!}
Furthermore, 
even in the follow up review session,
the casual fans could hardly describe their thoughts in watching the games.
As P3 acknowledged, 
she actually \quot{did not know what [she] was thinking of the game ... but just felt excited.}
By contrast, die-hard fans could clearly elaborate, comment on, and even suggest tactics of the players when watching the games. 
Generally speaking, 
our study suggested that
the casual fans' experience was closer to ``feeling'' the game
while the one of die-hard fans was closer to ``reading'' the game.
% \cmo{should echo back to the confusion of in-game decision making.}

\paragraph{C3: Casual fans rarely resolve their confusion proactively.}
% Despite that the confusion can result in poor watching experience,
% the casual fans seldomly resolve their confusion proactively.

Casual fans attributed their confusion to the limited information provided by the live streams.
All casual fans we interviewed provided that 
the commentaries and scoreboard of the live streams
were the primary way for them to obtain extra information about the game.
However, the information provided by live streams lacks diversity and controllability.
\quot{The commentaries are not enough for me to understand the game}, said PX.
Some participants further complained that
the scoreboard, although sometimes showing useful information, 
was annoying as it \quot{disappears before I finish reading it.} (PX)
In addition to the commentary and scoreboard,
some casual fans remarked that sometimes they tried to understand the game 
by listening to the cheering of the audience.
PX said that \quot{at least I can know if the shot is a good one [from the background cheering].}

Even though current live streams cannot provide enough information for casual fans to understand a game, casual fans rarley search extra information proactively, to resolve their confusion.
All casual fans we interviewed confirmed that they never search the internet to seek data while watching games.
The ''annoying'' context switching between the game and websites was a primary reason that made casual fans reluctant to search for extra data.
Specifically, casual fans thought that the game
\quot{is already overwhelming} and they could {miss a lot when looking up a webpage.} (PX)
On the other hand, die-hard fans noted that they frequently search third-party websites (e.g., ESPN) when watching basketball games,
though they also complained about the context switching between the game videos and another window, e.g., the mobile phone.
This finding revealed to us another main difference between casual fans and die-hard fans,
which is that casual fans \quot{did not know what to search for.} (PX)
% Another major reason of not searching the data was that the casual fans 
For example, \quot{how can I search [the data] if I do not even know how to describe my confusion?} (PX)
According to the casual fans,
perhaps the best way to seek information about game understanding was to \quot{ask my [experienced fan] friends.} (PX)
In summary, while the current live streams cannot provide enough information for casual fans to understand the game, casual fans prefer to \quot{let it [the confusions] go} rather
than to search the internet for the data, since the search process is annoying and the confusion is hard to describe.

% due to the annoyed, inconvenient searching process.
%% never search info in or after the game
%% bc
%% provide, overwhelming

\subsubsection{\textbf{Die-hard Fans' Suggestions for Understanding Live Basketball Games}}

\noindent
Since ''asking experienced friends'' was the preferred way to seek information by casual fans, we were particularly interested in what information die-hard fans suggest for understanding a live basketball game.
When interviewing die-hard fans, 
they did suggest a few critical insights to understand basketball games:

\paragraph{Being Aware of Ball Possessions.}
Basketball, from a certain perspective, is a turn-based game.
A basketball game consists of multiple possessions (i.e., turns), in which the team has possession of the ball is on offense and the other is on defense.
In each possession, the offensive team has 24 seconds (so-called \emph{shot clock}) to make a field goal.
After they make a field goal attempt or run out time,
the defensive team will get the possession of the ball and switch to be on the offense.
\cmo{Need Tica: How about rebounce? Correct me if I am incorrect}
Thus, a casual fan should be aware of the ball possession when watching basketball games, and follow the rhythm of transitioning between offense and defense.

\paragraph{Identifying Key Players.}
While basketball is a team sport, the importance of each player is different. 
In each possession, some \emph{``star'' players} have a higher chance to possess the ball and lead the offensive tactic since they are the core of the team.
\quot{The coach will develop tactics centered on the star.} (PX), and usually
there are several motifs between the five players in a team.
For example,
\quot{XXX frequently passes (XX\%) or receives (XX\%) the ball to and from XXX.}
\emph{Players with open spaces} are also critical to the offensive team as they have a higher chance to make the goal.
By identifying these key players, die-hard fans 
are able to watch the game more effectively and predicatively.
In addition to these key players,
we also discussed other key players on offense, such as those who play screens, and key defenders with the die-hard fans.
Overall they suggested not to help casual fans identify these key players, as their contributions to the possession outcome (e.g., a goal) are not explicit and focusing on these players can be overwhelming for casual fans.

\paragraph{Understanding Offensive and Defensive In-Game Decisions (\cmo{need a better term/title}).}
Knowing the offensive and defensive abilities of the players on the court is key to understanding their in-game decisions.
While basketball analysts have developed numerous metrics~\cite{} to evaluate players' performances for different purposes, die-hard fans suggested a couple of intuitive, easy-to-calculate metrics that can help casual fans understand the players' in-game decisions.
Specifically, for offensive players, we can present their \emph{location based expected point value}~\cite{},
which measures how many points a player can make at a specific location. \cmo{introduce how to calculate specifically?}
For defensive players, we can present their \emph{location based defense percentage points difference}~\cite{},
which measures how much the field goal percentage of a player in the offense is changing when being defended by the player in question.
%opposing player can change when the player is defending the opponent.
Both metrics can be calculated or directly obtained by using the data from the Official NBA Stats website~\cite{}.  
In addition, die-hard fans also suggested to visualize the one-on-one relationships between offensive and defensive players, as well as their distance, which can reveal interactions between offensive and defensive players and their tactics (e.g., defensive switching).

\subsection{Summary}
\cmo{a few sentence to summary}

Next, we introduce the two key components to enable \system{} -- the CV processing pipeline to embed visualizations into basketball videos (\autoref{sec:cv_pipeline})
and the gaze-moderated embedded visualizations (\autoref{sec:gaze_moderated_vis})
to facilitate game watching for casual fans.

==> tex/_deprecated/3-formative_v2.tex <==
\section{Formative Study with Basketball Fans}

To understand the practices, pain points, and requirements of casual fans in watching live basketball videos we conducted a formative study.

\subsection{Study Setup}

\paragraph{Participants.}
We recruited participants using university mailing lists and forums 
and used a pre-screening survey (\cmo{in supplemental material}) to select participants 
based on their fandom level, game watching frequency, and basketball knowledge. 
In total, we recruited 8 casual fans (P1-P8; M=3, F=5; Age: 18 - 35),
who only knew \quot{basic rules of basketball} and watched \quot{1 - 10 games per year}.
To better identify the pain points specific to casual fans, 
we further recruited 8 die-hard fans (P9 - P16; M=8; Age: 18 - 55), who knew \quot{basketball tactics and pros and cons of specific players} and watched \quot{at least 1 game per week}. No female die-hard fan responded to us.
All participants had normal vision or wore contact lenses or glasses to correct to normal vision.

{\renewcommand{\arraystretch}{1.3}% for the vertical padding
\begin{table}[h]
\begin{threeparttable}
    \centering
    \caption{Context information of the two game videos in the formative study.}
    \begin{tabular}{c c c c c c c c}
    % \toprule
     & \textbf{Date} & \textbf{Teams} & \textbf{Quarter} & \textbf{Scores} & \textbf{Game Clock (m:ss)} & \textbf{Video Duration (m:ss)} \\ \midrule
    %% -----
    \textbf{G1} & 2015.12.25 & GSW vs. CLE\tnote{*} & 4 & 67 : 71 & 7:00 & 9:02\\ \hline
    \textbf{G2} & 2015.12.22 & OKC vs. LAC\tnote{*} & 4 & 83 : 89 & 6:11 & 9:30\\
	\bottomrule
    \end{tabular}
    \label{tab:study1_games}
    %%% ---- 
	\begin{tablenotes}\footnotesize
    \item[*] GSW (Golden State Warriors), CLE (Cleveland Cavaliers), OKC (Oklahoma City Thunder), and LAC (Los Angeles Clippers)
    \end{tablenotes}
\end{threeparttable}
\end{table}
}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig_31_study_setup.pdf}
    \caption{a) Formative study setup. 
    b) In the review session, the participant's gaze is visualized in purple and overlaid on the video.}
    \label{fig:study_setup}
\end{figure}

\paragraph{Procedure.}
We started each session by introducing our research motivation and study protocol.
The experimenter then conducted a semi-structured interview with each participant, focusing on their current practices, pain points, and solutions to watching live basketball games.
Next, we followed the format of a \emph{contextual query}~\cite{hartson2012ux}
and asked participants to watch two regular-season NBA game videos(\autoref{tab:study1_games})
on a 24-inch monitor. %, each last for about 9 minutes.
These two games were rated as top-30 games of the season 
and have been watched millions of times.
Before watching the games, 
the experimenter asked participants to pretend to watch the game in a real-world scenario 
and encouraged them to think aloud as much as possible.
We collected think-aloud and gaze data during the game-watching process.
To collect the gaze data, we used Eyeware Beam~\cite{Eyeware},
a commercial software that leverages Apple's TrueDepth camera~\cite{TrueDepth}
to track the participant's head and gaze.
The participants sat approximately 60cm from the screen
and were asked to adjust their chair prior to watching the videos (\autoref{fig:study_setup}a).
The system was then calibrated and the participants
were allowed to move their head freely after the calibration.
We used a TrueDepth camera-based tracker as 
it provided sufficient accuracy~\cite{DBLP:conf/hci/GreinacherV20} 
for inspecting what video objects participants were looking at while watching the game, at a much lower budget than more proficient eye-trackers (e.g., Pupil Core~\footnote{https://pupil-labs.com/products/core}, > \$3K).
For more fine-grained gaze data (e.g., saccades, fixation), more proficient ey-trackers would be required.

After watching each game video,
we asked participants to re-watch the game with their gaze data overlaid (\autoref{fig:study_setup}b)
and to elaborate on any confusion, data needs, insights, and excitement they had felt when watching the game for the first time.
Participants could pause the video in the review session.
Each participant was compensated with a \$20 gift card for their time (1 hour).

\paragraph{Analysis.}
Interviews and think-alouds were audio-recorded, 
transcribed, 
and analyzed using a reflexive thematic analysis~\cite{}.
Three authors coded independently on the transcriptions to form sets of plausible codes
and iteratively refined the codes to converge on a single coding schema,
focusing on the difficulties participants experienced while watching the games.
Disagreements were resolved through discussions.
Moreover, three authors analyzed the gaze data by manually annotating
the video objects each participant was looking at while watching the games.
The categories of objects (\autoref{tab:study1_gaze} header) 
were generated both inductively (i.e., bottom-up, based on the data) 
and deductively (i.e., top-down, based on prior knowledge).
We classified participants as looking at an object only when their gaze
rested on the object for at least 0.25 seconds (fixation duration~\cite{}). 
The duration when the participant moved his/her gaze to the object
was also annotated as looking at the object.

% % {\renewcommand{\arraystretch}{1.2}% for the vertical padding
% \begin{table}[h]
%     \centering
%     % \vspace{-0.5mm}
%     \caption{The gaze distribution in seconds.}
%     \label{tab:study1_gaze}
%     % \vspace{-0.5em}
%     \begin{tabular}{c | c| c c c c c c c c c}
%     \toprule

%     \multicolumn{1}{c}{}  & \textbf{Fans} & \textbf{Player w/ ball} & \textbf{Player w/o ball} & \textbf{Referee} & \textbf{Basket} & \textbf{Score} & \textbf{Time} &\textbf{Ball} &\textbf{Others} &\textbf{Total}\\ \midrule
%     %% -----
%     \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{G1}}} & \textbf{Casual} & 254.39 & 141.10 & 4.74 & 27.32 & 23.65 & 9.98 & 3.66 & 75.55 & 540.39 \\ \cline{2-11} 
%      & \textbf{Die-hard} & 212.54 & 180.48 & 4.68 & 28.25 & 28.13 & 9.05 & 7.42 & 68.89 & 539.44\\ \hline
%     \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{G2}}} & \textbf{Casual}   & 221.63 & 115.41 & 4.80 & 30.01 & 37.54 & 14.33 & 2.78 & 134.36 & 560.86\\ \cline{2-11} 
%      & \textbf{Die-hard} & 199.70 & 144.38 & 4.80 & 23.52 & 27.74 & 8.53 & 4.49 & 149.32 & 562.48 
%  \\
% 	\bottomrule
% \end{tabular}
% \end{table}
% % }


\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_32_time_dist.pdf}
    \caption{The gaze distribution in seconds. TODO}
    \label{fig:gaze_dist}
\end{figure}

\subsection{Findings and Discussions}

%% Practices of Watching Live Basketball Games
All casual fans we interviewed
watched \quot{1 - 10 games per year}, mostly \quot{the important games, such as semi-finals or finals.} (P1-P8) 
Overall, they were not familiar with basketball games and the NBA, 
stating that they \quot{only knew the basic rules} of basketball
and \quot{the names of some superstars}, such as \quot{James} and \quot{Curry}. 
While they did not consider themselves fans of particular teams or players, some casual fans did support the team of their city (e.g., Boston Celtics); and one participant particularly felt connected to Stanley~\footnote{https://www.nba.com/player/1626169/stanley-johnson} since he was her high school's alumni. 
As for the game watching medium, 
all casual fans reported that they only watch live NBA games on TV,
usually with their die-hard fan friends at home or at bars.
In comparison, 
the die-hard fans we interviewed watched basketball games much more frequently, either with friends or alone. 
They had a rich knowledge about basketball (e.g., tactics), 
knew almost all NBA players, 
and even their strengths and shortcomings. 
TV was also the main way for die-hard fans to watch live basketball games.
Overall, for casual fans, watching live basketball games is a leisure activity, such as watching a movie or hiking, 
but it is a more serious hobby for die-hard fans. 

\subsubsection{\textbf{Casual Fans' Confusion in Watching Live Basketball Games}}

\noindent
In terms of the watching experience, 
all 16 participants confirmed that 
they were confused from time to time when watching basketball games 
and that they would like to seek extra information, other than the data provided by the scoreboard and commentaries.
Some confusion is common in both casual and die-hard fans, 
such as questions like \quot{who got a foul?} and \quot{which team called the timeout?}
These questions can usually be resolved easily by \quot{watching a replay of the game} (P5, P11) or simply by \quot{searching Google.} (P12)
However, we did identify some confusing aspects specific to casual fans 
that cannot be easily resolved by the current live streaming techniques, 
and which lead to a poor watching experience:

% \vspace{-4mm}
\paragraph{C1: Casual fans are unsure about which players they should focus on.}
\label{para:C1}
In a basketball game, 
the importance of players varies 
based on their skills, roles, and positions. 
% Focusing more on the key players can 
% \cmo{one more sentence to explain the necessity of focusing on key players?}
However, 
it is challenging for casual fans to identify the key players from the 10 moving players. 
Casual fans described that they did not understand the players' roles, 
the purpose of their movements, and their expected actions. 
Thus, casual fans often did not know whom to focus on when watching a game and felt that the players were just \quot{10 moving objects.} (P6)

The casual fans' inability to identify key players was also reflected in the participants' gaze patterns.
In our study, we found that casual fans spent more time on the player with the ball, 
while die-hard fans allocated more attention on other players (\autoref{fig:gaze_vis}). 
When we asked the reasons in the review session,
most of the casual fans explained that they focused on the player with the ball 
since they \quot{do not know who else to look at.} (P1)
As a result, 
casual fans often missed important off-ball movements and felt that the ball \quot{is magically passed to a player who is empty.} (P1) 
Moreover,
focusing on the player with the ball also indicated that casual fans generally pay more attention to the offensive team instead of the defensive one.
In some casual fans' gaze,
we noticed some rapid zigzag movement between the player with the ball and other players, 
revealing their attempts to watch other players without the ball.
P6, for example, explained that she was trying to look for the player to whom the ball would be passed to, 
while keeping an eye on the player with the ball.
However, she had to \quot{scan through the players one-by-one}
and felt such kind of scanning was \quot{exhausting} due to the heavy cognitive load.
On the other hand, 
die-hard fans scanned through the players much more effectively and predicatively, 
and often could directly identify the key player who, for example, would get the ball at the next pass. 

% explained that she was trying to look for the player whom the ball would be passed to but 
% Meanwhile, she was “worry about losing the ball.” 
% In our study, we observed several bahaviours that indicated poor watching experience due to the inability of identifying key players: 
% Since casual fans cannot identify other key players, 
% According to the gaze data, the casual fans spent X and X secs on the ballholder and others in average, while the die-hard fans spent X and X secs on each of them (Table. []). 

% Some casual fans (PX - X) attempted to inspect other players instead of only focusing on the ballholder. However, since they cannot efficiently identify the key players, they usually have to scan the players one-by-one, while keeping an eye on the ballholder, leading to a huge cognitive load. 
% In summary, since the casual fans cannot identify the key players, they either tended to focus more on the ballholder but failed to notice important off-ball movements, or attempted to inspect the off-ball movements but suffered from high cognitive loads.

\paragraph{C2: Casual fans are confused about the in-game decisions of players.}
\label{para:C2}
Even when casual fans focused on a specific player,
they usually could not understand the in-game decisions of the player. 
As a highly tactical and competitive sport, 
a basketball game includes numerous in-game decisions made by the players 
based on 
% the specific situation that involves 
situated factors such as the players’ abilities, positions, and shooting touches. 
However, these factors were mostly unknown or hard to interpret from the videos 
for casual fans, 
who only \quot{know the basic rules of basketball.}
Thus, casual fans could hardly understand the in-game decisions of the players.

Without understanding the in-game decisions of the players, 
casual fans could not appreciate and enjoy the game at the same deep level 
as die-hard fans 
and had difficulties to \quot{keep pace with other experienced spectators.} (P6)
This was also revealed in the study.
While we particularly encouraged participants to think aloud in the study,
most casual fans rarely provided meaningful comments when watching the two videos.
The most frequent verbal comments from casual fans were interjections, e.g., \quot{Oops}, \quot{Wooooow!}
Furthermore, 
even in the follow-up review session, casual fans could hardly describe their thoughts while watching the games.
As P3 acknowledged, 
she actually \quot{did not know what [she] was thinking of the game ... but just felt excited.}
By contrast, die-hard fans could clearly elaborate, comment on, and even suggest tactics of the players when watching the games. 
Generally speaking, 
our study suggests that
the casual fans' experience was closer to ``feeling'' the game
while the experience of die-hard fans was closer to ``reading'' the game.
% \cmo{should echo back to the confusion of in-game decision making.}

\paragraph{C3: Casual fans rarely resolve their confusion proactively.}
\label{para:C3}
Casual fans rarely seek extra information to proactively resolve their confusion, even if that results in a poor watching experience.
Casual fans agreed that the information provided by the live streams (e.g., commentaries, scoreboard)
is insufficient to resolve their confusion.
However, all casual fans we interviewed confirmed 
that they never search the internet to seek data while watching games.
The ``distracting'' context switching between the game 
and websites was a primary reason that made casual fans reluctant to search for extra data.
Specifically, casual fans thought that the game
\quot{is already overwhelming} and they could \quot{miss a lot when looking up a webpage} (P2-P5, P8).
On the other hand, 
die-hard fans noted that they frequently search third-party websites (e.g., ESPN) when watching basketball games,
though they also complained about the context switching between the game videos and another window, e.g., the mobile phone.
This finding revealed to us another main difference between casual fans and die-hard fans,
which is that casual fans \quot{did not know how to search} (P6).
For example, 
\quot{how can I search [the data] if I even do not know the player's name?} (P2, P5 - P7).
According to the casual fans,
perhaps the best way to seek information about game understanding was to \quot{ask my [experienced fan] friends} (P1-P8).
Some casual fans remarked that sometimes they tried to understand the game 
by listening to the cheering of the audience.
P2 said that \quot{at least I can know if the shot is a good one [from the background cheering].}
In summary, 
while the current live streams cannot provide enough information for casual fans to understand the game, 
casual fans prefer to \quot{let it [the confusions] go} rather
than to search the internet for the data, 
since the search process is 
distracting and overwhelming
and their confusion is sometimes hard to describe.

\subsubsection{\textbf{Die-hard Fans' Suggestions for Understanding Live Basketball Games}}

\noindent
Since ``asking experienced friends'' was the preferred way to seek information by casual fans, 
we were particularly interested in what information die-hard fans suggest for understanding a live basketball game.
When interviewing die-hard fans, 
they did suggest a few critical insights to understand basketball games:

% \paragraph{Being Aware of Ball Possessions.}
\paragraph{Following the Rhythm of Basketball Games.}
Basketball, from a certain perspective, is a turn-based game.
A basketball game consists of multiple possessions (i.e., turns), 
in which the team has possession of the ball is on offense, and the other team is on defense.
In each possession, 
the offensive team has 24 seconds (so-called \emph{shot clock}) to make a field goal in the NBA.
After they make a field goal, miss a shot and the rebound, or run out of time,
the defensive team will get possession of the ball 
and switch to be on the offense.
Being aware of the ball possession when watching basketball games
can help casual fans better follow
the rhythm of transitioning between offense and defense.

\paragraph{Identifying Key Offensive Players.}
While basketball is a team sport, 
the importance of each player, especially when he/she is on offense, is different.
For example, in each possession, 
some \emph{``star'' players} have a higher chance to possess the ball 
and lead the offensive tactic since they are the core of the team.
\quot{The coach will develop tactics centered on the stars} (P13)
and usually there are some passing patterns between the stars and other players in a team.
For example,
\quot{Westbrook [a star] frequently passes or receives the ball to and from Ibaka.} (P10)
\emph{Players with open spaces} are also critical to the offensive team as they have a higher chance of making the goal.
By identifying these key players, 
die-hard fans 
are able to watch the game more effectively and predictably.
In addition to the aforementioned key players,
we also discussed other players as helpers on offense, 
such as those who play screens, 
and key defenders with the die-hard fans.
Overall they suggested not to help casual fans identify other helpers and defenders, 
as their contributions to the possession outcome (e.g., a goal) are not explicit 
and thus can confuse casual fans.
% and focusing on these players can be overwhelming for casual fans.

\paragraph{Understanding In-game Decisions.}
Knowing the offensive and defensive performance of players is key to understanding their in-game decisions. \cmo{While die-hard fans usually rely on their extensive game-watching experience to evaluate players' decisions on the spot, casual fans have no such knowledge. Therefore, die-hard fans suggested using a subset of offensive and defensive metrics~\cite{} to help casual fans evaluate  the players' in-game decisions.}
% While basketball analysts have developed numerous metrics~\cite{} to evaluate players' performances for different purposes, the die-hard fans suggested a couple of simple but effective metrics that can help casual fans understand the players' in-game decisions.
Specifically, 
for offensive players, we can present their location-based \emph{expected point value} (EPV),
which measures how many points a player is expected to make if they shoot at a specific location. 
% \cmo{introduce how to calculate specifically?}
For defensive players, 
we can present their location-based \emph{percentage points difference} (DIFF\%),
which measures how much the field goal percentage of a player on the offense is changing when being defended by the player in question.
Both metrics can be calculated or directly obtained by using the data from the Official NBA Stats website~\cite{nbastats}.  
In addition, die-hard fans also suggested to visualize the one-on-one relationships between offensive and defensive players, as well as their distance, 
which can reveal interactions between offensive and defensive players and their tactics (e.g., defensive switching).

\subsection{Summary}
In summary,
the casual fans confirmed that they were often confused about the key players and their in-game decisions,
but rarely sought data proactively to resolve their confusion 
since their confusion is sometimes hard to describe
and the search process is distracting.
\cmo{
To help casual fans better understand the game, die-hard fans suggested a few critical insights in
following the rhythm of basketball games, 
identifying key players, 
and understanding players' in-game decisions.}
Informed by these findings,
we designed and implemented \system{}
to improve casual fans' understanding and engagement in watching live basketball videos.
Next, we introduce the two key 
components to enable \system{} -- 
a CV processing pipeline 
to embed visualizations into basketball videos (\autoref{sec:cv_pipeline})
and a set of gaze-moderated embedded visualizations to seamlessly present extra in-game data (\autoref{sec:gaze_moderated_vis}).

==> tex/_deprecated/3-formative_v3.tex <==
\section{Formative Study with Basketball Fans}

To understand the practices, pain points, and requirements of casual fans in watching live basketball videos,
we conducted a formative study.

% that compared the game-watching behaviors between 8 casual and 8 die-hard fans
% in a formative study.

\subsection{Study Setup}

\paragraph{Participants.}
We recruited participants using university mailing lists and forums 
and used a pre-screening survey to select participants 
based on their fandom level, game watching frequency, and basketball knowledge. 
In total, we recruited 8 casual fans (P1-P8; M=3, F=5; Age: 18 - 35),
who only knew \quot{basic rules of basketball} and watched \quot{1 - 10 games per year}.
To better identify the pain points specific to casual fans, 
we further recruited 8 die-hard fans (P9 - P16; M=8; Age: 18 - 55), 
who knew \quot{basketball tactics and pros and cons of specific players} 
and watched \quot{at least 1 game per week}. No female die-hard fan responded to us.
All participants had normal vision or wore contact lenses or glasses to correct to normal vision.

{\renewcommand{\arraystretch}{1.3}% for the vertical padding
\begin{table}[h]
\begin{threeparttable}
    \centering
    \caption{Context information of the two game videos in the formative study.}
    \begin{tabular}{c c c c c c c c}
    % \toprule
     & \textbf{Date} & \textbf{Teams} & \textbf{Quarter} & \textbf{Scores} & \textbf{Game Clock (m:ss)} & \textbf{Video Duration (m:ss)} \\ \midrule
    %% -----
    \textbf{G1} & 2015.12.25 & GSW vs. CLE\tnote{*} & 4 & 67 : 71 & 7:00 & 9:02\\ \hline
    \textbf{G2} & 2015.12.22 & OKC vs. LAC\tnote{*} & 4 & 83 : 89 & 6:11 & 9:30\\
	\bottomrule
    \end{tabular}
    \label{tab:study1_games}
    %%% ---- 
	\begin{tablenotes}\footnotesize
    \item[*] GSW (Golden State Warriors), CLE (Cleveland Cavaliers), OKC (Oklahoma City Thunder), and LAC (Los Angeles Clippers)
    \end{tablenotes}
\end{threeparttable}
\end{table}
}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig_31_study_setup.pdf}
    \caption{a) Formative study setup. 
    b) In the review phase, the participant's gaze is visualized in purple and overlaid on the video.}
    \label{fig:study_setup}
\end{figure}

\paragraph{Procedure.}
We started each session 
by introducing our research motivation and study protocol.
The experimenter then conducted a semi-structured interview with each participant, 
focusing on their current practices, pain points, and solutions in watching live basketball games.
Next, we followed the format of \emph{contextual query}~\cite{hartson2012ux}
to asked participants to watch two regular-season NBA game videos(\autoref{tab:study1_games})
on a 24-inch monitor.
These two games were rated as top-30 games of the season 
and have been watched millions of times.
% Before watching the games, 
% the experimenter asked participants to pretend to watch the game in a real-world scenario 
% and encouraged them to think aloud as much as possible.
We collected think-aloud and gaze data during the game-watching process.
To collect the gaze data, we used Eyeware Beam~\cite{Eyeware},
a commercial software that leverages Apple's TrueDepth camera~\cite{TrueDepth}
to track the participant's head and gaze.
The participants sat approximately 60cm from the screen
and were asked to adjust their chair prior to watching the videos (\autoref{fig:study_setup}a).
The system was then calibrated and the participants
were allowed to move their head freely after the calibration.
We used a TrueDepth camera-based tracker as 
it provided sufficient accuracy~\cite{DBLP:conf/hci/GreinacherV20} 
for inspecting what video objects participants were looking at while watching the game, 
at a much lower budget than more proficient eye-trackers (e.g., Pupil Core~\footnote{https://pupil-labs.com/products/core}, > \$3K).
For more fine-grained gaze data (e.g., saccades, fixation), more proficient eye-trackers would be required.

After watching each game video,
we asked participants to re-watch the game with their gaze data overlaid (\autoref{fig:study_setup}b)
and to elaborate on any confusion, data needs, insights, and excitement they had felt when watching the game for the first time.
Participants could pause the video in the review phase.
Each participant was compensated with a \$20 gift card for their time (1 hour).

\paragraph{Analysis.}
Interviews and think-alouds were audio-recorded, 
transcribed, 
and analyzed using a reflexive thematic analysis~\cite{reflexiveTA}.
Three authors coded independently on the transcriptions to form sets of plausible codes
and iteratively refined the codes to converge on a single coding schema,
focusing on the difficulties participants experienced while watching the games.
Disagreements were resolved through discussions.
Besides, three authors analyzed the gaze data by manually annotating
the video objects each participant was looking at while watching the games.
The categories of objects (\autoref{fig:gaze_dist} x-axis)
were generated both inductively (i.e., based on the data) 
and deductively (i.e., based on prior knowledge).
We classified participants as looking at an object only when their gaze
rested on the object for at least 0.25 seconds (fixation duration~\cite{}). 
The duration when the participant moved her/his gaze to the object
was also annotated as looking at the object.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_32_time_dist.pdf}
    \caption{The gaze distribution in seconds shows that, compared to die-hard fans, casual fans spent more time on watching the player with ball in both games. Due to the small sample size, we discuss these results with a descriptive approach and focus more on other behavioral observations.}
    \label{fig:gaze_dist}
\end{figure}

\subsection{Findings and Discussions}

%% Practices of Watching Live Basketball Games
All casual fans we interviewed
only watched \quot{the important games, such as semi-finals or finals.} (P1-P8) 
Overall, they were not familiar with basketball and the NBA, 
stating that they only knew \quot{the basic rules} of basketball
and \quot{the names of some superstars}, such as \quot{James} and \quot{Curry}. 
While they did not consider themselves fans of particular teams or players, 
some casual fans did support the team of their city (e.g., Boston Celtics); 
and one participant particularly felt connected to Stanley~\footnote{https://www.nba.com/player/1626169/stanley-johnson} since he was her high school's alumni. 
As for the game watching medium, 
all casual fans reported that they only watch live NBA games on TV.
% usually with their die-hard fan friends at home or at bars.
In comparison, 
the die-hard fans we interviewed watched basketball games much more frequently.
% either with friends or alone. 
They had a rich knowledge about basketball (e.g., tactics), 
knew almost all NBA players, 
and even their strengths and shortcomings. 
TV was also the main way for die-hard fans to watch live basketball games.
Overall, for casual fans, watching live basketball games is a leisure activity, such as watching a movie or hiking, 
but it is a more serious hobby for die-hard fans. 

\subsubsection{\textbf{Casual Fans' Confusion in Watching Live Basketball Games}}

\noindent
In terms of the watching experience, 
all 16 participants confirmed that 
they were confused from time to time when watching basketball games 
and that they would like to seek extra information, other than the data provided by the scoreboard and commentaries.
Some confusion is common in both casual and die-hard fans, 
such as questions like \quot{who got a foul?} and \quot{which team called the timeout?}
These questions can usually be resolved by \quot{watching a replay of the game} (P5, P11) 
or simply by \quot{searching Google.} (P12)
However, 
we did identify some confusing aspects specific to casual fans 
that cannot be easily resolved by the current livestreams %,techniques, 
and thus lead to a poor watching experience:

\paragraph{C1: Casual fans are unsure about which players they should focus on.}
\label{para:C1}
In a basketball game, 
the importance of players varies 
based on their skills, roles, and positions. 
Without knowing these details,
the casual fans often could not identify the important players
and felt that the players were just \quot{10 moving objects.} (P6)
The casual fans' inability to identify key players was also reflected in the their gaze patterns.
In our study, we found that casual fans spent more time on the player with the ball than the die-hard fans (\autoref{fig:gaze_dist}).
This was because 
the casual fans \quot{do not know who else to look at} (P1)
when watching the game.
As a result, 
casual fans often missed important off-ball movements 
and felt that the ball \quot{is magically passed to a player who is open.} (P1) 
Moreover,
focusing on the player with the ball also indicated that 
casual fans generally pay more attention to the offensive team than the defensive one.
In some casual fans' gaze,
we noticed some rapid zigzag movement between the player with the ball and other players, 
revealing their attempts to watch other players without the ball.
P6, for example, explained that she was 
\quot{scan[ning] through the players one-by-one}
to predict the ball receiver at the next pass,
while keeping an eye on the player with the ball.
However, she felt such kind of scanning was \quot{exhausting} due to the heavy cognitive load.
On the other hand, 
die-hard fans scanned through the players much more effectively and predicatively, 
and often could directly identify the key player who, for example, would receive the ball.

\paragraph{C2: Casual fans are confused about the in-game decisions of players.}
\label{para:C2}
As a highly tactical and competitive sport, 
a basketball game includes numerous in-game decisions made by the players 
based on 
situated factors such as the players’ abilities, positions, and shooting touches. 
However, these factors were mostly unknown or hard to interpret from the videos 
for casual fans.
Thus, the casual fans could hardly understand the in-game decisions of the players.
% Without understanding the in-game decisions of the players, 
Consequently,
the casual fans could not appreciate and enjoy the game at the same deep level as die-hard fans 
and had difficulties to \quot{keep pace with other [experienced] friends.} (P6)
This was also revealed in the study.
While we particularly encouraged participants to think aloud in the study,
most casual fans rarely provided meaningful comments when watching the two videos.
The most frequent verbal comments from casual fans were interjections, e.g., \quot{Oops}, \quot{Wooooow!}
Furthermore, 
even in the follow-up review session, casual fans could hardly describe their thoughts while watching the games.
As P3 acknowledged, 
she actually \quot{did not know what [she] was thinking of the game ... but just felt excited.}
By contrast, die-hard fans could clearly elaborate, comment on, and even suggest tactics of the players when watching the games. 
Generally speaking, 
our study suggests that
the casual fans' experience was closer to ``feeling'' the game
while the experience of die-hard fans was closer to ``reading'' the game.
% \cmo{should echo back to the confusion of in-game decision making.}

\paragraph{C3: Casual fans rarely seek information proactively to resolve their confusion,}
\label{para:C3}
even if that results in a poor watching experience.
The casual fans agreed that the information provided by the livestreams (e.g., commentaries, scoreboard)
is insufficient to resolve their confusion.
However, 
all of them never searched the internet to seek data while watching games,
since the game \quot{is already overwhelming} and they could \quot{miss a lot when looking up webpages} (P2-P5, P8).
On the other hand, 
die-hard fans noted that they would search websites (e.g., ESPN) when watching basketball games,
though they also complained about the context switching between the game videos and another windows, e.g., the mobile phone.
This finding revealed to us another main difference between casual fans and die-hard fans,
which is that casual fans \quot{did not know how to search} (P6).
For example, 
\quot{how can I search [the data] if I even do not know the player's name?} (P2, P5 - P7).
According to the casual fans,
perhaps the best way to seek information about game understanding was to \quot{ask my [experienced] friends} (P1-P8).
In summary, if the casual fans could not ask their experienced friends for help,
they would just \quot{let it [the confusions] go}.

\subsubsection{\textbf{Die-hard Fans' Suggestions for Understanding Live Basketball Games}}

\noindent
Since ``asking experienced friends'' was the preferred way to seek information by casual fans, 
we were particularly interested in what information die-hard fans suggest for understanding a live basketball game.
When interviewing die-hard fans, 
they did suggest a few critical insights to this end:

% \paragraph{Being Aware of Ball Possessions.}
\paragraph{Following the Rhythm of Basketball Games.}
Basketball, from a certain perspective, is a turn-based game.
A basketball game consists of multiple possessions (i.e., turns), 
in which the team has possession of the ball is on offense, and the other team is on defense.
In each possession, 
the offensive team has 24 seconds (so-called \emph{shot clock}) to make a field goal in the NBA.
After they make a field goal, miss a shot and the rebound, or run out of time,
the defensive team will get possession of the ball 
and switch to be on the offense.
Being aware of the ball possession when watching basketball games
can help casual fans better follow
the rhythm of transitioning between offense and defense.

\paragraph{Identifying Key Players.}
While basketball is a team sport, 
the importance of each player, especially when she/he is on offense, is different.
Generally speaking, 
on the offensive side,
\emph{the player with the ball}
and \emph{the ball receiver} at the next pass are the most important ones.
% \cmo{need one sentence about how to predict the ball receiver}
% For example, in each possession, 
% some \emph{``star''} players are the core of the team 
% and thus have a higher chance to possess the ball 
% and lead the offensive tactic.
% \quot{The coach will develop tactics centered on the stars} (P13)
% and usually there are some passing patterns between the stars and other players in a team.
% For example,
% \quot{Westbrook [a star] frequently passes or receives the ball to and from Ibaka.} (P10)
\emph{Players with open spaces} are also critical to the offensive team as they have a higher chance of making the goal.
On the defensive side,
all the defenders who are guarding the player with the ball are important.
By identifying these key players, 
die-hard fans 
are able to watch the game more effectively and predictably.
In addition to the aforementioned key players,
we also discussed other players,
such as offensive helpers who play screens,
with the die-hard fans.
Overall they suggested not to help casual fans identify other players, 
as their contributions to the possession outcome (e.g., a goal) are not explicit 
and thus can confuse casual fans.

\paragraph{Understanding In-game Decisions.}
Knowing the offensive and defensive abilities of players is key to understanding their in-game decisions. 
The die-hard fans suggested a subset of offensive and defensive metrics~\cite{}
to help casual fans understand the players' abilities.
Specifically, 
for offensive players, we can present their location-based \emph{expected point value},
which measures how many points a player is expected to make if they shoot at a specific location. 
For defensive players, 
we can present their location-based \emph{percentage points difference},
which measures how much the field goal percentage of a player on the offense is changing when being defended by the player in question.
Both metrics can be calculated or directly obtained by using the data from the Official NBA Stats website~\cite{nbastats}.  
In addition, die-hard fans also suggested to visualize the one-on-one relationships 
between offensive and defensive players, 
as well as their distance, 
which can reveal interactions between the players and their tactics (e.g., defensive switching).

\subsection{Summary}
In summary,
the casual fans were often confused about the key players and their in-game decisions,
but rarely sought data proactively to resolve their confusion 
since their confusion is sometimes hard to describe
and the search process is distracting.
To help casual fans better understand the game, 
die-hard fans suggested a few critical insights in
following the rhythm of basketball games, 
identifying key players, 
and understanding players' in-game decisions.
Informed by these findings,
we designed and implemented \system{}
to improve casual fans' understanding and engagement in watching live basketball videos.
Next, we introduce the two key 
modules to enable \system{} -- 
a CV processing pipeline 
to embed visualizations into basketball videos (\autoref{sec:cv_pipeline})
and a set of gaze-moderated embedded visualizations to seamlessly present extra in-game data (\autoref{sec:gaze_moderated_vis}).

==> tex/_deprecated/3-formative_v4.tex <==
\section{Formative Study with Basketball Fans}

To understand the practices, pain points, and solutions of casual fans in watching basketball videos,
we conducted a formative study.

% that compared the game-watching behaviors between 8 casual and 8 die-hard fans
% in a formative study.

\subsection{Study Setup}

\subsubsection{\textbf{Participants}}
\noindent
We recruited participants using university mailing lists and forums 
and pre-screened participants 
based on their fandom level, game-watching frequency, and basketball knowledge. 
In total, we recruited 
8 casual fans (P1-P8; M=3, F=5; Age: 18 - 35),
who only knew \quot{basic rules of basketball} 
and watched \quot{1 - 10 games per year}.
To better identify the pain points specific to casual fans, 
we further recruited 8 die-hard fans (P9 - P16; M=8; Age: 18 - 55), 
who knew \quot{basketball tactics and pros and cons of specific players} 
and watched \quot{at least 1 game per week}. No female die-hard fan responded to us.
All participants had normal vision or wore contact lenses or glasses to correct to normal vision.

{\renewcommand{\arraystretch}{1.3}% for the vertical padding
\begin{table}[h]
\begin{threeparttable}
    \centering
    \caption{Context information of the two game videos in the formative study.}
    \begin{tabular}{c c c c c c c c}
    % \toprule
     & \textbf{Date} & \textbf{Teams} & \textbf{Quarter} & \textbf{Scores} & \textbf{Game Clock (m:ss)} & \textbf{Video Duration (m:ss)} \\ \midrule
    %% -----
    \textbf{G1} & 2015.12.25 & GSW vs. CLE\tnote{*} & 4 & 67 : 71 & 7:00 & 9:02\\ \hline
    \textbf{G2} & 2015.12.22 & OKC vs. LAC\tnote{*} & 4 & 83 : 89 & 6:11 & 9:30\\
	\bottomrule
    \end{tabular}
    \label{tab:study1_games}
    %%% ---- 
	\begin{tablenotes}\footnotesize
    \item[*] GSW (Golden State Warriors), CLE (Cleveland Cavaliers), OKC (Oklahoma City Thunder), and LAC (Los Angeles Clippers)
    \end{tablenotes}
\end{threeparttable}
\end{table}
}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig_31_study_setup.pdf}
    \caption{a) Formative study setup. 
    b) In the review phase, the participant's gaze is visualized in purple and overlaid on the video.}
    \label{fig:study_setup}
\end{figure}

\subsubsection{\textbf{Procedure}}
\noindent
We started each session 
by introducing our research motivation and study protocol.
The experimenter then conducted a semi-structured interview with each participant, 
focusing on their current practices, pain points, and solutions when watching live basketball games.
Next, we followed the format of \emph{contextual query}~\cite{hartson2012ux}
to ask participants to watch two videos (\autoref{tab:study1_games})
on a 24-inch monitor.
These two games were rated as top-30 games of the season 
and have been watched millions of times.
We collected think-aloud and gaze data during the game-watching process.
To collect the gaze data, we used Eyeware Beam~\cite{Eyeware},
a commercial software that leverages Apple's TrueDepth camera~\cite{TrueDepth}
to track the participant's head and gaze.
The participants sat approximately 60cm from the screen
and were asked to adjust the chair before watching the videos (\autoref{fig:study_setup}a).
The system was then calibrated and the participants
were allowed to move the head freely after the calibration.
We used a TrueDepth camera-based tracker as 
it provided sufficient accuracy~\cite{DBLP:conf/hci/GreinacherV20} 
for inspecting what video objects participants were looking at while watching the game, 
at a much lower budget.
% than more proficient eye-trackers (e.g., Pupil Core~\footnote{https://pupil-labs.com/products/core}, > \$3K).
For more fine-grained gaze data (e.g., saccades, fixation), more proficient eye-tracker would be required.

After watching each game video,
we asked participants to re-watch the game with their gaze data overlaid (\autoref{fig:study_setup}b)
and to elaborate on any confusion, data needs, insights, and excitement they had felt when watching the game for the first time.
Participants could pause the video in the review phase.
Each participant was compensated with a \$20 gift card for their time (1 hour).

\subsubsection{\textbf{Analysis}}
\noindent
Interviews and think-alouds were audio-recorded, 
transcribed, 
and analyzed using a reflexive thematic analysis~\cite{reflexiveTA}.
Three authors coded independently on the transcriptions to form sets of plausible codes
and iteratively refined the codes to converge on a single coding schema.
% focusing on the difficulties participants experienced while watching the games.
% Disagreements were resolved through discussions.
Besides, three authors analyzed the gaze data by manually annotating
the video objects each participant was looking at while watching the games.
The categories of objects (\autoref{fig:gaze_dist} x-axis)
were generated based on the data and prior knowledge.
We classified participants as looking at an object only when their gaze
rested on the object for at least 0.25 seconds (fixation duration~\cite{DBLP:conf/ozchi/PenkarLW12}). 
The duration when the gaze was moving to the object
was also annotated as looking at the object.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_32_time_dist.pdf}
    \caption{The gaze distribution in seconds shows that, compared to die-hard fans, casual fans spent more time watching the player with the ball in both games. Due to the small sample size, we discuss these results with a descriptive approach and focus more on other behavioral observations.}
    \label{fig:gaze_dist}
\end{figure}

\subsection{Findings and Discussions}

%% Practices of Watching Live Basketball Games
All the casual fans
only watched \quot{important games, such as semi-finals or finals.} (P1-P8)
They were neither familiar with basketball nor the NBA.
% stating that they only knew \quot{the basic rules} of basketball
% and \quot{the names of some superstars}, such as \quot{James} and \quot{Curry}. 
% While they did not consider themselves fans of particular teams or players, 
% some casual fans did support the team of their city (e.g., Boston Celtics).
% and one participant particularly felt connected to Stanley~\footnote{https://www.nba.com/player/1626169/stanley-johnson} since he was her high school's alumni. 
% As for the game watching medium, 
% All casual fans reported that they only watch live NBA games on TV.
% usually with their die-hard fan friends at home or at bars.
In comparison, 
the die-hard fans watched basketball games much more frequently.
They had a rich knowledge about basketball (e.g., tactics), 
knowing almost all NBA players and even their strengths and shortcomings. 
TV was the main way for both casual and die-hard fans to watch live basketball games.
Overall, for casual fans, 
watching live basketball games is a leisure activity, such as hiking, 
but it is a more serious hobby for die-hard fans. 

\subsubsection{\textbf{Casual Fans' Confusion in Watching Basketball Games}}

\noindent
In terms of the watching experience, 
all 16 participants confirmed that 
they were confused from time to time when watching basketball games
and that they would like to seek extra information, other than the data provided by the scoreboard and commentaries.
Some confusion is common among both casual and die-hard fans, 
such as questions like \quot{who got a foul?} and \quot{which team called the timeout?}
These questions can usually be resolved by \quot{watching the replay} (P5, P11) 
or simply by \quot{searching Google.} (P12)
However, 
we did identify some confusing aspects specific to casual fans 
that cannot be easily resolved by the current live streams %,techniques, 
and thus lead to a poor watching experience:

\paragraph{C1: Casual fans are unsure about which players they should focus on.}
\label{para:C1}
When watching basketball games,
the casual fans often could not identify the important players
and felt that the players were just \quot{10 moving objects.} (P6)
The casual fans' inability to identify key players was also reflected in their gaze patterns.
In our study, 
we found that casual fans spent more time on the player with the ball than the die-hard fans (\autoref{fig:gaze_dist}),
since they
\quot{do not know who else to look at} (P1)
when watching the game.
As a result, 
casual fans often missed important off-ball movements 
and felt that the ball \quot{is magically passed to a player who is open.} (P1)
Moreover,
% focusing on the player with the ball also indicated that 
% casual fans generally pay more attention to the offensive team than the defensive one.
% Finally, 
in some casual fans' gaze,
we noticed some rapid zigzag movement between the player with the ball and other players, 
revealing their attempts to scan through the players.
% watch other players without the ball.
P6, for example, explained that she was 
\quot{scan[ning] through the players}
to predict the ball receiver at the next pass
while keeping an eye on the player with the ball,
leading to a heavy cognitive load.
% However, she felt such kind of scanning was \quot{exhausting} due to the heavy cognitive load.
In contrast,
die-hard fans scanned through the players much more effectively and predicatively, 
and often could directly identify the key player who, for example, would receive the ball.

\paragraph{C2: Casual fans are confused about the in-game decisions of players.}
\label{para:C2}
The casual fans could hardly understand the in-game decisions 
made by the players,
since 
the situated factors (e.g., players’ abilities, positions, and shooting touches)
behind these decisions
were mostly unknown or hard to interpret from the videos 
for casual fans.
Consequently,
the casual fans could not appreciate the game at the same deep level as die-hard fans 
and had difficulties \quot{keeping pace with other [experienced] friends.} (P6)
This was also revealed in the think-aloud data of the participants.
When watching the two videos,
the most frequent verbal comments from the casual fans were interjections, e.g., \quot{Oops}, \quot{Wooooow!}
Even in the follow-up review session, 
casual fans could hardly describe their thoughts while watching the games.
P3 acknowledged that 
she actually \quot{did not know what [she] was thinking of the game ... but just felt excited.}
By contrast, die-hard fans could clearly elaborate, comment on, and even suggest tactics of the players when watching the games. 
Generally speaking, 
our study suggests that
the casual fans' experience was closer to ``feeling'' the game
while the experience of die-hard fans was closer to ``reading'' the game.

% \paragraph{C3: Casual fans rarely seek information proactively to resolve their confusion.}
\paragraph{\cmo{C3: Casual fans have trouble seeking customized information to resolve their confusion.}}
\label{para:C3}
% even if that results in a poor watching experience.
% The casual fans agreed that the information provided by the livestreams (e.g., commentaries, scoreboard)
% is insufficient to resolve their confusion.
% However, 
All the casual fans never searched the internet to seek data to resolve their confusion
since the game \quot{is already overwhelming} and they could \quot{miss a lot when looking up webpages.} (P2-P5, P8)
Differently, 
the die-hard fans would search websites (e.g., ESPN) when watching basketball games,
though they also complained about the context switching between the game videos and other windows, e.g., the mobile phone.
This finding revealed to us another main difference between casual fans and die-hard fans,
which is that casual fans \quot{did not know how to search.} (P6)
For example, 
\quot{how can I search [the data] if I even do not know the player's name?} (P2, P5 - P7)
According to the casual fans,
perhaps the best way to seek information about game understanding was to \quot{ask my [experienced] friends.} (P1-P8)
In summary, if the casual fans could not ask their experienced friends for help,
they would just \quot{let it [the confusions] go.}

\subsubsection{\textbf{Die-hard Fans' Suggestions for Understanding Basketball Games}}

\noindent
Since casual fans preferred to \quot{ask experienced friends} to seek information, 
we were interested in what information die-hard fans suggest for understanding a live basketball game.
In the interview,
% When interviewing the die-hard fans, 
they did suggest a few critical insights:

% \paragraph{Being Aware of Ball Possessions.}
% \paragraph{Following the Rhythm of Basketball Games.}
\paragraph{\cmo{Distinguishing between offense and defense.}}
Basketball, from a certain perspective, is a turn-based game.
A basketball game consists of multiple possessions (i.e., turns), 
in which the team has possession of the ball is on offense, and the other team is on defense.
\cmo{
A player can have completely different roles, tactics, and behaviors between offense and defense.
Being aware of players' offense and defense status 
can help casual fans better understand and follow the game.
}
% In each possession, 
% the offensive team has 24 seconds (so-called \emph{shot clock}) to make a field goal in the NBA.
% After they make a field goal, miss a shot and the rebound, or run out of time,
% the defensive team will get possession of the ball 
% and switch to be on the offense.
% ball possession 
% when watching basketball games
% follow the rhythm of transitioning between offense and defense.

\paragraph{Identifying Key Players.}
While basketball is a team sport, 
the importance of each player, especially when she/he is on offense, is different.
Generally speaking, 
on the offensive side,
\emph{the player with the ball}
and \emph{the ball receiver} at the next pass are the most important ones.
\emph{Players with open spaces} are also critical to the offensive team as they have a higher chance of making the goal.
On the defensive side,
all the defenders who are guarding the player with the ball are important.
By identifying these key players, 
die-hard fans 
can watch the game more effectively and predictably.
In addition to the aforementioned key players,
we also discussed other players with the die-hard fans,
such as offensive helpers who play screens.
Overall, they suggested not to help casual fans identify these players, 
as their contributions to the possession outcome (e.g., a goal) are not explicit 
and thus can confuse casual fans.

\paragraph{Understanding In-game Decisions.}
Knowing the offensive and defensive abilities of players is key to understanding their in-game decisions. 
The die-hard fans suggested two metrics
to help casual fans understand the players' abilities.
For offensive players, we can present their location-based \emph{expected point value},
which measures how many points a player is expected to make if they shoot at a specific location. 
For defensive players, 
we can present their location-based \emph{percentage points difference},
which measures how much the field goal percentage of a player on the offense is changing when being defended by the player in question.
Both metrics can be calculated or directly obtained by using the data from the Official NBA Stats website~\cite{nbastats}.  
In addition, die-hard fans also suggested visualizing the one-on-one relationships 
between offensive and defensive players, 
as well as their distance, 
which can reveal interactions between the players and their tactics (e.g., defensive switching).

\subsection{Summary}

{\renewcommand{\arraystretch}{1.3}% for the vertical padding
\begin{table}[h]
\small
% \begin{threeparttable}
    \centering
    \caption{Sfawerqwerqwe.}
    \begin{tabular}{p{0.27\linewidth} p{0.32\linewidth} p{0.33\linewidth}}
    \toprule
      \cmo{\normalsize\textbf{Confusion}}  & \cmo{\normalsize\textbf{Takeaways}} & \cmo{\normalsize\textbf{Design Solutions}}  \\ \midrule
    %% -----
    \cmo{\emph{C1}: Casual fans are unsure about which players they should focus on.} & \cmo{\emph{T1}: Casual fans need help identifying important offensive and defensive players.} & \cmo{Visualizing players' importances based on their offensive and defensive status. (\autoref{sec:direct_att})} \\ \hline
    \cmo{\emph{C2}: Casual fans are confused about the in-game decisions of players.} & \cmo{\emph{T2}: Casual fans need help understanding a player’s offensive and defensive abilities.} & \cmo{Visualizing players' offensive and defensive abilities. (\autoref{sec:gaze_int})} \\ \hline
    \emph{C3}: & 2015.12.22 & OKC vs. LAC \\
	\bottomrule
    \end{tabular}
    \label{tab:findings}
    %%% ---- 
% 	\begin{tablenotes}\footnotesize
%     \item[*] GSW (Golden State Warriors), CLE (Cleveland Cavaliers), OKC (Oklahoma City Thunder), and LAC (Los Angeles Clippers)
%     \end{tablenotes}
% \end{threeparttable}
\end{table}
}

\noindent
In summary,
the casual fans were often confused about the key players and their in-game decisions,
but rarely sought data proactively to resolve their confusion 
since their confusion is sometimes hard to describe
and the search process is distracting.
To help casual fans better understand the game, 
die-hard fans suggested a few critical insights, including
following the rhythm of basketball games, 
identifying key players, 
and understanding players' in-game decisions.
Informed by these findings,
we designed and implemented \system{}.
% to improve casual fans' understanding and engagement in watching live basketball videos.
Next, we introduce the two key 
modules to enable \system{} -- 
a CV processing pipeline 
% to embed visualizations into basketball videos 
(\autoref{sec:cv_pipeline})
and a set of gaze-moderated embedded visualizations 
% to seamlessly present extra in-game data 
(\autoref{sec:gaze_moderated_vis}).

==> tex/_deprecated/4-cv_pipeline_v1.tex <==
\section{A CV Pipeline for Embedding Visualizations into Basketball Videos}
\label{sec:cv_pipeline}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.1\textwidth]{figs/fig_41_cv_pipeline.pdf}
    \caption{Our CV pipeline takes a raw video as the input, 
    outputs the bounding box, identity, and keypoints of each player, 
    and separates the image frame into foreground (humans) and background (all others). 
    The outputs of players are used to create visualizations,
    which are then composited with the foreground and background to form the augmented video.}
    \label{fig:cv_pipeline}
\end{figure}

\noindent
Based on the findings in our formative study,
we aim to present extra data about players in basketball videos through embedded visualizations.
To embed visualizations to the players,
we need to recognize the players (e.g., bounding box, identity, and keypoints)
and segment them from the background if the visualizations are rendered on the court.
To this end,
we design a CV processing pipeline
that is possible to run in real live streaming scenarios.
% using state-of-the-art techniques, 
% which can process video streams in real time with a constant buffer time of less than one minute. 

\subsection{Recognizing the Players}
To visualize data, e.g., the name, of a player in the video, 
one must know 
the 2D position (bounding box) of the specific player (identity) in each video frame.
Besides, one may also need the keypoints of the player for properly placing the visualization.
For each player,
% Given a raw video frame,
we obtain these results 
% of each player 
via three steps:
1) detecting his/her bounding box,
2) tracking his/her identity across frames,
and 3) estimating his/her keypoints.

% The purpose of the player tracking module is to determine the identities of the players and their 2D positions in each frame of a sport video in real time, 
% using only a raw footage as input. 
% For each frame, the module should output a list of tuples, one for each player and containing the player's bounding box, globally unique player ID, and keypoints. 
% We accomplish this goal using a three-step pipeline, which we will describe below.

The goal of this stage is to track players across frames in order to better infer the identity of the players in the current frame. 
% \paragraph{Object Detection and Classification}
\paragraph{Detecting the Players' Bounding Box}
% \cmo{talk about object detection first, the goal of object detection is to obtain bounding box of human. we use YoloX to achieve this.}
% \cmo{since YoloX cannot distinguish player and audience, we train a classifier to filter out audiences.}
The first step of the player tracking module is to detect the bounding boxes of all players on the court. 
This is a human-only object detection task, and we achieve this using a YoloX model trained on CrowdHuman, MOT17, Cityperson and ETHZ (pretrained weights come from ByteTrack authors). 
However, this model it self does not distinguish players from non-players such as referees. 
To improve the downstream accuracy of MOT, 
we use the vision transformer as backbone to train a player classifier that can detect the identity of the players (with one class for non-players), 
then use it to filter the bounding box detections of YoloX to minimize the number of candidates when matching. 

\paragraph{Multi-Object Tracking and Interpolation}
\cmo{The goal of MOT is to obtain the ids of each player across different frames.}
To track players across frames, we initialize a multi-object tracking task using ByteTrack with FastREID at the start of the video stream based on the information from the object detector and classifier. On the first frame, the tracker will construct a tracker instance for each bounding box that it receives. On every subsequent frame, we first attempt to associate the players detected in the current frame with existing trackers based on motion and appearance in the same way as ByteTrack+FastREID, and for the players that are associated with a tracker with a different player ID, we use the confidence score of the association to decide if we should update the player ID of the tracker to that of the player classifier's prediction going forward. For players that are not matched with any existing tracker, we use the classifier's prediction to create new trackers for them.

To account for occasional misses in the MOT model’s player detection, such as when a player is hidden behind another player, we approximate the missing bounding boxes of these players from those in nearby frames by independently interpolating the the x, y, width, and height attributes. We also apply smoothing to these four bounding box attributes across time to reduce noises in the detected bounding boxes. These post-processing steps are possible in a video streaming context because of the constant buffer time.

\paragraph{Pose Estimation}
 We also use ViTPose to compute the keypoints of each player given the MOT bounding boxes, in order to compute their horizontal centers when drawing the embedded visualizations. 

\subsection{Separate Foreground and Background}

\cmo{-why we need this step? ---> occlusion, drawing vis on the ground}

\cmo{-what we want to get from this step? --> foreground and background}

\cmo{-how do we obtain these?}

For each frame, we use ViT-Adapter (trained on COCO 160K) to perform binary semantic segmentation and isolate humans from the ground, in order to draw visualizations on the ground but beneath the players.

\subsection{Generalizability and Limitations}

 For better performance, we cached the segmentation masks and keypoints ahead of time when generating the demo videos, but these steps can theoretically be run in real time given sufficient hardware.
 
\cmo{which components rely on the buffer time?}
 
\cmo{which components rely on the annotated dataset?}

==> tex/_deprecated/4-cv_pipeline_v2.tex <==
\section{A CV Pipeline for Embedding Visualizations into Team Sports Videos}
\label{sec:cv_pipeline}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.1\textwidth]{figs/fig_41_cv_pipeline.pdf}
    \caption{Our CV pipeline takes a raw video as the input, 
    outputs the bounding box, identity, and keypoints of each player, 
    and separates the image frame into foreground (humans) and background (all others). 
    The outputs of players are used to create visualizations,
    which are then composited with the foreground and background to form the augmented video.}
    \label{fig:cv_pipeline}
\end{figure}

\noindent
% Based on the findings in our formative study,
% we aim to present extra data about players in basketball videos through embedded visualizations.
To embed visualizations to the players,
we need to recognize the players (e.g., bounding box, identity, and keypoints)
and segment them from the background if the visualizations are rendered on the court.
To this end,
we design a CV processing pipeline
that, theoretically, can be run in real live streaming scenarios for team sports.
% that can be run in real live streaming scenarios.
% using state-of-the-art techniques, 
% which can process video streams in real time with a constant buffer time of less than one minute. 

\subsection{Recognizing the Players}
To embed visualizations to a player in the video,
% visualize data, e.g., the name, of a player in the video, 
one must know 
the 2D position (bounding box) of the specific player (identity) in each video frame.
Besides, one may also need the keypoints of the player for properly placing the visualization.
% For each player,
Given a raw video frame,
we obtain these results of each player
via three steps:
1) detecting his/her bounding box,
2) tracking his/her identity across frames,
and 3) estimating his/her keypoints.

% The goal of this stage is to track players across frames in order to better infer the identity of the players in the current frame. 

\paragraph{Detecting the Players' Bounding Box.}
%% talk about design first
Detecting humans in videos is a common task in CV.
While there are many out-of-the-box human detectors,
they cannot distinguish players from non-players such as referees and audiences.
One feasible solution is to fine-tune or re-trained these human detectors
but needs significant time and computational resources.
Instead, we decide to train a light weight classifier 
that takes the outputs of a human detector as the input
and classifies them into players and non-players.
In our implementation,
we first used a pretrained YoLoX~\cite{} to detect all the humans in a video frame.
Then, we used a vision transformer based classifier~\cite{} to classify the detected bounding boxes.
The classifier was trained on a player dataset
manually annotated by ourselves.
The details of the dataset can be found in the supplemental materials.

% all humans detected in the frame
%% talk about implementation
% The first step of the player tracking module is to detect the bounding boxes of all players on the court. 
% This is a human-only object detection task, 
% and we achieve this using a YoloX model trained on CrowdHuman, MOT17, Cityperson and ETHZ (pretrained weights come from ByteTrack authors). 
% However, 
% this model it self does not distinguish players from non-players such as referees. 
% To improve the downstream accuracy of MOT, 
% we use the vision transformer as backbone to train a player classifier that can detect the identity of the players (with one class for non-players), 
% then use it to filter the bounding box detections of YoloX to minimize the number of candidates when matching. 

\paragraph{Tracking the Players' Identity.}
\cmo{The goal of MOT is to obtain the ids of each player across different frames.}
To track players across frames, 
we initialize a multi-object tracking task using ByteTrack with FastREID at the start of the video stream based on the information from the object detector and classifier. 
On the first frame, 
the tracker will construct a tracker instance for each bounding box that it receives. 
On every subsequent frame, 
we first attempt to associate the players detected in the current frame with existing trackers based on motion and appearance in the same way as ByteTrack+FastREID, and for the players that are associated with a tracker with a different player ID, we use the confidence score of the association to decide if we should update the player ID of the tracker to that of the player classifier's prediction going forward. 
For players that are not matched with any existing tracker, 
we use the classifier's prediction to create new trackers for them.

To account for occasional misses in the MOT model’s player detection, such as when a player is hidden behind another player, we approximate the missing bounding boxes of these players from those in nearby frames by independently interpolating the the x, y, width, and height attributes. We also apply smoothing to these four bounding box attributes across time to reduce noises in the detected bounding boxes. These post-processing steps are possible in a video streaming context because of the constant buffer time.

\paragraph{Pose Estimation}
 We also use ViTPose to compute the keypoints of each player given the MOT bounding boxes, in order to compute their horizontal centers when drawing the embedded visualizations. 

\subsection{Separate Foreground and Background}

\cmo{-why we need this step? ---> occlusion, drawing vis on the ground}

\cmo{-what we want to get from this step? --> foreground and background}

\cmo{-how do we obtain these?}

For each frame, we use ViT-Adapter (trained on COCO 160K) to perform binary semantic segmentation and isolate humans from the ground, in order to draw visualizations on the ground but beneath the players.

\subsection{Generalizability and Limitations}

 For better performance, we cached the segmentation masks and keypoints ahead of time when generating the demo videos, but these steps can theoretically be run in real time given sufficient hardware.
 
\cmo{which components rely on the buffer time?}
 
\cmo{which components rely on the annotated dataset?}

\cmo{the design space and the CV pipeline}

==> tex/_deprecated/4-cv_pipeline_v3.tex <==
\section{A CV Pipeline for Embedding Visualizations into Team Sports Videos}
\label{sec:cv_pipeline}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.1\textwidth]{figs/fig_41_cv_pipeline.pdf}
    \caption{Our CV pipeline takes a raw video as the input, 
    outputs the bounding box, identity, and key points of each player, 
    and separates the image frame into foreground (humans) and background (all others). 
    The bounding boxes, identities, and key points are used to create visualizations,
    which are then composited with the foreground and background to form the augmented video.}
    \label{fig:cv_pipeline}
\end{figure}

\noindent
To embed visualizations into a basketball video, 
% where the visualizations are shown on the court and situated next to the players,
we need to recognize the players (e.g., bounding box, identity, and key points)
and segment them from the background.
To this end,
we designed a CV processing pipeline (\autoref{fig:cv_pipeline})
that can run in real live streaming scenarios for team sports.

\subsection{Recognizing the Players}
To embed visualizations for a player,
one must first recognize the player in the video.
For example, to display a label with the name of a player, 
the system needs to detect 
which video object corresponds to the player (identity),
where the player is in the video frame (bounding box),
and sometimes the player's key body joints (key points) for placing the label.
Given a raw video frame,
we obtain this information for each player
via three steps:
% 1) detecting all the players (\autoref{fig:cv_pipeline}a),
% 2) identifying each player (\autoref{fig:cv_pipeline}b),
% and 3) estimating the key points of each player (\autoref{fig:cv_pipeline}c).

\paragraph{Step 1. Detecting Players (\autoref{fig:cv_pipeline}a).}
%% talk about design first
Detecting humans in images is a common task in CV.
While there are many out-of-the-box human detectors,
they cannot distinguish players from non-players such as referees and audiences.
One feasible solution is to fine-tune or retrain these human detectors,
which needs significant time and computational resources.
Instead, we trained a lightweight binary classifier 
that takes in image patches from the outputs of a human detector
and classifies them into players and non-players.
In our implementation,
we first use a pretrained YoLoX~\cite{ge2021yolox} to detect all the humans in a video frame.
Then, we use a vision transformer (ViT) based classifier~\cite{dosovitskiy2020image} to classify the detected bounding boxes 
and filter out all non-player bounding boxes.
The classifier was fine-tuned on an NBA player dataset manually annotated by ourselves.
The details of the dataset can be found in the supplemental material.
The output of this step is the bounding boxes of all the players in the video frame.

\paragraph{Step 2. Identifying Each Player (\autoref{fig:cv_pipeline}b).}
%%%% The goal of MOT is to obtain the ids of each player across different frames.
To embed the visualization to the correct player,
we further need to know the identity of each bounding box.
Ideally, this can be achieved by a player ID classifier 
that inputs a bounding box and outputs the player's identity as the class.
However, 
such a classifier only uses 
the visual appearance information of a player
and is unreliable at tracking players across frames. For example, the same player may face the camera from different angles or being occluded by others. This appearance variation can cause the classifier to predict incorrectly, resulting in poor identification performance.
To better identify each bounding box,
we further use a multi-object tracker~\cite{DBLP:journals/ai/LuoXMZLK21}
to exploit the motion information of a player across frames.
Specifically,
for a bounding box $b_{i}$ in the current frame $F_t$,
the tracker attempts to match it with a bounding box
in the previous frame $F_{t-1}$:
The tracker first uses a Kalman filter to
predict the new position in $F_t$ of each bounding box in $F_{t-1}$ 
based on their historical positions. 
Second, the tracker calculates the Intersection over Union (IoU) between $b_i$ and all these predicted bounding boxes.
All the predicted bounding boxes whose IoU exceeds a threshold are considered as \emph{matching}.
We assign the identity of the matching bounding boxes with the maximum IoU to $b_i$.
If $b_i$ does not match any bounding box in $F_{t-1}$,
we use our ID classifier to determine its player identity.
In our implementation,
we developed our tracker based on ByteTrack~\cite{zhang2022bytetrack} and Bot-SORT~\cite{aharon2022bot},
and fine-tuned a ViT-based model as the ID classifier 
by using the player dataset annotated by ourselves.

Occasionally, some players are missed in Step 1's detection
when they are occluded by other players.
Since the identities of bounding boxes associate players across frames,
we can interpolate the bounding box of a missing player
from his bounding boxes in nearby frames.
Specifically,
we independently interpolate the x, y, width, and height attributes of the missing bounding box using up to four nearby frames.
After interpolation,
we also apply smoothing to these four bounding box attributes 
across time to reduce noise from the player detector.
These post-processing steps are possible in a video streaming context 
because of the 5-second time window, which is created by the difference between the reality and the time the user sees in their livestream.
In summary, the output of this step is a list of refined bounding boxes for each frame
and their corresponding player identities.

\paragraph{Step 3. Estimating Players' Key Points.}
To better embed the visualizations into the video,
we also need to know the positions of the players' key points, such as head, hands, hip, and feet.
We achieve this by using a ViT-based pose estimation model.
In our implementation,
we first use the bounding boxes produced in the previous steps
to extract the players from the video frame
and then feed those bounding boxes to ViTPose~\cite{xu2022vitpose} to estimate the key points. 

\subsection{Separating Foreground and Background}
Embedding visualizations into the video often requires
resolving occlusion relationships between 
the visualizations and the video objects.
For example, 
to display player trajectories or empty areas,
we must visualize the data on the court, beneath the players' feet.
To achieve this, 
we need to separate the video frame into foreground (objects on the court) 
and background (the court),
draw the visualizations onto the background,
and finally composite the foreground with the background to
form the augmented video frame (\autoref{fig:cv_pipeline}d).
Since humans are the major objects on the court in a basketball video,
we thus use a ViT-Adapter~\cite{chen2022vitadapter} to perform binary semantic segmentation 
to segment humans from the court.
In our implementation, the ViT-Adapter is trained on COCO 164K~\cite{caesar2018coco}.

\subsection{Performance, Generalizability, and Limitations}

The contribution of our pipeline does not lie in the individual components
but a workable solution that shows
which CV models are required
and how they can be composited together 
to process basketball videos for the purpose of embedding visualizations into live video streams.
The models we used in our implementation can easily be substituted by others, 
based on the specific scenario and videos to process.
To inspire future research,
we further discuss the performance, generalizability, and limitations of our pipeline:

\paragraph{Performance.}
The models [\citealp{xu2022vitpose, chen2022vitadapter, zhang2022bytetrack, aharon2022bot, ge2021yolox, dosovitskiy2020image, DBLP:journals/ai/LuoXMZLK21}] used in our pipeline all achieve state-of-the-art performance in their own tasks.
In this work, we use this pipeline to process the two game videos (\autoref{tab:study1_games}) used in the formative study.
Since there is no ground truth data for these two videos,
we cannot quantitatively evaluate our pipeline on these two videos.
However, 
the performance of the pipeline 
can be qualitatively evaluated by inspecting the augmented videos,
which are lauded by the participants in the user study (\autoref{sec:evaluation}).
We provide multiple examples in the supplemental material for reference.

\paragraph{Generalizability.}
The CV pipeline is not only designed for the two basketball videos 
but can also be applied to other basketball videos 
and even other team sports videos.
The bottleneck of generalizing to other basketball videos
is to develop a player dataset for fine-tuning the id classifier.
For example, there are approximately 450 players in NBA~\cite{NBA}.
To generalize the pipeline to all NBA videos,
one needs to develop an image dataset with these 450 players
and fine-tune a 450-class classifier.
In practices, 
this is not impossible  
as modern deep learning-based image classifiers show the ability to
achieve superhuman performance on tasks with more than 1000 classes~\cite{yu2022coca}
and many priors can be used to optimize the model results, 
e.g., there are usually no more than 24 players in a game.

\paragraph{Limitations.}
There are several limitations in the pipeline.
First, in our current implementation,
the processing time for one frame is about 8 seconds on a machine with Nvidia Tesla V100 graphic card.
In reality,
the processing time can be accelerated with 
more powerful graphic cards, 
more lightweight models,
and better engineering implementation.
Second, our pipeline presumes a buffer time in the live streaming for the bounding box post-processing component (i.e., interpolation and smoothing).
In our implementation, we restrict the buffer time to be 5 seconds.
Yet, the requirement of the buffer time, 
as well as the post-processing component, can be eliminated
if the detection and tracking models can achieve a better performance.
Finally,
our pipeline only 
extracts 2D information from the video,
limiting the design space of available embedded visualizations.
For example, 
without extracting the camera parameters (i.e., intrinsic, extrinsic),
we cannot embed visualizations that are static in relation to the court, 
such as player trajectories.
Nonetheless, 
our pipeline supports embedded visualizations that are static in relation to the players,
which is sufficient to present 
a wide range of useful in-game data.
Next, we will show how we design gaze-moderated embedded visualizations
to improve casual fans' understanding and engagement in watching basketball games.


==> tex/_deprecated/4-cv_pipeline_v4.tex <==
\section{A CV Pipeline for Embedding Visualizations into Team Sports Videos}
\label{sec:cv_pipeline}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/fig_41_cv_pipeline@v2.pdf}
    \caption{Our CV pipeline takes a raw video as the input, 
    outputs the bounding box, identity, and key points of each player, 
    and separates the image frame into the foreground (humans) and background (all others). 
    The bounding boxes, identities, and key points are used to create visualizations,
    which are then composited with the foreground and background to form the augmented video.}
    \label{fig:cv_pipeline}
\end{figure}

\noindent
To embed visualizations into a basketball video, 
% where the visualizations are shown on the court and situated next to the players,
we need to recognize the players (e.g., bounding box, identity, and key points)
and segment them from the background.
To this end,
we designed a CV processing pipeline (\autoref{fig:cv_pipeline})
\cmo{to pre-process team sports videos.}
% that can run in real live streaming scenarios for team sports.

\subsection{Recognizing the Players}
To embed visualizations for a player,
one must first recognize the player in the video.
For example, to display a label with the name of a player, 
the system needs to detect 
which video object corresponds to the player (identity),
where the player is in the video frame (bounding box),
and sometimes the player's key body joints (key points) for placing the label.
Given a raw video frame,
we obtain this information for each player
via three steps:
% 1) detecting all the players (\autoref{fig:cv_pipeline}a),
% 2) identifying each player (\autoref{fig:cv_pipeline}b),
% and 3) estimating the key points of each player (\autoref{fig:cv_pipeline}c).

\paragraph{Step 1. Detecting Players (\autoref{fig:cv_pipeline}a).}
%% talk about design first
Detecting humans in images is a common task in CV.
While there are many out-of-the-box human detectors,
they cannot distinguish players from non-players such as referees and audiences.
One feasible solution is to fine-tune or retrain these human detectors,
which needs significant time and computational resources.
Instead, we trained a lightweight binary classifier 
that takes in image patches from the outputs of a human detector
and distinguishes players from non-players.
In our implementation,
we first use a pretrained YoLoX~\cite{ge2021yolox} to detect all the humans in a video frame.
Then, we use a vision transformer (ViT) based classifier~\cite{dosovitskiy2020image} to classify the detected bounding boxes 
and filter out all non-players.
The classifier was fine-tuned on an NBA player dataset manually annotated by ourselves.
The details of the dataset and training process can be found in Appendix A.
The output of this step is the bounding boxes of all the players in the video frame.

\paragraph{Step 2. Identifying Each Player (\autoref{fig:cv_pipeline}b).}
%%%% The goal of MOT is to obtain the ids of each player across different frames.
To embed the visualization to the correct player,
we further need to know the identity of each bounding box.
We accomplish this by using 
a multi-object tracker~\cite{DBLP:journals/ai/LuoXMZLK21}
and an ID classifier
to exploit the motion and visual appearance information of players across frames.
Specifically,
for a bounding box $b_{it}$ in the current frame $F_t$,
the tracker attempts to match it with a bounding box
in the previous frame $F_{t-1}$:
The tracker first uses a Kalman filter to
predict the new position in $F_t$ of each bounding box in $F_{t-1}$ 
based on their historical positions. 
Second, the tracker calculates the Intersection over Union (IoU) between $b_{it}$ and all these predicted bounding boxes.
All the predicted bounding boxes whose IoU exceeds a threshold are considered as \emph{matching}.
We assign the identity of the matching bounding boxes with the maximum IoU to $b_{it}$.
If $b_{it}$ does not match any bounding box in $F_{t-1}$,
we use the ID classifier to predict its player identity.
We refer the reader to Bot-SORT~\cite{aharon2022bot} for more technical details.
In our implementation,
we developed our tracker based on ByteTrack~\cite{zhang2022bytetrack},
and fine-tuned a ViT-based model as the ID classifier 
by using the player dataset annotated by ourselves.

Occasionally, some players are missed in Step 1's detection
when they are occluded by other players.
Since the identities of bounding boxes associate players across frames,
we can interpolate the bounding box of a missing player
from his bounding boxes in nearby frames.
Specifically,
we independently interpolate the x, y, width, and height attributes of the missing bounding box using up to four nearby frames.
After interpolation,
we also apply smoothing to these four attributes 
across time to reduce noise from the player detector.
We can interpolate and smooth the current frame
by using the next frames
by taking advantage of a 5-seconds streaming delay (i.e., buffer time) we set for ourselves.
In summary, the output of this step is a list of refined bounding boxes
and their corresponding player identities.

\paragraph{Step 3. Estimating Players' Key Points (\autoref{fig:cv_pipeline}c).}
To better embed the visualizations into the video,
we also need to know the positions of the players' key points, such as head, hands, hip, and feet.
We achieve this by using a ViT-based pose estimation model.
In our implementation,
we first use the bounding boxes produced in Step. 2
to extract the players from the video frame
and then feed those bounding boxes to ViTPose~\cite{xu2022vitpose} to estimate the key points. 

\subsection{Separating Foreground and Background}
Embedding visualizations into the video often requires
resolving occlusion relationships between 
the visualizations and the video objects.
For example, 
to display player trajectories or empty areas,
we must visualize the data on the court, beneath the players' feet.
To achieve this, 
we need to separate the video frame into foreground (objects on the court) 
and background (the court),
draw the visualizations onto the background,
and finally composite the foreground with the background to
form the augmented video frame (\autoref{fig:cv_pipeline}d).
Since humans are the major objects on the court in a basketball video,
we thus use a ViT-Adapter~\cite{chen2022vitadapter} to perform binary semantic segmentation 
to segment humans from the court.
In our implementation, the ViT-Adapter is trained on COCO 164K~\cite{caesar2018coco}.

\subsection{Performance, Generalizability, and Limitations}
\label{sec:cv_limitation}

The contribution of our pipeline does not lie in individual components
but a workable solution that shows
which CV models are required
and how they can be composited together 
to process basketball videos for the purpose of embedding visualizations into live video streams.
The models we used in our implementation can easily be substituted by others, 
based on the specific scenario and videos to process.
To inspire future research,
we further discuss the performance, generalizability, and limitations of our pipeline:

\paragraph{Performance.}
The models [\citealp{xu2022vitpose, chen2022vitadapter, zhang2022bytetrack, aharon2022bot, ge2021yolox, dosovitskiy2020image, DBLP:journals/ai/LuoXMZLK21}] used in our pipeline all achieve state-of-the-art performance in their own tasks, and we used their default hyperparameters whenever possible.
Due to the lack of ground truth data,
we cannot quantitatively evaluate our pipeline on the two videos in our study.
However, 
the performance of the pipeline 
can be qualitatively evaluated by inspecting the augmented videos,
which are lauded by the participants in the user study (\autoref{sec:evaluation}).
Examples are provided in the supplemental material for reference.

\paragraph{Generalizability.}
The CV pipeline 
can be applied to other basketball videos 
and even other team sports videos.
The bottleneck of generalizing to other basketball videos
is to develop a player dataset for fine-tuning the ID classifier.
For example, there are about 450 players in NBA~\cite{NBA}.
To generalize the pipeline to all NBA videos,
one needs to develop an image dataset with these 450 players
and fine-tune a 450-class classifier.
This is not impossible  
as modern deep learning-based image classifiers show the ability to
achieve superhuman performance on tasks with more than 1000 classes~\cite{yu2022coca}
and many priors can be used to optimize the model results, 
e.g., there are no more than 24 players in a game.

\paragraph{Limitations.}
There are several practical limitations in the pipeline.
First, 
the processing time of our pipeline
for one frame is about 8 seconds on a machine with a Nvidia Tesla V100 graphic card.
Thus, we used our pipeline to preprocess the game videos instead of running it in real-time for the user study.
% the two game videos (\autoref{tab:study1_games}) used in the formative study.
In reality,
the processing time can be accelerated with 
more powerful graphic cards, 
more lightweight models,
and better engineering implementation.
Second, 
our pipeline presumes a buffer time in the live streaming for the bounding box interpolation and smoothing.
Yet, the requirement of the buffer time, 
as well as the post-processing component, can be eliminated
if the detection and tracking models can achieve a better performance.
Finally,
our pipeline only 
extracts 2D information from the video,
limiting the design space of available embedded visualizations.
For example, 
without extracting the camera parameters (i.e., intrinsic, extrinsic),
we cannot embed visualizations that are static in relation to the court, 
such as player trajectories.
Nonetheless, 
our pipeline supports embedded visualizations that are static in relation to the players,
which is sufficient to present 
a wide range of useful in-game data.
% Next, we will show how we design gaze-moderated embedded visualizations
% to improve casual fans' understanding and engagement in watching basketball games.

==> tex/_deprecated/4-cv_pipeline_v5.tex <==
\section{A CV Pipeline for Embedding Visualizations into Team Sports Videos}
\label{sec:cv_pipeline}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_41_cv_pipeline@v2.pdf}
    \caption{Our CV pipeline takes a raw video as the input, 
    outputs the bounding box, identity, and key points of each player, 
    and separates the image frame into the foreground (humans) and background (all others). 
    The bounding boxes, identities, and key points are used to create visualizations,
    which are then composited with the foreground and background to form the augmented video.}
    \label{fig:cv_pipeline}
\end{figure}

\noindent
To embed visualizations into a basketball video, 
% where the visualizations are shown on the court and situated next to the players,
we need to recognize the players (e.g., bounding box, identity, and key points)
and segment them from the background.
To this end,
we designed a CV processing pipeline (\autoref{fig:cv_pipeline})
\cmo{to pre-process team sports videos.}

\subsection{Recognizing the Players}
To embed visualizations for a player,
one must first recognize the player in the video.
For example, to display a label with the name of a player, 
the system needs to detect the video object corresponds to the player (bounding box and identity)
and sometimes the player's key body joints (key points) for placing the label.
Given a raw video frame,
we obtain this information for each player
via three steps:

\paragraph{\textbf{Step 1. Detecting Players} (\autoref{fig:cv_pipeline}a).}
%% talk about design first
\cmo{
% we can use an object detection model.
% Object detection models usually output the category of each object in an image.
% Object detection is a common task in CV, 
% which 
To obtain the players' bounding boxes and identities in a video frame,
we can train an object detection model
that locates each player 
and classifies them into different categories.
Different from common object detection tasks,
we use the players' identities as their categories.
% and use the categories as their identities.
%detect the players in a video frame
% by using the players' identities as the categories.
In our implementation,
we fine-tuned a COCO~\cite{caesar2018coco} pretrained YoLoX~\cite{ge2021yolox} model
% we use YoLoX~\cite{ge2021yolox} to finish this task.
% The YoLoX model was pretrained on COCO
% and fine-tuned 
on an NBA player dataset (details in Appendix A). % manually annotated by ourselves.
% The details of the dataset and training process can be found in Appendix A.
The output of the model is
a set of bounding boxes associated with their identities and confidence scores (i.e., $score_{c}$).
By convention,
only those bounding boxes with $score_{c}$ greater than a threshold $T_{high}$
are considered successful detections.
}

\paragraph{\textbf{\cmo{Step 2. Post-Processing the Detections [Optional]}} (\autoref{fig:cv_pipeline}b).}
\cmo{
One limitation of the object detector is that
it only utilizes the players' visual appearance information
to determine their confidence score.
Consequently,
the detector can assign low confidence scores to players 
whose visual quality are low (e.g., when they are occluded by others)
and filter them out.
% some players can be missed due to low confidence score 
% the object detector in Step 1 can miss players,
% especially when their confidence scores are low .
% as these players 
% usually 
% This is because 
% the detector 
We thus use object trackers to exploit the players' motion information
to complement the detector.
An object tracker stores the history of an object's bounding boxes in the previous frames
and can predict the object's bounding box in the next frame by using a Kalman filter.
We use object trackers as follows:}
\begin{enumerate}
    \item 
\cmo{
    For a frame $F_t$,
    we divide all the detected bounding boxes into three clusters based on their $score_{c}$: 
    high-quality boxes ($score_{c} > T_{high}$),
    low-quality boxes ($T_{low} < score_{c} < T_{high}$),
    and rejected boxes ($score_{c} < T_{low}$).
    }
    
    \item 
    \cmo{
    For each high-quality box, 
    we match it with the trackers in the previous frame $F_{t-1}$
    by calculating the Intersection over Union (IoU)
    between the box and the predicted boxes of the trackers.
    A tracker is considered as \emph{matched} with the high-quality box if it maximizes the IoU.
    If matching successful, 
    % If a matched tracker exists, 
    we assign the matched tracker to the box;
    otherwise, we initialize a new object tracker for the  box.
    }
    
    \item 
    \cmo{
    For each low-quality box, 
    we match it with the remaining trackers 
    % in the previous frame $F_{t-1}$ 
    (i.e., those have not been matched with any high-quality boxes).
    If matching successful, 
    we assign the matched tracker to the box.
    }

    \item 
    \cmo{Finally, we output all the boxes with matched trackers.}

\end{enumerate}

\noindent
\cmo{
Intuitively, 
this method uses the motion information of the players to select 
some low-quality bounding boxes to complement the output of the detector.
% preserves , in addition to the high-quality ones, by using their motion information.
This step can be omitted when the object detector is perfect enough.
We refer the readers to Bot-SORT~\cite{aharon2022bot} for more details
of the tracker and the matching process.
}


% Occasionally, some players are missed in Step 1's detection
% when they are occluded by other players.
% Since the identities of bounding boxes associate players across frames,
% we can interpolate the bounding box of a missing player
% from his bounding boxes in nearby frames.
% Specifically,
% we independently interpolate the x, y, width, and height of the missing bounding box using up to four nearby frames.
% After interpolation,
% we also apply smoothing to these four attributes 
% across time to reduce noise from the player detector.
% We can interpolate and smooth the current frame
% by using the next frames
% by taking advantage of a 5-seconds streaming delay (i.e., buffer time) we set for ourselves.
    
% In summary, the output of this step is 
% a list of refined bounding boxes
% and their corresponding player identities.

\paragraph{\textbf{Step 3. Estimating Players' Key Points} (\autoref{fig:cv_pipeline}c).}
Finally, 
we use a pose estimation model to obtain the players' key points, 
such as head, hands, hip, and feet.
% achieve this by using a ViT-based 
In our implementation,
we first use the bounding boxes produced in Step. 2
to extract the players from the video frame
and then feed those bounding boxes to ViTPose~\cite{xu2022vitpose} 
to estimate the key points. 

\subsection{Separating Foreground and Background}
Embedding visualizations into the video often requires
resolving occlusion relationships between 
the visualizations and the video objects.
For example, 
to display player trajectories or empty areas,
we must visualize the data on the court, beneath the players' feet.
To achieve this, 
we need to separate the video frame into foreground (objects on the court) 
and background (the court),
draw the visualizations onto the background,
and finally composite the foreground with the background to
form the augmented video frame (\autoref{fig:cv_pipeline}d).
Since humans are the major objects on the court in a basketball video,
we thus use a ViT-Adapter~\cite{chen2022vitadapter} to perform binary semantic segmentation 
to segment humans from the court.
In our implementation, the ViT-Adapter is trained on COCO 164K~\cite{caesar2018coco}.

\subsection{\cmo{Computational Evaluation}}
\cmo{We conduct several computational experiments to evaluate the performance of our pipeline.
We are particularly interested in three questions:
1) Can the object detector detect players (i.e., bounding box and identity)?;
2) Can our post-processing step improve the detection results?;
3) How much time does each component in the pipeline take?
To answer these three questions, 
we manually annotated the bounding box and identity of each player 
in each frame of the two game videos used in~\autoref{sec:formative} (i.e., G1 and G2).
The details of the dataset can be found in Appendix A.
% To challenge our pipeline,
We evenly sampled 1/10 of the frames to fine-tune the object detector 
and used the remaining 9/10 to evaluate the components.
We didn't evaluate the accuracy of 
the models in the Pose Estimation and Semantic Segmentation components
because we used off-the-shelf models for their standard tasks in these two components.
% However, 
% the performance of these
% can be qualitatively evaluated by inspecting the augmented videos,
% which are lauded by the participants in the user study (\autoref{sec:evaluation}).
% Examples are provided in the supplemental material for reference.
To inspect the performance of these models,
we refer the readers to the papers~\cite{chen2022vitadapter, xu2022vitpose} 
and our example augmented videos in the supplemental material.
}

\begin{table}[h]
    % \begin{tabular}{p{0.27\linewidth} p{0.315\linewidth} p{0.34\linewidth}}
    \begin{minipage}[t]{.6\linewidth}\vspace{0pt}%
    % \small
    \centering
    \caption{.}
    \label{tab:model_exps}

    \begin{tabular}{l l l l l}
    
    \toprule
     \cmo{\textbf{Dataset}}   & \textbf{Component}  & \cmo{$\mathbf{AP_{50:95}}$} & \cmo{$\mathbf{AP_{50}}$} & \cmo{$\mathbf{AP_{75}}$}  \\ \midrule
    %% -----
    \multirow{2}{*}{\cmo{\textbf{G1}}}& Player Detection & 69.3 & 92.4 & 83.2\\
                                     &  Post-Processing & 73.2 (+3.9) & 96.4 (+4.0) & 86.9 (+3.7) \\ \hline
                                    %  &  Total &  & 96.4 & 86.9\\ \hline

    \multirow{2}{*}{\cmo{\textbf{G2}}}& Player Detection & 72.5 & 92.9 & 86.5\\
                                     &  Post-Processing & 77.4 (+4.9) & 97.3 (+4.4) & 91.0 (+4.5) \\ \hline
                                    %  &  Total &  &  & \\
        \textbf{COCO} & YoLoX & 51.2 & 69.6 & 55.7 \\
    \bottomrule
    \end{tabular}
    \end{minipage}%
    \begin{minipage}[t]{.4\textwidth} \vspace{0pt}%
    % \small
    \centering
    \caption{\cmo{
        }
    }
    \label{tab:model_time}
    \begin{tabular}{l r}
    \toprule
    \textbf{\textbf{Component}}  & \cmo{\textbf{Time (ms)}} \\ \midrule
    Player Detection & 31.98 \\
    Post-Processing & 2.40 \\
    Pose Estimation & 121.00 \\ \hline
    Semantic Seg. & 3674.96 \\  \bottomrule
    \end{tabular}
    \end{minipage}
\end{table}

\paragraph{Can the object detector detect players?}
Table.~\ref{tab:model_exps} 
shows the performance of our fine-tuned object detector on G1 and G2.
To access the detector,
we calculated the Average Precision (AP) metrics over different IoUs (the three columns in Table.\ref{tab:model_exps}),
which is a standard method to evaluate object detection tasks.
The higher the AP, the better it is.
$AP_{50:95}$ is the average AP over different IoU, from 0.5 to 0.95 with step 0.05.
$AP_{50}$ and $AP_{75}$ are the APs calculated at IoU 0.5 and 0.75, respectively.
The larger the IoU, the stricter the metric will be.
Due to the lack of benchmarks, we provide YoLoX's performance on COCO dataset as a reference.
Overall, these results reveal that our fine-tuned object detector 
can achieve a good performance on detecting players.

\paragraph{Can the post-processing component improve the detection results?}
Table.~\ref{tab:model_exps} also shows the AP of the outputs of our post-processing component.
All the AP increase after applying the post-processing component.
The results demonstrate that the post-processing component is useful and can improve the detection results.

\paragraph{How much time does each component in the pipeline take?}
Table.~\ref{tab:model_time} shows the average time in milliseconds (ms) each component takes to process a video frame.
We tested the pipeline on a machine with a Nvidia Tesla V100 graphic card
and only counted the inference time of the models by excluding the model and dataset loading time.
Overall, the player detector and post-processing components use ~34ms for one frame,
almost achieving a 30FPS.
Other components, especially the semantic segmentation, need longer time to process one frame.
These results show that the semantic segmentation model we used is the bottleneck
for extending the pipeline to a real-time setting.


% The models [\citealp{xu2022vitpose, chen2022vitadapter, zhang2022bytetrack, aharon2022bot, ge2021yolox, dosovitskiy2020image, DBLP:journals/ai/LuoXMZLK21}] used in our pipeline all achieve state-of-the-art performance in their own tasks, and we used their default hyperparameters whenever possible.
% Due to the lack of ground truth data,
% we cannot quantitatively evaluate our pipeline on the two videos in our study.





\subsection{Extendibility, Generalizability, and Limitations}
\label{sec:cv_limitation}

The contribution of our pipeline does not lie in the individual components
but a workable solution that shows
which CV models are required
and how they can be composited together 
to process basketball videos for the purpose of embedding visualizations into videos.
To inspire future research,
we further discuss the extendibility, generalizability and limitations of the pipeline:

\paragraph{Extendibility.}
It is not difficult to improve or extend our pipeline.
For example,
the models we used in our implementation can easily be substituted by better ones.
Further steps can be added to the post-processing component to process the detections.
For example, in our implementation, we further added an
interpolation and smoothing step to refine the bounding boxes.
In summary, our pipeline can server as a reference for other researchers
to develop their own ones
based on the specific scenario, videos to process, and tasks.

\paragraph{Generalizability.}
The CV pipeline 
can be applied to other basketball videos
and even other team sports videos.
The bottleneck of generalizing to other basketball videos
is to develop a player dataset for fine-tuning the player detector.
For example, there are about 450 players in NBA~\cite{NBA}.
To generalize the pipeline to all NBA videos,
one needs to develop an image dataset with these 450 players
and fine-tune a 450-class classifier.
This is not impossible  
as modern deep learning-based image classifiers show the ability to
achieve superhuman performance on tasks with more than 1000 classes~\cite{yu2022coca}
and many priors can be used to optimize the model results, 
e.g., there are no more than 24 players in a game.

\paragraph{Limitations.}
There are two major practical limitations in the pipeline.
First, 
as shown in Table.~\ref{tab:model_time}, 
the processing time of our pipeline
for one frame is about 4 seconds.
% on a machine with a Nvidia Tesla V100 graphic card.
While the semantic segmentation component can run in parallel with others,
our implementation still can only 
preprocess the game videos instead of running in real-time.
To accelerate the pipeline, we must reduce the time cost of the semantic segmentation component.
% In reality,
% the processing time can be accelerated with 
% more powerful graphic cards, 
% more lightweight models,
% and better engineering implementation.
% for the user study.
% cannot run in real-time
% it is still not possible
% Thus, we used our pipeline to 
Second, 
% in our implementation, we added a
% interpolation and smoothing step to refine the bounding boxes.
% To 
% our pipeline presumes a buffer time in the live streaming for the bounding box interpolation and smoothing.
% Yet, the requirement of the buffer time, 
% as well as the post-processing component, can be eliminated
% if the detection and tracking models can achieve a better performance.
% Finally,
our pipeline only 
extracts 2D information from the video,
limiting the design space of available embedded visualizations.
For example, 
without extracting the camera parameters (i.e., intrinsic, extrinsic),
we cannot embed visualizations that are static in relation to the court, 
such as player trajectories.
Nonetheless, 
our pipeline supports embedded visualizations that are static in relation to the players,
which is sufficient to present 
a wide range of useful in-game data.

==> tex/_deprecated/5-gaze_vis_v1.tex <==
\section{Gaze-moderated Embedded Visualizations}
\label{sec:gaze_moderated_vis}

\noindent
Based on the formative study, 
we design a set of gaze-moderated embedded visualizations
% to improve the game understanding and engagement of casual fans
% in watching live basketball videos.
that consist of three main components: 
using embedded visualizations to 
1) direct audiences' attention (\autoref{fig:gaze_vis}a)
and to 2) reveal players' offensive and defensive abilities (\autoref{fig:gaze_vis}b),
and 3) using gaze interactions to moderate the embedded visualizations (\autoref{fig:gaze_vis}c).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_50_gazevis.pdf}
    \caption{
        The system takes positional tracking data and historical stats as input to calculate the players' importance and offensive and defensive abilities.
        Only the important players and their offensive and defensive abilities will be highlighted and visualized into the video.
        The user can use gaze points to adjust the players' importance, as well as controlling whose abilities to show.
    }
    \label{fig:gaze_vis}
\end{figure}

\subsection{Directing Audiences' Attention}
\label{sec:direct_att}

% One major pain point of casual fans in watching basketball games 
% is that they are unsure about which players they should focus on (\hyperref[para:C1]{C1}).
% Thus, 
% casual fans usually spend much time and cognitive effort trying to identify the key players.
% , which degrades their game-watching experience.
To help casual fans effectively focus on the important players (\hyperref[para:C1]{C1}),
we first rank the players' importance levels according to die-hard fans' suggestions
and then highlight the players accordingly.
% visualize them using embedded visualizations.

\subsubsection{\textbf{Ranking Players' Importance Levels}}

\noindent
% Considering both the casual and die-hard fans' feedback in our formative study,
Based on the feedback from our formative study,
we adopt an offensive-first method to
rank the players' importance into three levels:
\begin{itemize}
    \item [\textbf{Lv3 -}] \textbf{Key offensive players}: 
        % On the offensive side,
        The player with the ball, 
        the next ball receiver, % of the ball,
        and the players with open spaces
        are considered as the most important offensive players.
        During a game, 
        the player with the ball or 
        with open spaces can be calculated based on the positional tracking data~\cite{sportvu}.
        In principle, machine learning models~\cite{DBLP:conf/soict/SanoN19} could be used to detect 
        the next ball receiver.
        % the player 
        % whom the ball will be passed to.
        In this work, however, we decided to leverage the buffer time that consistently exists in all live streaming videos to obtain the next ball receiver.
        Specifically, in each frame, 
        we look ahead into the next 1.8s (selected empirically) to obtain the next player with the ball.
    \item [\textbf{Lv2 -}] \textbf{Key defensive players}: 
        % On the defensive side,
        The players who are defending the player with the ball are considered as the important defenders.
        In our implementation,
        % These defenders can be estimated by the positional tracking data. 
        % That is, 
        the defensive players
        whose closest opponent is the offensive player with the ball 
        within a time interval 
        are considered as defending the player with the ball.
        While there is no ground truth data for defining these defenders,
        we manually verified the results 
        and found that they are overall accurate.

    \item [\textbf{Lv1 -}] \textbf{Other players}:
    All other players who do not belong to \textbf{Lv3} and \textbf{Lv2} fall into this level.
\end{itemize}

\noindent
To detect if a player is in offense or defense,
we also use the positions of the players and the ball:
if a player or one of her/his teammate is the closest player to the ball within a predefined time interval (0.5s in our implementation),
she/he is in offense; otherwise, in defense.
Note that we deliberately ignore some important players,
such as those who play screens or specific tactics,
since casual fans usually cannot understand why these players are important.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/fig_51_attention_level.pdf}
    \caption{Visualization of various importance levels: 
        \textbf{Lv3}, key offensive players;
        \textbf{Lv2.5}, players of interest to the user, triggered by \GFo{};
        \textbf{Lv2}, key defensive players;
        \textbf{Lv1}, other players.
    }
    \label{fig:att_lv}
\end{figure}

\subsubsection{\textbf{Visualizing Importance Levels}}

\noindent
To visualize the players in different importance levels,
we design multiple highlight effects (\autoref{fig:att_lv}).
% -- \autoref{fig:att_lv}a, b, and d for \textbf{Lv1}, \textbf{Lv2,} and \textbf{Lv3}, respectively.
% \textbf{Lv2.5} (\autoref{fig:att_lv}c) is designed to highlight the players that are of the user's interest, 
% which we will describe in \autoref{sec:gaze_int}.
We designed these highlighting effects considering both their effectiveness and aesthetics,
ensuring that they are \emph{natural}, \emph{intuitive},
and the one for a higher importance level is more \emph{attractive}, and vice verse.
% ensuring that they are  and 
% \emph{attractive} in an ascending order in basketball videos.
% Overall, the highlighted effects for 
Besides, 
we display the name of players whose importance level are greater than \textbf{Lv2}.
We also color the name of ``star'' players in golden
and add an icon in before to shows their roles (i.e., \inlinefig{figs/shooter.png} means good shooter and \inlinefig{figs/defender.png} means good defender).
To further encode the reason for highlighting of \textbf{Lv3} players,
we use a \emph{green} spotlight to highlight players with open spaces
and \emph{white} for others.

% a  spotlight to highlight the current and the next player with the ball,
% and 

\subsection{Revealing Players' Abilities} 
Casual fans rarely can understand, predict, and evaluate players' in-game decisions
due to their lack of knowledge about the players' offensive and defensive abilities (\hyperref[para:C2]{C2}).
% Based on die-hard fans' suggestions,
We compute and visualize two location-based metrics of the players whose attention level is higher than \textbf{Lv1}
to help casual fans understand the players' abilities (\autoref{fig:gaze_vis}b).

\subsubsection{\textbf{Measuring Players' Offensive and Defensive Abilities}}

\begin{figure}[h]
    \centering
    % \vspace{-2mm}
    \includegraphics[width=0.5\textwidth]{figs/fig_523_epv_map.png}
    \vspace{-2mm}
    \caption{An example EPV map of Steven Curry based on his shooting records in 2015-16 season. The darker color, the higher EPV.}
    \label{fig:epv_map}
\end{figure}

\noindent
We use two well-established metrics to indicate the players' offensive and defensive abilities:

\begin{itemize}
    \item \textbf{Offense - Expected Point Value (EPV)} 
    measures how many points a player is expected to make if he/she shoots from the current position.
    In basketball, it is a value between 0 and 3.
    Fundamentally, the goal of offensive tactics in basketball games
    is to maximize the EPV of the shooter.
    Thus, visualizing the EPV can
    help casual fans better understand and evaluate the in-game decisions of offensive players (e.g., pass or shoot).
    We obtain the EPV for each player based on their historical shot records.
    Specifically, 
    we create a shot chart~\cite{} for each player 
    by grouping the player's historical shot records 
    based on the shooting regions (defined by Official NBA Stats~\cite{nbastats}).
    Then we calculate the EPV per region by multiplying the player's field goal percentage and points they can make (i.e., 2 or 3) in the region
    and cache the results as an EPV map, 
    which we can access efficiently in a live game.
    Figure~\ref{fig:epv_map} shows an example EPV map.

    \item \textbf{Defense - Percentage Points Difference (DIFF\%)} \textcolor{cb_red}{measures the difference between 
    the normal shot percentage of an offensive player
    and the shot percentage of the offensive player 
    when guarded by the current defensive player.} \textcolor{cb_blue}{replace by "measures the difference of shot percentage when the offensive player is guarded or not." }
    Good defenders will have a negative DIFF\% since they hold their opponent to a lower percentage than normal.
    In addition to DIFF\%, the distance between a defender and the offensive player with the ball (DIST) is critical to the defensive performance.
    With these two metrics, casual fans can better understand both the defensive and offensive players' actions.
    We acquire DIFF\% by regions for each player directly through the Official NBA Stats~\cite{nbastats}
    and calculate DIST based on the positional tracking data.
\end{itemize}

\begin{figure}[h]
    \centering
    % \vspace{-2mm}
    \includegraphics[width=0.98\textwidth]{figs/fig_52_dataVis.pdf}
    \vspace{-2mm}
    \caption{Three embedded visualizations for in-game data:
        a) \OffR{} shows the offensive performance of an offensive player. The darker, larger, the better.
        b) \DefS{} shows the defensive performance of the defender. The thicker, longer, the better.
        c) \OOOL{} shows the one-on-one relationship between the offensive player with the ball and the defenders.
    }
    \label{fig:od_data}
\end{figure}

\subsubsection{\textbf{Visualizing Players' Offensive and Defensive Abilities}}
\noindent
We designed two embedded visualizations 
based on prior work~\cite{lin2022the, yao2022visualization} and video games~\cite{}
for the offensive (EPV) and defensive (DIFF\% and DIST) metrics, 
respectively.
We further visualize the one-on-one relationship between the defenders and the offensive player with the ball:
\begin{itemize}
    \item \textbf{\OffR{}} (\autoref{fig:od_data}a) 
    presents the location-based EPV of a player.
    An offensive ring is a radial (not tangential) progress bar, 
    whose inner and outer rings represent the minimum and maximum possible EPV (i.e., 0 and 3).
    We adopt a double encoding method for EPV, using both size and color of the middle ring to represent a player's EPV at the current position.
    In short, the larger, darker, the better.

    \item \textbf{\DefS{}} (\autoref{fig:od_data}b) 
    shows the location-based DIFF\% of a defender and his/her DIST.
    We use the thickness of the ``shield'' to represent the inverse DIFF\%, 
    which is a negative value, to make the visualization intuitive and easy to understand.
    We further use the length of the ``shield'' to encode \underline{\emph{maximum guarding distance} $-$ DIST}.
    Thus, the larger the DIST, the shorter the ``shield''.
    We choose this design also for intuitive understanding.
    We display a outer boarder of the ``shield'' to hint the maximum guarding distance, 
    which is selected empirically as 12 feet.
    In sum, the thicker, longer, the better.

    \item \textbf{\OOOL{}} (\autoref{fig:od_data}c) 
    visualize the one-on-one relationship between the defenders and the offensive player with the ball.
    % are visualized directly by using connected lines between 
    The relationships are computed in identifying the key defensive players (\autoref{sec:direct_att}).
    The player with the ball can be defended by multiple defenders.
\end{itemize}

\noindent
All these three visualizations are updated dynamically in the game based on the players' positions.
We particularly designed the visualizations to be placed on the ground to not obstruct the view of the main parts of the game, 
such as the players and ball.
We also 
darken the background image
to provide enough contrast 
for reading the visualizations.

\subsection{Gaze-based Interactions}
\label{sec:gaze_int}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/fig_53_interactions.pdf}
    \vspace{-4mm}
    \caption{Two gaze interactions to adjust the embedded visualizations:
        a) \GFo{} lift the importance level and shows in-game data of players that are of interest to the user.
        b) \GFi{} drop the importance level of video objects who are not the user's focus (e.g., open players out of the focus, audiences).
    }
    \label{fig:gaze_int}
\end{figure}

\noindent
While the aforementioned embedded visualizations provide extra information for the user,
they may still fail to fulfill casual fans' individual data needs.
Meanwhile, 
casual fans seldomly proactively take action to fulfill their own data needs (\hyperref[para:C3]{C3}).
Besides, the embedded visualizations can overwhelm casual fans 
who have various game and data literacy.
We design two gaze interactions (\autoref{fig:gaze_vis}c) 
to help casual fans 
naturally moderate the embedded visualizations during their game watching,
achieving a balance between the machine's suggestions and user preferences.

% personalize the embedded visualizations
% implicitly and naturally.
% With these two interactions,
% \system{} enables users 

\subsubsection{\textbf{\GFo{} -- Fetching Data of Players of Interest to the User}}
% gaze-focus, show the data of the user's interest
\noindent
Although \system{} automatically highlights important players, 
users very often have their own players of interest.
To show data for the players of interest to the user, 
we design \emph{\GFo{}} that 
allows the user to lift the importance level of these players.
\GFo{} comprises the following three considerations:
% \cmo{should have one sentence to summarize how it looks like}
\begin{itemize}
    \item \textbf{Trigger}: 
    According to our formative study, the users' gaze can move rapidly between, and across, players.
    To avoid showing data of players glanced over by the user accidentally, 
    we define a ``dwell time''~\cite{DBLP:conf/ozchi/PenkarLW12} for the interaction.
    Simply put, the user needs to dwell her/his gaze on a player for 0.2 second to trigger the interaction.

    \item \textbf{Visual feedback}:
    It is crucial to provide visual feedback on interactions built upon ``dwell time'' 
    so that the user can realize that she/he is gazing at a player
    and triggering the interaction.
    Thus, we designed a highlight effect (\autoref{fig:att_lv}c) in which 
    the glow of the player 
    will gradually increase when the user is gazing on the player, until the interaction is triggered.
    Our design not only provides intuitive visual feedback for the user but also naturally 
    fits into the visual design of importance levels. 
    % by satisfying all the three XXX (\cmo{more explicit about which three considerations?}).

    \item \textbf{Outcome}: 
    Once the user triggers the interaction, \system{} lifts the targeted player to \textbf{Lv2.5} if she/he is currently in a lower level (\autoref{fig:gaze_int}a).
    As a result, the system will also visualize the name and offensive or defensive data of the player.
    Lastly, when the user moves her/his gaze away from the player, 
    the player will stay in \textbf{Lv2.5} for 1.8s before reverting to their original player importance level.
    We design such a lasting duration to cope with the users' rapid saccade in game watching. % (\cmo{found in the formative study}).
\end{itemize}


\subsubsection{\textbf{\GFi{} -- De-emphasizing Video Objects Out of the Sight}}
% Augmenting basketball games easily, 
% which is already fast enough for casual fans,
% can overwhelm the user.
% \cmo{need to elaborate that our idea is that overwhelming is bc attention issue.}
\noindent
Although we use various highlighting effects 
to help users focus on the more important players,
sometimes the users can still be overwhelmed 
due to too many highlighted players,
% there can be too many highlighted players
% the number of highlighted players sometimes can be too many,
e.g., several offensive players are open and highlighted by a green spotlight.
To reduce the number of highlighted players
while still helping the user identify important players,
we designed \emph{\GFi{}} that enables the user to
drop the importance level of video objects who are not the user's focus.
\GFi{} incorporates three considerations:

\begin{itemize}
    \item \textbf{Trigger}:
    % Since we have already used ``dwell time'', 
    % the most common way to trigger gaze interactions, for \GFo{}, 
    % we take a different approach for triggering the \GFi{}.
    % To distinguish from the trigger of 
    % Different from \GFo{},
    Generally speaking, the system should always avoid overwhelming the user.
    Thus, we designed \GFi{} to be consistently triggered and updated when the user moves his/her gaze.
    
    \item \textbf{Visual feedback}:
    To indicate the user that the interaction is triggering, 
    we designed a radial blurring effect 
    that darkens the audiences outside a filter radius (650px in our implementation).
    This radial blurring effect is centered at the user's gaze point 
    and thus moves dynamically along with the user's gaze.
    We smooth the movement of the radial blurring effect
    to prevent it from abruptly changing location due to the user's saccade.
    Note that the blurring effect will not be applied to players and the court to ensure their readability.
    This visual feedback can notify the user about the existence of the interaction
    but also create a theater mode that helps the user focus on and engage with the game.
    
    \item \textbf{Outcome}: 
    The interaction will turn off all the green spotlights,
    which are used to highlight offensive players with open spaces, 
    outside the filter radius (\autoref{fig:gaze_int}b).
    Again, this filtering is updated dynamically when the user moves his/her gaze.
    An ease-in-out effect is applied to the spotlight when it is toggled between on and off.

\end{itemize}


==> tex/_deprecated/5-gaze_vis_v2.tex <==
\section{User Study}
\label{sec:evaluation}

To assess the usability, usefulness, and engagement 
of using our gaze-moderated embedded visualizations in watching live basketball videos,
we conducted a comparative study between three modes --
watch with raw footage (\RAW{}), 
with solely embedded visualizations (\AUG{}),
and with gaze-moderated embedded visualizations (\FULL{}).

\subsection{Study Settings}

\subsubsection{\textbf{Participants and Apparatus}}
\noindent
We recruited 16 casual fans (F1-F16; M = 10, F = 6; Age: 18 - 35) through university mailing lists and forums 
after screening for their fandom levels and basketball knowledge.
All participants
watched \quot{less than 10 games per year} 
and only \quot{know the basic rules} about basketball.
All participants had not participated in our formative study.
The study was conducted in lab with a 24-inch monitor.
We followed the same ergonomic settings in the formative study 
but changed to use a Tobii eye tracker 5~\cite{}
for more accurate gaze interactions.
The study took about one hour and each participant was compensated with a \$20 gift card.

\subsubsection{\textbf{Design and Procedure}}
\noindent
The study consisted of two tasks, namely,
\textbf{Task1 - \RAW{} vs. \AUG{}}, 
% comparing \RAW{} and \AUG{} mode, 
and \textbf{Task2 - \AUG{} vs. \FULL{}}.
Each task compared two modes.
% comparing \AUG{} and \FULL{} mode.
For each task,
we used a game video from the formative study
and evenly splitted it into two video clips (each lasting around 4.5 minutes)
for each mode.
The videos and the order of modes in each task
were counterbalanced across participants.
Each session included the following phases:

\paragraph{Phase 1. Introduction (10mins).}
The study started with an introduction of the research motivation, 
the purpose of the study, 
and the protocol.
After the participants signed the consent form, 
we conducted a warm-up interview of basketball game-watching experiences.

\paragraph{Phase 2. Comparative Tasks (40mins).}
After the introduction,
we asked participants to finish two comparative tasks (each lasted 20 mins):
In \textbf{Task1 - \RAW{} vs. \AUG{}}, 
the participants watched two video clips in \RAW{} and \AUG{} modes, respectively.
    Before \AUG{} mode, we conducted a training session to
    walk the participant through the four embedded visualizations in a separate video (about 20 seconds).
    We only proceeded to the \AUG{} mode when participants were clear and confident enough to use the embedded visualizations.
In \textbf{Task2 - \AUG{} vs. \FULL{}}, 
the participants watched another two video clips in \AUG{} and \FULL{} mode, respectively. 
Again, a training session was conducted before starting \FULL{} mode to ensure the participant were confident to use the gaze interactions.
Participants were encouraged to think aloud about their game observations when watching the videos.
% After watching each video clip, 
At the end of each video clip,
we performed a post-video interview to
collect the participants' feedback on the mode they had just experienced.
% either the embedded visualizations or the gaze interactions
% based on the specific mode they had just experienced.
At the end of each task, 
participants filled out a post-task questionnaire to rate their experiences.

\paragraph{Phase 3. Post-study Questionnaire (10mins).}
At the end of the session,
we asked participants to complete a post-study questionnaire of 
their subjective ratings on the overall system,
rank the three modes,
and provide feedback on the entire system.

\subsubsection{\textbf{Measures}}
\noindent
Similar to the formative study, 
we recorded the think-aloud for each task.
Besides, 
we collect quantitative measurements of user subjective ratings 
in the post-task 
and post-study questionnaires.
At the end of each task, 
participants were asked to rate the usefulness, engagement, and usability of the features 
they had just experienced,
i.e., the four visualizations (i.e., Player Highlight, \OffR{}, \DefS{}, and \OOOL{}) in \textbf{Task1}
and the two gaze interactions (i.e., \GFo{} and \GFi{}) in \textbf{Task2},
on a 7-point Likert scale.
In the post-study questionnaires,
we asked participants to rated the overall system on five questions regarding system usefulness and engagement~\cite{} 
and ranked the three modes. 
% We also collected and analyzed qualitative feedback from the participants in post-task and post-study interviews.

\subsection{Study Results}
We first report 
% the participants' 
the ratings of the overall system 
and the rankings of the three modes,
and then discuss the feedback on the usefulness, engagement, and usability of
individual visualizations and interactions.

\subsubsection{\textbf{The overall user experience of \system{} was predominantly positive, with \FULL{} being most preferred}}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_61_overall.pdf}
    \caption{Left: Ratings on the overall system. Right: Rankings of different conditions, 
        i.e., \RAW{} -- watch with raw footage,
        \AUG{} -- watch with embedded visualizations solely,
        \FULL{} -- watch with gaze interaction and embedded visualizations.
        }
    \label{fig:overall}
\end{figure}

\noindent
% The participants overarchingly spoke highly of \system{}.
As shown in \autoref{fig:overall} left, 
the majority rated \system{} as \quot{helpful} and \quot{fun}, 
felt \quot{in control} and \quot{encouraged} when using the system,
and were \quot{likely to use} the system for watching basketball games.
Figure~\ref{fig:overall} right presents the rankings of the three modes,
showing that 
\FULL{} was the most preferred mode by 12 participants, 
followed by \AUG{} by 4 and \RAW{} by none. 
% The rankings revealed that the gaze-moderated embedded visualizations designed by us were preferred by most of the participants.
%% P11, don't like the bluring of the audiences
%% P7 don't like the blurring due to the visual artifacts
%% p8 don't like the blurring of audience seems abnormal, and don't feel overwhelming.
Among four participants who didn't rank \FULL{} as the best,
% While there is 
% one participant simple preferred \AUG{} over \FULL{} for no reason;
they were mainly concerned about  
the blurring effect of the audience in the \GFi{}, 
stating that 
% They disliked the visual artifacts introduced by the blurring effect %of the audiences
a game video without audiences seemed abnormal.
However, all of them agreed that the filtering of open players (highlighted in green) was useful.
Such customization
can be easily achieved 
by providing a \quot{Preferences} panel to enable users to configure their preferred settings.
In summary,
while \GFi{} can be improved by providing more customization,
participants provided very positive feedback on \system{},
demonstrating that the system
can effectively improve the experience of casual fans in watching live basketball videos.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_62_vis+gaze.pdf}
    \caption{Ratings on the embedded visualizations and gaze interactions.}
    \label{fig:rate_vis}
\end{figure}


% \subsubsection{\textbf{Simple visualizations that link to immediate game actions and react to user's gaze were favored by participants}}
% \noindent
% Taken together, 
% each embedded visualization supports different game insights for audience, similar to the findings of~\cite{lin2022the}. 
% What's more interesting is that casual fans in our study preferred visualizations that can be easily noticed (e.g., Player Highlight or player name with \GFo{}) 
% and link to immediate action, 
% such as indicating shooting action with \OffR{} or \DefS{}.

\subsubsection{\textbf{Embedded visualizations are useful if they are attrative and informative}}
\noindent
Participants rated positively on the usefulness of each visualization (\autoref{fig:rate_vis}a).
Among the four embedded visualizations,
Player Highlight was considered to be the most useful
in \quot{predicting the ball receiver} at the next pass,
\quot{highlighting the open players},
and thus \quot{making the game much clearer}, 
as mentioned by the participants.

Participants also rated \OffR{} and \DefS{} as useful to understand players' in-game decisions.
For example, F8 thought that \OffR{}
can \quot{help me expect when he's gonna shoot. Otherwise, it's just like this person can shoot anytime.};
F3 commented that \DefS{} clearly showed \quot{who's able to defend} 
and explained why \quot{James can easily score on Iguodala}.
However, 
some participants found them less useful 
since the visualizations were placed on the ground,
different from the ball at hand-height,
and thus often hard to notice in a tense game.
Nevertheless, most of the participants agreed that 
\quot{it was nice to have} \OffR{} and \DefS{} in the system.

\OOOL{} was controversial in terms of usefulness. 
Some participants 
considered it helpful \quot{to follow the game and to see who was involved [in defending]} (F6)
while others felt it suffers from the same limitations 
as \OffR{} and \DefS{} (i.e., cannot be noticed)
with less useful information 
that was already \quot{clear from the video} (F1).
P13 also suggested that we could show the one-on-one relationships for more players 
other than just for the player with the ball.

\subsubsection{\textbf{Gaze interactions are useful 
as they satisfy audiences' own information and cognitive needs
}}
\noindent
Both \GFo{} and \GFi{}
received very positive ratings regarding usefulness (\autoref{fig:rate_vis}a).
% With gaze interactions, participants naturally adjusted the embedded visualizations
% to satisfy their own information needs and cognitive bandwidth.
Participants particularly enjoyed using \GFo{}
as it could help them \quot{know the name of the player [who I am looking at]} (e.g., F1 - F16).
This simple yet effective information can significantly help casual fans to \quot{follow the game and understand who is who} (F16).
\GFi{} also 
improved the game understanding of participants
as it could \quot{make the scene tidier} (F22)
and \quot{focus the information on what I'm looking [at]} (F4).

\subsubsection{\textbf{Embedded visualizations are engaging since they provide a deeper epistemic pleasure}}
\noindent
The participants felt that 
the embedded visualizations are engaging (\autoref{fig:rate_vis}b)
since they can help them \quot{understand and follow the game}.
This is also reflected 
in the positive relationship between the usefulness and engagement of the embedded visualizations -- 
the more useful, the more engaging.
For example,
F1, a novice in watching NBA games, 
commented that \quot{it is nice to know who the star players are because otherwise, they all look like regular players to me.}
F5 remarked that he \quot{always tried to predict the receiver of a pass but always failed}.
With the visualizations, he felt much more confident in predicting the receiver and 
felt quite a sense of accomplishment whenever he was correct.

\subsubsection{\textbf{Gaze interactions are engaging since they promote proactive game viewing experiences}}
\noindent
Gaze interactions are also engaging (\autoref{fig:rate_vis}b)
since they make the passive watching experience
interactive and proactive.
As F2 explained, when the video scene responded to her gaze, 
she felt that she was \quot{also a part of the game.}
F4 particularly enjoyed using the gaze interactions 
which made the videos much more \quot{responsive}
and made him \quot{almost feel like I'm there}.
% P9 feel the theater mode
% \cmo{Participants' gaze patterns also revealed that the participants would more actively look for players when using gaze interactions.}
Moreover, participants suggested that using the gaze interactions was \quot{natural} (e.g., F9, F14) 
and would not add further cognitive cost to the game watching 
since \quot{you can actively control it ... you don't have to [use it]} (F5).
Overall, 
the participants' feedback
provides a strong hint 
that the engagement of watching sports videos can be significantly improved
if video content responds to the audience's gaze.

\subsubsection{\textbf{The gaze-moderated embedded visualizations are easy to understand and use}}
\noindent
All participants confirmed the usability of the embedded visualizations and gaze interactions in \system{} (\autoref{fig:rate_vis}c).
They thought both the visualizations and gaze interactions were \quot{easy to understand} and \quot{use}
(e.g., F8, F14 - F16).
We noticed that while some participants thought that \OOOL{} was not that useful,
they still agreed that it was easy to understand.
Their ratings demonstrated that our design of \system{} 
is effective: even the games were fast and tense, 
the visualizations and interactions were still easy to understand and use
while watching the game.

\subsection{Implications for Designing Gaze-moderated Embedded Visualizations}
We now discuss the design implications we learned from the feedback and observations in the user study.

\subsubsection{\textbf{Attention to Visual Attention}}
% -- pay attention to visual attention, overwhelming, attentions,
\noindent
While we were concerned that embedded visualizations would impose additional cognitive load on watching an already fast-paced basketball game, 
most participants in our study did not find the visualizations overwhelming.
Instead, some participants even could not 
notice several embedded visualizations (e.g., \OffR{} and \DefS{}).
The participants' feedback actually reveals the Inattentional Blindness~\cite{DBLP:journals/tvcg/HealeyE12} phenomena,
in which viewers can completely fail to perceive visually salient objects or activities.
This finding implies that 
when designing embedded visualizations, % for dynamic scenarios, such as in sports,
\textbf{properly directing the user's attention sometimes can be more effective and important
than reducing the visual complexity
for avoiding overwhelming}.
Additionally,
this finding also implies that 
designer must consider users' attention in designing embedded visualizations
for effectively conveying information.
For example,
F5 discussed with us that 
we should highlight the \OffR{}, instead of players,
if we want to help the audiences efficiently identify which player has the highest EPV.
Besides, one could also highlight visualizations that link to immediate actions
to increase the information salience, 
e.g., highlight the \OffR{} when the player is about to shoot.

% -- commentaries and augmentations
\subsubsection{\textbf{The Interaction Between Seeing and Hearing}}
\noindent
F4 particularly mentioned that
he paid less attention to the commentaries in \AUG{} mode
but listened to them more carefully in \RAW{} mode,
which implied that the embedded visualizations can ``overlay'' the commentaries.
In fact, 
almost all the participants 
switch their main information source 
from the commentaries to the embedded visualizations
when watching the game in \AUG{} or \FULL{} mode.
This observation indicates that
there is an interaction between 
the participants' perception of the embedded visualizations and commentaries.
Such an interaction between human's hearing and vision system has long been identified (e.g., McGurk effect~\cite{}).
Interestingly, in \FULL{} mode,
several participants provided that they would try to search the players mentioned by the commentators by using the gaze interactions.
Thus,
it is crucial to synchronize the commentaries (hearing) 
and embedded visualizations (vision)
to achieve a consistent and convivial watching experience.
Several participants suggested that we can leverage the commentaries to create embedded visualizations.
A recent paper~\cite{chen2022sporthesia} explores this direction for racket-based sports.


%% gaze interactions open free exploration space, interfering the watching
\subsubsection{\textbf{Gaze Interactions Shift the Game from Explanatory to Exploratory}}
\noindent
In \FULL{} mode,
sometimes the participants would continuously follow the players highlighted by their gaze,
thereby missing important passes or shots.
On the other hand, in \AUG{} mode,
participants tended to follow and
focused more on the players highlighted by the system.
Such a difference suggests 
that \AUG{} mode is more explanatory
while adding gaze interactions can shift it towards exploratory.
This is not surprise as the audiences have larger space to actively explore with the gaze interactions.
As such,
when designing gaze interactions for game viewing systems or, broadly speaking, 
any situated visualizations systems that involve visual guidance,
designers must bear the ultimate goal of the systems in mind
and strike a balance between explanatory and exploratory.
Future work can extend this line to consider human-AI interaction for embedded visualizations.

% -- learn by watching
\subsubsection{\textbf{Gaze Interactions Enable Learning by Watching}}

\noindent
The gaze interactions can not only improve game watching experience 
but also help audiences progressively learn basketball tactics.
For example, 
\GFi{} only highlights empty players with green spotlight when the players are near the user's gaze.
With this feature,
F3 could verify if his hypothesis is correct.
When sometimes he thought that 
there should be open players in a corner,
he could move his gaze to the corner
and confirm his guessing if the system \quot{showed green [highlighting]} there.
Besides, F15 also elaborated that \GFo{}
helped him better recognize players
by showing the name of a player to confirm 
that he was looking at the right person.
Such a hypothesis-testing process 
made the participants feel more confident in 
interpreting the game.
We see this as an interesting opportunity 
to leverage gaze-moderated embedded visualization 
to develop long term impact 
for the users
beyond improving their watching experience within individual games.

\subsubsection{\textbf{Suggestions}}
\noindent
%% Limitations
% -- visual artifacts,  overlaps, 
While the participants generally spoken highly of \system{},
they did complain about a few limitations related to the system implementations.
For example, F8 disliked the visual artifacts introduced by the imperfect segmentation model;
some participants said that \GFo{} could not accurately highlight the target when the players crowded together.
These limitations can be resolved with more advanced models or eye trackers.
Besides,
the participants did suggest several features 
that can improve the user experience of \system{}.
% when applying it in practice.
% -- further customizability
First, the system should provide more customization 
such as supporting toggling off / on some visualizations,
visualizing other data,
and modifying the parameters of the interactions.
This can be easily implemented 
by allowing the user to configure the system in a \quot{Preference} panel.
% --  adapt to pace, information load
Second, multiple participants pointed out that
the visualizations were 
more readable in slow paced situations 
(e.g., when a player is dribbling outside the three-point line)
and harder to notice when the game is fast paced
(e.g., when a player is cutting in).
Thus, they suggested that the visualizations should also adapt to the pace of the game.
One solution is to use the average moving speed of the players as
an indicator of the pace of the game to adapt the visualizations.
% -- play by play replay
Another point worth to mention is that 
a few participant 
wished the system can generated play-by-play replays with embedded visualizations
to explain the game in details
rather than augmenting the live videos.
We see this requirement as an interesting future research direction.

==> tex/_deprecated/6-user_study_v1.tex <==
\section{User Study}
\label{sec:evaluation}

To assess the usefulness, usability, and engagement 
of using our gaze-moderated embedded visualizations in watching live basketball videos,
we conducted a comparative study between three modes --
watch with raw footage (\RAW{}), 
with solely embedded visualizations (\AUG{}),
and with gaze-moderated embedded visualizations (\FULL{}).\jb{use active voice, not passive voice, in this section}

\subsection{Participants and Apparatus}

We recruited 16 casual fans (F1-F16; M = 10, F = 6; Age: 18 - 35) through university mailing lists and forums 
after screening for their fandom levels and basketball knowledge.
All participants
watched \quot{less than 10 games per year} 
and only \quot{know the basic rules} about basketball.
All participants had not participated in our formative study.
The study was conducted in lab with a 24-inch monitor.
We followed the same ergonomic settings in the formative study 
but changed to use a Tobii eye tracker 5~\cite{}
for more accurate gaze interactions.
% to better support the gaze interactions.
The study took about one hour and each participant was compensated with a \$20 gift card.

\subsection{Design \& Procedure}
The study consisted of two tasks, including \textbf{Task 1}, comparing RAW vs. AUG mode, and \textbf{Task 2}, comparing AUG vs. FULL mode.
Four video clips (each lasting around 4.5 minutes) were prepared by evenly splitting the two videos from the formative study, and two were used in each task. 
The video clips and the order of modes in each task
were counterbalanced across participants.
Similar to the formative study, we recorded the think-aloud and gaze data for each task.
Each study included the following phases:

\noindent \textbf{I. Introduction (10mins).}
The study started with an introduction of the research motivation, 
the purpose of the study, and the protocol.
After the participants signed the consent form, we then conducted a warm-up interview of basketball game-watching experiences.

\noindent \textbf{II. Comparative Tasks (40mins).}
After the introduction,
we asked participants to finish two comparative tasks (each lasted 20 mins).   Participants were encouraged to think aloud about their game observations when watching the videos.
\begin{itemize}
    \item \textbf{Task 1} -- \RAW{} vs. \AUG{}. 
    The participants watched two basketball video clips in \RAW{} and \AUG{} modes, respectively.
    Before \AUG{} mode, we conducted a training session to
    walk the participant through the four embedded visualizations in a separate video (about 20 seconds).
    We only proceeded to the \AUG{} mode when participants were clear and confident enough to use the embedded visualizations.
    % At the end of Task 1,
    % the participants were asked to rate the usefulness, engagement, and usability of
    % the four embedded visualizations (i.e., key players highlight, offense ring, defense shield, and one-on-one line) 
    % using a 1 - 7 point Likert scale.
    
    \item \textbf{Task 2} -- \AUG{} vs. \FULL{}. 
    Participants watched two more basketball video clips in \AUG{} and \FULL{} mode, respectively. 
    Again, a training session was conducted before starting \FULL{} mode to ensure the participant were confident to use the gaze interactions.
    % The participants rated the usefulness, engagement, and usability of
    % the two gaze interactions (i.e., \GFo{} and \GFi{}) using 1 to 7 points at the end of this task.
\end{itemize}

% We encouraged participants to think aloud when watching the video clips.
% We evenly split each of the two videos in the formative study into two halves
% to gather four video clips (each lasting around 4.5 minutes) for Task 1 and 2.
% The video clips and the order of modes in each task
% were counterbalanced across participants.
% Similar to the formative study, we recorded the think aloud and gaze data for each task.

After watching each video clip, 
we performed a semi-structured interview to
collect the participants' feedback on either the embedded visualizations or the gaze interactions
% we asked the participant to provide feedback 
based on the specific mode they had just experienced.
% We also encouraged the participants to
% describe what they had found when watching the video. 
At the end of each task, participants filled out a post-task questionnaire to rate their experiences.

\noindent \textbf{III. Post-study ratings and feedback (10mins).}
At the end, 
participants were asked to complete a post-study questionnaire on their subjective ratings and feedback on the overall system and ranking of three system modes.
% we asked the participants to rate the system as a whole using 1 to 7 points,
% where we derived ,
% We also asked participants to rank the three modes based on their preferences.
% Finally, we collected suggestions and criticisms of the entire system.

\subsection{Measures}
We collect quantitative measurements of user subjective ratings in the post-task and post-study questionnaires.
At the end of each task, participants were asked to rate the usefulness, engagement, and usability of the study conditions on a 7-point Likert scale, including evaluating four visualizations (i.e., key players highlight, offense ring, defense shield, and one-on-one line) in Task 1 and two gaze interactions (i.e., \GFo{} and \GFi{}) in Task 2. Participants also rated the overall system on five questions regarding system usefulness and engagement~\cite{} and ranked three system modes. We also collected and analyzed qualitative feedback from the participants in post-task and post-study interviews.

\subsection{Study Results}
We first report 
% the participants' 
the ratings of the overall system 
and the rankings of the three modes,
and then discuss the feedback on the usefulness, engagement, and usability of
individual visualizations and interactions.

\subsubsection{The overall user experience of \system{} was deemed positive and gaze interactions were most preferred.}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_61_overall.pdf}
    \caption{Left: Ratings on the overall system. Right: Rankings of different conditions.}
    \label{fig:overall}
\end{figure}

\noindent
% The participants overarchingly spoke highly of \system{}.
As shown in \autoref{fig:overall} left, the majority rated \system{} as \quot{helpful} and \quot{fun}, felt \quot{in control} and \quot{encouraged} when using the system,
and were \quot{likely to use} the system for watching basketball games.
Figure~\ref{fig:overall} right shows the rankings of the three modes,
% Among the three modes,
showing that 
\FULL{} was the most preferred mode by 12 participants, followed by \AUG{} by 4 and \RAW{} by none. 
% one (Rank1 x 11),
% followed by \AUG{} (Rank1 x 4) and \RAW{} (Rank1 x 0).
% ranked by 11 participants as the best;
% \AUG{} was championed by 5 participants;
% \RAW{} received 0 vote for the best.
% The rankings revealed that the gaze-moderated embedded visualizations designed by us were preferred by most of the participants.
%% P11, don't like the bluring of the audiences
%% P7 don't like the blurring due to the visual artifacts
%% p8 don't like the blurring of audience seems abnormal, and don't feel overwhelming.
Among four participants who didn't rank \FULL{} as the best,
% While there is 
% one participant simple preferred \AUG{} over \FULL{} for no reason;
they were mainly concerned about  
the blurring effect of the audience in the \GFi{} 
% (P7, P8, P11)
, stating that 
% They disliked the visual artifacts introduced by the blurring effect %of the audiences
% and felt that 
a game video without audiences seemed abnormal.
However, all of them agreed that the filtering of open players (highlighted in green) was useful.
% Thus, they suggested keeping the filtering of open players but remove the blurring of the audience,
Such customization
can be easily achieved 
by providing a \quot{Preferences} panel to enable users to configure their preferred settings.
In summary,
while \GFi{} can be improved by providing more customization,
participants provided very positive feedback on \system{},
demonstrating that the system
can effectively improve the experience of casual fans in watching live basketball videos.

% Such positive feedback demonstrated that our design of \system{}
% Their critics on the blurring effect is also reflected 
% This is also reflected in the detailed ratings on the gaze filter feature, 
% which will be elaborated in the following sections.
%% P10, not useful

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_62_vis+gaze.pdf}
    \caption{Ratings on the embedded visualizations and gaze interactions.}
    \label{fig:rate_vis}
\end{figure}

\subsubsection{Usefulness -- how can \system{} improve game understanding?}
\noindent
Figure.~\ref{fig:rate_vis}a shows the participants' rating on the usefulness of each visualization and interaction.
%%%% the vis
Among the four embedded visualizations,
Player Highlight was considered to be the most useful
as it \quot{helps me predict whom the ball will be passed to},
\quot{spotlights the open players},
and thus \quot{make[s] the game much clearer} (e.g., P5 - P7, P12, P13).

Participants also rated Offense Ring and Defense Shield as useful
because they helped to understand players' in-game decisions.
For example, P8 thought that Offense Ring
can \quot{help me expect when he's gonna shoot. Otherwise, it's just like this person can shoot anytime...};
P3 commented that Defense Shield clearly showed \quot{who's able to defend} 
and explained why \quot{James can easily score on Iguodala} for example.
However, 
some participants also complained about the usefulness of Offense Ring and Defense Shield
since they \quot{often cannot be noticed} (e.g., P2 - P6).
Specifically, the participants could hardly allocate attention to read the visualizations
because 1) the games were often too tense 
and 2) the visualizations were beneath the players' feet while the ball was mostly at hand-height.
P5 said that \quot{the visualizations can be more natural for football [since] the audience mainly stares at the players' feet.}
Yet, P5 was also concerned about the visual clutter that would result when visualizing data in mid-air rather than beneath the players' feet.
Nevertheless, most of the participants agreed that 
\quot{it is nice to have} Offense Ring and Defense Shield in the system.

One-on-one link was controversial in terms of usefulness.
On one hand, 
some participants (e.g., P3, P6, P9)
lauded one-on-one link 
as it could help audiences \quot{to follow the game and to see who was involved [in defending]} (P6).
%% good things
On the other hand,
participants also indicated that
it suffers from the same limitations 
as Offense Ring and Defense Shield (i.e., cannot be noticed)
but providing less useful information. % to the participants.
P1 felt the line \quot{is not really necessary} because the line only shows the relationships between 
the player with the ball and
the defenders, which were already \quot{clear from the video}.
P13 also suggested that we could show the one-on-one relationships for more players 
other than just for the player with the ball.

Finally, both \GFo{} and \GFi{}
received very positive ratings regarding usefulness.
With gaze interactions, participants naturally adjusted the embedded visualizations
to satisfy their own information needs and cognitive bandwidth.
Participants particularly enjoyed using \GFo{}
as it could help them \quot{know the name of the player [who I am looking at]} (e.g., P1 - P16).
This simple yet effective information can significantly help casual fans to \quot{follow the game and understand who is who} (P16).
\GFi{} also 
improved the game understanding of participants
as it could \quot{make the scene tidier} (P22)
and \quot{focus the information on what I'm looking [at]} (P4).


% I felt like the line is really necessary because the defenders are only shown anyways for the person who has the ball. Yeah, so it's clear that this is a 1 to 1 relationship. So ii didn't really look for the line because it was clear from the from the defender, having a bar and the others, not having a bar.

% Another interesting finding is that participants slightly prefer Defense Shield than Offense Ring
% since it was easier to read due to its placement between the offensive and defensive players
% and the metaphor of shield was semantically related to defense.

\subsubsection{Engagement -- how can iBall improve engagement?}
\noindent
Participants rated 
that the embedded visualizations and gaze interactions improved engagement while watching basketball games (\autoref{fig:rate_vis}b).
The engagement afforded by the embedded visualizations
is deeply rooted in the deeper epistemic pleasure these visualizations can provide for casual users.
This is also reflected 
in the positive relationship between the usefulness and engagement of the embedded visualizations -- 
the more useful, the more engaging.
Specifically,
all participants agreed that the embedded visualizations are engaging 
since they can help them \quot{understand and follow the game}.
With the embedded visualizations, participants felt that they had a much clearer understanding and sometimes even felt \quot{omniscient} (P5) about the games.
P1, a novice in watching NBA games, 
commented that \quot{it is nice to know who the star players are because otherwise, they all look like regular players to me.}
P5 remarked that he \quot{always tried to predict the receiver of a pass but always failed}.
With iBall, he felt much more confident in predicting the receiver and 
felt quite a sense of accomplishment whenever he was correct.

Gaze interactions can improve the engagement in game watching
since they make the watching experience interactive and proactive rather than passive.
As P2 explained, when the video scene responded to her gaze, 
she felt that she was \quot{also a part of the game.}
P4 particularly enjoyed using the gaze interactions 
which made the videos much more \quot{responsive}
and made him \quot{almost feel like I'm there}.
% P9 feel the theater mode
\cmo{Participants' gaze patterns also revealed that the participants would more actively look for players when using gaze interactions.}
Moreover, participants suggested that using the gaze interactions was \quot{natural} (e.g., P9, P14) 
and would not add further cognitive cost to the game watching 
since \quot{you can actively control it ... you don't have to [use it]} (P5).
Overall, 
the participants' feedback
provides a strong hint 
that the engagement of watching sports videos can be significantly improved
if video content responds to the audience's gaze.

% since he felt the videos were much more responsive
% The interactions can help 
% With the interactions, participants
% also improve the engagement in watching games

% The embedded visualizations can make the game more engaging
% since they can provide a deeper epistemic pleasures for the casual users.
% The embedded visualizations can improve the engagement since they can \quot{help me understanding and follow the game} (e.g., P1).

%% engagement provide

\subsubsection{Usability -- how easy to use iBall?}
% how easy to use and understand the augmentation
\noindent
All participants confirmed the usability of the embedded visualizations and gaze interactions in iBall (\autoref{fig:rate_vis}c).
They thought both the visualizations and gaze interactions were \quot{easy to understand} and \quot{use}
(e.g., P8, P14 - P6).
We noticed that while some participants thought that one-on-one link was not that useful,
they still agreed that it was easy to understand.
Their ratings demonstrated that our design of \system{} %interactive embedded visualizations % in live basketball videos
is effective: even the games were fast and tense, 
the visualizations and interactions were still easy to understand and use
when watching the game.
% when watching the games.

\subsection{Feedback, Observations, and Implications}


\paragraph{Attention to Visual Attention in Designing Embedded Visualizations.}
% -- pay attention to visual attention, overwhelming, attentions,
One of our major concern in designing \system{} is 
that the embedded visualizations can overwhelm the users,
given that the basketball games are already overwhelming.
%% overwhelming
However, in our study, 
most of the participants didn't feel the visualizations were overwhelming.
Instead, some participants even could not notice several embedded visualizations (e.g., Offense Ring and Defense Shield).
% Some participants (e.g., P8, P10) even didn't feel 
The participants' feedback actually reveals the Inattentional Blindness~\cite{DBLP:journals/tvcg/HealeyE12} phenomena,
in which viewers can completely fail to perceive visually salient objects or activities.
This finding implies that 
when designing embedded visualizations, % for dynamic scenarios, such as in sports,
\textbf{properly directing the user's attention sometimes can be more effective and important
than reducing the visual complexity
for avoiding overwhelming}.
Additionally,
this finding also implies that 
designer must consider the user's attention in designing embedded visualizations
for effectively conveying information.
For example,
P5 discussed with us that 
we should highlight the Offense Rings, instead of players,
if we want to help the audience efficiently identify which player has the highest EPV.
\cmo{potential solution?}

\paragraph{The interaction between seeing and hearing.}
% -- commentaries and augmentations
One participant (P4) particularly mentioned that
he paid less attention to the commentaries in \AUG{} mode
but listened to them more carefully in \RAW{} mode.
% the commentaries were more clear to him ,
which implied that the embedded visualizations can ``overlay'' the commentaries.
In fact, 
almost all the participants 
switch their main information source 
from the commentaries to the embedded visualizations
when watching the game in \AUG{} mode.
This observation indicates that
there is an interaction between 
the participants' perception of the embedded visualizations and commentaries.
Such an interaction between human's hearing and vision system has long been identified (e.g., McGurk effect~\cite{}).
Interestingly, in \FULL{} mode,
several participants provided that they would try to search the players mentioned by the commentators by using the gaze interactions.
All these observations together suggested 
that it is crucial to synchronize the commentaries (hearing) and embedded visualizations (vision)
to achieve a consistent and convivial watching experience.
Several participants (e.g., P1, P5, P11) suggested that we can leverage the commentaries to create embedded visualizations.
A recent paper~\cite{chen2022sporthesia} explores the method to directly create embedded visualizations based on commentary text. 

\paragraph{Gaze interactions shift the game from explanatory to exploratory.}
%% gaze interactions open free exploration space, interfering the watching
In \FULL{} mode,
sometimes the participants would continuously follow the players highlighted by their gaze,
thereby missing important passes or shots.
On the other hand, in \AUG{} mode,
participants tended to follow and
focused more on the players highlighted by the system.
Such a difference suggests 
that \AUG{} mode is more explanatory
while adding gaze interactions can shift it towards exploratory.
This is not surprise as the audiences have larger space to actively explore with the gaze interactions.
As such,
when designing gaze interactions for game viewing systems or, broadly speaking, 
any situated visualizations systems that involve visual guidance,
designers must bear the ultimate goal of the systems in mind
and strike a balance between explanatory and exploratory.

\paragraph{Gaze interactions enable learning by watching.}
% -- learn by watching
The gaze interactions can not only improve game watching experience 
but also help audiences progressively learn basketball tactics.
For example, \GFi{} only highlights empty players with green spotlight when the players are near the user's gaze.
With this feature,
P3 could verify if his hypothesis is correct.
When sometimes he thought that 
there should be open players in a corner,
he could move his gaze to the corner
and confirm his guessing if the system \quot{showed green [highlighting]} there.
Besides, P15 also elaborated that \GFo{}
could help him better recognize players
by showing the name of a player to confirm 
that he was looking at the right person.
Such a hypothesis-testing process 
made him feel more confident in analyzing the game 
and interpreting the tactics of the players.
We see this as an interesting opportunity 
to leverage gaze-moderated embedded visualization 
to develop long term impact 
for the users
beyond improving their watching experience within individual games.
% This observation shows that embedded visualizations plus gaze interactions
% can not only improve watching experiences within games 
% but also 
% improve game watching experiences of casual fans in

\paragraph{Suggestions.}
%% Limitations
% -- visual artifacts,  overlaps, 
While the participants generally spoken highly of \system{},
they did complain about a few limitations related to the system implementations.
For example, P8 hated the visual artifacts introduced by the imperfect segmentation model;
some participants said that \GFo{} could not accurately highlight the target when the players crowded together.
These limitations can be resolved with more advanced models or eye trackers.
Besides,
the participants did suggest several features 
that can significantly improve the user experience of \system{}
when applying it in practice.
% -- further customizability
First, the system should provide more customization 
such as supporting toggling off / on some visualizations,
visualizing other data,
and modifying the parameters of the interactions.
This can be easily implemented 
by allowing the user to configure the system in a \quot{Preference} panel.
% --  adapt to pace, information load
Second, multiple participants pointed out that
the visualizations were 
more readable in slow paced situations 
(e.g., when a player is dribbling outside the three-point line)
and harder to notice when the game is fast paced
(e.g., when a player is cutting in).
Thus, they suggested that the visualizations should also adapt to the pace of the game.
One solution is to use the average moving speed of the players as
an indicator of the pace of the game to adapt the visualizations.
% -- play by play replay
Another point worth to mention is that 
a few participant 
wished the system can generated play-by-play replays with embedded visualizations
to explain the game in details
rather than augmenting the live videos.
We see this requirement as an interesting future research direction.

==> tex/_deprecated/6-user_study_v2.tex <==
\section{User Study}
\label{sec:evaluation}

To assess the usefulness, usability, and engagement 
of using our gaze-moderated embedded visualizations in watching live basketball videos,
we conducted a comparative study between three modes --
watch with raw footage (\RAW{}), 
with solely embedded visualizations (\AUG{}),
and with gaze-moderated embedded visualizations (\FULL{}).\jb{use active voice, not passive voice, in this section}

\subsection{Participants and Apparatus}

We recruited 16 casual fans (F1-F16; M = 10, F = 6; Age: 18 - 35) through university mailing lists and forums 
after screening for their fandom levels and basketball knowledge.
All participants
watched \quot{less than 10 games per year} 
and only \quot{know the basic rules} about basketball.
All participants had not participated in our formative study.
The study was conducted in lab with a 24-inch monitor.
We followed the same ergonomic settings in the formative study 
but changed to use a Tobii eye tracker 5~\cite{}
for more accurate gaze interactions.
% to better support the gaze interactions.
The study took about one hour and each participant was compensated with a \$20 gift card.

\subsection{Design and Procedure}
\cmo{The study consisted of two tasks, including \textbf{Task 1}, comparing RAW vs. AUG mode, and \textbf{Task 2}, comparing AUG vs. FULL mode.
Four video clips (each lasting around 4.5 minutes) were prepared by evenly splitting the two videos from the formative study, and two were used in each task. 
The video clips and the order of modes in each task
were counterbalanced across participants.
Similar to the formative study, we recorded the think-aloud and gaze data for each task.}
Each study included the following phases:

\noindent \textbf{I. Introduction (10mins).}
The study started with an introduction of the research motivation, 
the purpose of the study, and the protocol.
After the participants signed the consent form, we then conducted a warm-up interview of basketball game-watching experiences.

\noindent \textbf{II. Comparative Tasks (40mins).}
After the introduction,
we asked participants to finish two comparative tasks (each lasted 20 mins).   Participants were encouraged to think aloud about their game observations when watching the videos.
\begin{itemize}
    \item \textbf{Task 1} -- \RAW{} vs. \AUG{}. 
    The participants watched two basketball video clips in \RAW{} and \AUG{} modes, respectively.
    Before \AUG{} mode, we conducted a training session to
    walk the participant through the four embedded visualizations in a separate video (about 20 seconds).
    We only proceeded to the \AUG{} mode when participants were clear and confident enough to use the embedded visualizations.
    % At the end of Task 1,
    % the participants were asked to rate the usefulness, engagement, and usability of
    % the four embedded visualizations (i.e., key players highlight, offense ring, defense shield, and one-on-one line) 
    % using a 1 - 7 point Likert scale.
    
    \item \textbf{Task 2} -- \AUG{} vs. \FULL{}. 
    Participants watched two more basketball video clips in \AUG{} and \FULL{} mode, respectively. 
    Again, a training session was conducted before starting \FULL{} mode to ensure the participant were confident to use the gaze interactions.
    % The participants rated the usefulness, engagement, and usability of
    % the two gaze interactions (i.e., \GFo{} and \GFi{}) using 1 to 7 points at the end of this task.
\end{itemize}

% We encouraged participants to think aloud when watching the video clips.
% We evenly split each of the two videos in the formative study into two halves
% to gather four video clips (each lasting around 4.5 minutes) for Task 1 and 2.
% The video clips and the order of modes in each task
% were counterbalanced across participants.
% Similar to the formative study, we recorded the think aloud and gaze data for each task.

After watching each video clip, 
we performed a semi-structured interview to
collect the participants' feedback on either the embedded visualizations or the gaze interactions
% we asked the participant to provide feedback 
based on the specific mode they had just experienced.
% We also encouraged the participants to
% describe what they had found when watching the video. 
At the end of each task, participants filled out a post-task questionnaire to rate their experiences.

\noindent \textbf{III. Post-study ratings and feedback (10mins).}
At the end, 
participants were asked to complete a post-study questionnaire on their subjective ratings and feedback on the overall system and ranking of three system modes.
% we asked the participants to rate the system as a whole using 1 to 7 points,
% where we derived ,
% We also asked participants to rank the three modes based on their preferences.
% Finally, we collected suggestions and criticisms of the entire system.

\subsection{Measures}
\cmo{We collect quantitative measurements of user subjective ratings in the post-task and post-study questionnaires.
At the end of each task, participants were asked to rate the usefulness, engagement, and usability of the study conditions on a 7-point Likert scale, including evaluating four visualizations (i.e., key players highlight, offense ring, defense shield, and one-on-one line) in Task 1 and two gaze interactions (i.e., \GFo{} and \GFi{}) in Task 2. Participants also rated the overall system on five questions regarding system usefulness and engagement~\cite{} and ranked three system modes. We also collected and analyzed qualitative feedback from the participants in post-task and post-study interviews.}

\subsection{Study Results}
We first report 
% the participants' 
the ratings of the overall system 
and the rankings of the three modes,
and then discuss the feedback on the usefulness, engagement, and usability of
individual visualizations and interactions.

\subsubsection{\cmo{The overall user experience of \system{} was predominantly positive, with gaze interactions being most preferred.}}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_61_overall.pdf}
    \caption{Left: Ratings on the overall system. Right: Rankings of different conditions.}
    \label{fig:overall}
\end{figure}

\noindent
% The participants overarchingly spoke highly of \system{}.
As shown in \autoref{fig:overall} left, the majority rated \system{} as \quot{helpful} and \quot{fun}, felt \quot{in control} and \quot{encouraged} when using the system,
and were \quot{likely to use} the system for watching basketball games.
Figure~\ref{fig:overall} right shows the rankings of the three modes,
% Among the three modes,
showing that 
\FULL{} was the most preferred mode by 12 participants, followed by \AUG{} by 4 and \RAW{} by none. 
% one (Rank1 x 11),
% followed by \AUG{} (Rank1 x 4) and \RAW{} (Rank1 x 0).
% ranked by 11 participants as the best;
% \AUG{} was championed by 5 participants;
% \RAW{} received 0 vote for the best.
% The rankings revealed that the gaze-moderated embedded visualizations designed by us were preferred by most of the participants.
%% P11, don't like the bluring of the audiences
%% P7 don't like the blurring due to the visual artifacts
%% p8 don't like the blurring of audience seems abnormal, and don't feel overwhelming.
Among four participants who didn't rank \FULL{} as the best,
% While there is 
% one participant simple preferred \AUG{} over \FULL{} for no reason;
they were mainly concerned about  
the blurring effect of the audience in the \GFi{} 
% (P7, P8, P11)
, stating that 
% They disliked the visual artifacts introduced by the blurring effect %of the audiences
% and felt that 
a game video without audiences seemed abnormal.
However, all of them agreed that the filtering of open players (highlighted in green) was useful.
% Thus, they suggested keeping the filtering of open players but remove the blurring of the audience,
Such customization
can be easily achieved 
by providing a \quot{Preferences} panel to enable users to configure their preferred settings.
In summary,
while \GFi{} can be improved by providing more customization,
participants provided very positive feedback on \system{},
demonstrating that the system
can effectively improve the experience of casual fans in watching live basketball videos.

% Such positive feedback demonstrated that our design of \system{}
% Their critics on the blurring effect is also reflected 
% This is also reflected in the detailed ratings on the gaze filter feature, 
% which will be elaborated in the following sections.
%% P10, not useful

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_62_vis+gaze.pdf}
    \caption{Ratings on the embedded visualizations and gaze interactions.}
    \label{fig:rate_vis}
\end{figure}

% \subsubsection{Usefulness -- how can \system{} improve game understanding?}
\subsubsection{\cmo{Simple visualizations that link to immediate game actions and react to user's gaze were favored by participants.}}
\noindent
Figure.~\ref{fig:rate_vis}a shows the participants' rating on the usefulness of each visualization and interaction.
%%%% the vis
Among the four embedded visualizations,
Player Highlight was considered to be the most useful
in \quot{predicting whom the ball will be passed to},
\quot{highlighting the open players},
and thus \quot{making the game much clearer}, as mentioned by five participants.
% Player Highlight was considered to be the most useful
% as it \quot{helps me predict whom the ball will be passed to},
% \quot{spotlights the open players},
% and thus \quot{make[s] the game much clearer} (e.g., P5 - P7, P12, P13).

Participants also rated Offense Ring and Defense Shield as useful to understand players' in-game decisions.
For example, P8 thought that Offense Ring
can \quot{help me expect when he's gonna shoot. Otherwise, it's just like this person can shoot anytime.};
P3 commented that Defense Shield clearly showed \quot{who's able to defend} 
and explained why \quot{James can easily score on Iguodala}.
However, 
some participants found them less useful due to the limited mental bandwidth, particularly due to the tense game pace and the position of visualizations different from the ball at hand-height. 
% since they \quot{often cannot be noticed} (e.g., P2 - P6).
% Specifically, the participants could hardly allocate attention to read the visualizations
% because 1) the games were often too tense and 2) the visualizations were beneath the players' feet while the ball was mostly at hand-height.
% P5 said that \quot{the visualizations can be more natural for football [since] the audience mainly stares at the players' feet.}
% Yet, there was also concern about the visual clutter when placing visualization above the player.
% P5 was also concerned about the visual clutter that would result when visualizing data in mid-air rather than beneath the players' feet.
Nevertheless, most of the participants agreed that 
\quot{it was nice to have} Offense Ring and Defense Shield in the system.

One-on-one link was controversial in terms of usefulness. 
Some participants 
% (e.g., P3, P6, P9)
considered it helpful \quot{to follow the game and to see who was involved [in defending]} (P6)
%% good things
% On the other hand,
% participants also indicated that
while others felt it suffers from the same limitations 
as Offense Ring and Defense Shield (i.e., cannot be noticed)
with less useful information % to the participants.
% P1 felt the line 
% \quot{is not really necessary} because the line only shows the relationships between 
% the player with the ball and
% the defenders, which 
that was already \quot{clear from the video (P1)}.
P13 also suggested that we could show the one-on-one relationships for more players 
other than just for the player with the ball.

Finally, both \GFo{} and \GFi{}
received very positive ratings regarding usefulness.
With gaze interactions, participants naturally adjusted the embedded visualizations
to satisfy their own information needs and cognitive bandwidth.
Participants particularly enjoyed using \GFo{}
as it could help them \quot{know the name of the player [who I am looking at]} (e.g., P1 - P16).
This simple yet effective information can significantly help casual fans to \quot{follow the game and understand who is who} (P16).
\GFi{} also 
improved the game understanding of participants
as it could \quot{make the scene tidier} (P22)
and \quot{focus the information on what I'm looking [at]} (P4).

\cmo{Taken together, each embedded visualization supports different game insights for audience, similar to the findings of \cite{lin2022the}. What's more interesting is that casual fans in our study preferred visualizations that can be easily noticed (e.g., Player Highlight or player name with Gaze Focus) and link to immediate action, such as indicating shooting action with Offense Ring or Defense Shield.}

% I felt like the line is really necessary because the defenders are only shown anyways for the person who has the ball. Yeah, so it's clear that this is a 1 to 1 relationship. So ii didn't really look for the line because it was clear from the from the defender, having a bar and the others, not having a bar.

% Another interesting finding is that participants slightly prefer Defense Shield than Offense Ring
% since it was easier to read due to its placement between the offensive and defensive players
% and the metaphor of shield was semantically related to defense.

% \subsubsection{Engagement -- how can iBall improve engagement?}
\subsubsection{\cmo{The engaging visualizations and responsive gaze interactions promote proactive game viewing experiences.}}
\noindent
Participants rated
that the embedded visualizations and gaze interactions improved engagement while watching basketball games (\autoref{fig:rate_vis}b).
The engagement afforded by the embedded visualizations
is deeply rooted in the deeper epistemic pleasure these visualizations can provide for casual users.
This is also reflected 
in the positive relationship between the usefulness and engagement of the embedded visualizations -- 
the more useful, the more engaging.
Specifically,
all participants agreed that the embedded visualizations are engaging 
since they can help them \quot{understand and follow the game}.
With the embedded visualizations, participants felt that they had a much clearer understanding and sometimes even felt \quot{omniscient} (P5) about the games.
P1, a novice in watching NBA games, 
commented that \quot{it is nice to know who the star players are because otherwise, they all look like regular players to me.}
P5 remarked that he \quot{always tried to predict the receiver of a pass but always failed}.
With iBall, he felt much more confident in predicting the receiver and 
felt quite a sense of accomplishment whenever he was correct.

Gaze interactions can improve the engagement in game watching
since they make the watching experience interactive and proactive rather than passive.
As P2 explained, when the video scene responded to her gaze, 
she felt that she was \quot{also a part of the game.}
P4 particularly enjoyed using the gaze interactions 
which made the videos much more \quot{responsive}
and made him \quot{almost feel like I'm there}.
% P9 feel the theater mode
\cmo{Participants' gaze patterns also revealed that the participants would more actively look for players when using gaze interactions.}
Moreover, participants suggested that using the gaze interactions was \quot{natural} (e.g., P9, P14) 
and would not add further cognitive cost to the game watching 
since \quot{you can actively control it ... you don't have to [use it]} (P5).
Overall, 
the participants' feedback
provides a strong hint 
that the engagement of watching sports videos can be significantly improved
if video content responds to the audience's gaze.

% since he felt the videos were much more responsive
% The interactions can help 
% With the interactions, participants
% also improve the engagement in watching games

% The embedded visualizations can make the game more engaging
% since they can provide a deeper epistemic pleasures for the casual users.
% The embedded visualizations can improve the engagement since they can \quot{help me understanding and follow the game} (e.g., P1).

%% engagement provide

\subsubsection{Usability -- how easy to use iBall?}
% how easy to use and understand the augmentation
\noindent
All participants confirmed the usability of the embedded visualizations and gaze interactions in iBall (\autoref{fig:rate_vis}c).
They thought both the visualizations and gaze interactions were \quot{easy to understand} and \quot{use}
(e.g., P8, P14 - P6).
We noticed that while some participants thought that one-on-one link was not that useful,
they still agreed that it was easy to understand.
Their ratings demonstrated that our design of \system{} %interactive embedded visualizations % in live basketball videos
is effective: even the games were fast and tense, 
the visualizations and interactions were still easy to understand and use
when watching the game.
% when watching the games.

% \subsection{Feedback, Observations, and Implications}
\subsection{\cmo{Implications for designing gaze-moderated embedded visualizations}}


\paragraph{Attention to Visual Attention in Designing Embedded Visualizations.}
% -- pay attention to visual attention, overwhelming, attentions,
One of our major concern in designing \system{} is 
that the embedded visualizations can overwhelm the users,
given that the basketball games are already overwhelming.
%% overwhelming
However, in our study, 
most of the participants didn't feel the visualizations were overwhelming.
Instead, some participants even could not notice several embedded visualizations (e.g., Offense Ring and Defense Shield).
% Some participants (e.g., P8, P10) even didn't feel 
The participants' feedback actually reveals the Inattentional Blindness~\cite{DBLP:journals/tvcg/HealeyE12} phenomena,
in which viewers can completely fail to perceive visually salient objects or activities.
This finding implies that 
when designing embedded visualizations, % for dynamic scenarios, such as in sports,
\textbf{properly directing the user's attention sometimes can be more effective and important
than reducing the visual complexity
for avoiding overwhelming}.
Additionally,
this finding also implies that 
designer must consider the user's attention in designing embedded visualizations
for effectively conveying information.
For example,
P5 discussed with us that 
we should highlight the Offense Rings, instead of players,
if we want to help the audience efficiently identify which player has the highest EPV.
\cmo{This resonates with the finding that visualizations that link to immediate action were considered most useful for users. For example, one could highlight the Offense Rings when the player is about to shoot.}

\paragraph{The interaction between seeing and hearing.}
% -- commentaries and augmentations
One participant (P4) particularly mentioned that
he paid less attention to the commentaries in \AUG{} mode
but listened to them more carefully in \RAW{} mode,
% the commentaries were more clear to him ,
which implied that the embedded visualizations can ``overlay'' the commentaries.
In fact, 
almost all the participants 
switch their main information source 
from the commentaries to the embedded visualizations
when watching the game in \AUG{} mode.
This observation indicates that
there is an interaction between 
the participants' perception of the embedded visualizations and commentaries.
Such an interaction between human's hearing and vision system has long been identified (e.g., McGurk effect~\cite{}).
Interestingly, in \FULL{} mode,
several participants provided that they would try to search the players mentioned by the commentators by using the gaze interactions.
% All these observations together suggested 
% that 
Thus,
it is crucial to synchronize the commentaries (hearing) and embedded visualizations (vision)
to achieve a consistent and convivial watching experience.
Several participants (e.g., P1, P5, P11) suggested that we can leverage the commentaries to create embedded visualizations.
A recent paper~\cite{chen2022sporthesia} explores the method to directly create embedded visualizations based on commentary text. 

\paragraph{Gaze interactions shift the game from explanatory to exploratory.}
%% gaze interactions open free exploration space, interfering the watching
In \FULL{} mode,
sometimes the participants would continuously follow the players highlighted by their gaze,
thereby missing important passes or shots.
On the other hand, in \AUG{} mode,
participants tended to follow and
focused more on the players highlighted by the system.
Such a difference suggests 
that \AUG{} mode is more explanatory
while adding gaze interactions can shift it towards exploratory.
This is not surprise as the audiences have larger space to actively explore with the gaze interactions.
As such,
when designing gaze interactions for game viewing systems or, broadly speaking, 
any situated visualizations systems that involve visual guidance,
designers must bear the ultimate goal of the systems in mind
and strike a balance between explanatory and exploratory. \cmo{Future work can extend this line to consider human-AI interaction for embedded visualizations.}

\paragraph{Gaze interactions enable learning by watching.}
% -- learn by watching
The gaze interactions can not only improve game watching experience 
but also help audiences progressively learn basketball tactics.
For example, \GFi{} only highlights empty players with green spotlight when the players are near the user's gaze.
With this feature,
P3 could verify if his hypothesis is correct.
When sometimes he thought that 
there should be open players in a corner,
he could move his gaze to the corner
and confirm his guessing if the system \quot{showed green [highlighting]} there.
Besides, P15 also elaborated that \GFo{}
could help him better recognize players
by showing the name of a player to confirm 
that he was looking at the right person.
Such a hypothesis-testing process 
made him feel more confident in analyzing the game 
and interpreting the tactics of the players.
We see this as an interesting opportunity 
to leverage gaze-moderated embedded visualization 
to develop long term impact 
for the users
beyond improving their watching experience within individual games.
% This observation shows that embedded visualizations plus gaze interactions
% can not only improve watching experiences within games 
% but also 
% improve game watching experiences of casual fans in

\paragraph{Suggestions.}
%% Limitations
% -- visual artifacts,  overlaps, 
While the participants generally spoken highly of \system{},
they did complain about a few limitations related to the system implementations.
For example, P8 disliked the visual artifacts introduced by the imperfect segmentation model;
some participants said that \GFo{} could not accurately highlight the target when the players crowded together.
These limitations can be resolved with more advanced models or eye trackers.
Besides,
the participants did suggest several features 
that can significantly improve the user experience of \system{}
when applying it in practice.
% -- further customizability
First, the system should provide more customization 
such as supporting toggling off / on some visualizations,
visualizing other data,
and modifying the parameters of the interactions.
This can be easily implemented 
by allowing the user to configure the system in a \quot{Preference} panel.
% --  adapt to pace, information load
Second, multiple participants pointed out that
the visualizations were 
more readable in slow paced situations 
(e.g., when a player is dribbling outside the three-point line)
and harder to notice when the game is fast paced
(e.g., when a player is cutting in).
Thus, they suggested that the visualizations should also adapt to the pace of the game.
One solution is to use the average moving speed of the players as
an indicator of the pace of the game to adapt the visualizations.
% -- play by play replay
Another point worth to mention is that 
a few participant 
wished the system can generated play-by-play replays with embedded visualizations
to explain the game in details
rather than augmenting the live videos.
We see this requirement as an interesting future research direction.

==> tex/_deprecated/6-user_study_v3.tex <==
\section{User Study}
\label{sec:evaluation}

To assess the usability, usefulness, and engagement 
of using our gaze-moderated embedded visualizations in watching live basketball videos,
we conducted a comparative study between three modes --
watch with raw footage (\RAW{}), 
with solely embedded visualizations (\AUG{}),
and with gaze-moderated embedded visualizations (\FULL{}).

\subsection{Study Settings}

\subsubsection{\textbf{Participants and Apparatus}}
\noindent
We recruited 16 casual fans (F1-F16; M = 10, F = 6; Age: 18 - 35) through university mailing lists and forums 
after screening for their fandom levels and basketball knowledge.
All participants
watched \quot{less than 10 games per year} 
and only \quot{know the basic rules} about basketball.
All participants had not participated in our formative study.
The study was conducted in lab with a 24-inch monitor.
We followed the same ergonomic settings in the formative study 
but changed to use a Tobii eye tracker 5~\cite{}
for more accurate gaze interactions.
The study took about one hour and each participant was compensated with a \$20 gift card.

\subsubsection{\textbf{Design and Procedure}}
\noindent
The study consisted of two tasks, namely,
\textbf{Task1 - \RAW{} vs. \AUG{}}, 
% comparing \RAW{} and \AUG{} mode, 
and \textbf{Task2 - \AUG{} vs. \FULL{}}.
Each task compared two modes.
% comparing \AUG{} and \FULL{} mode.
For each task,
we used a game video from the formative study
and evenly splitted it into two video clips (each lasting around 4.5 minutes)
for each mode.
The videos and the order of modes in each task
were counterbalanced across participants.
Each session included the following phases:

\paragraph{Phase 1. Introduction (10mins).}
The study started with an introduction of the research motivation, 
the purpose of the study, 
and the protocol.
After the participants signed the consent form, 
we conducted a warm-up interview of basketball game-watching experiences.

\paragraph{Phase 2. Comparative Tasks (40mins).}
After the introduction,
we asked participants to finish two comparative tasks (each lasted 20 mins):
In \textbf{Task1 - \RAW{} vs. \AUG{}}, 
the participants watched two video clips in \RAW{} and \AUG{} modes, respectively.
    Before \AUG{} mode, we conducted a training session to
    walk the participant through the four embedded visualizations in a separate video (about 20 seconds).
    We only proceeded to the \AUG{} mode when participants were clear and confident enough to use the embedded visualizations.
In \textbf{Task2 - \AUG{} vs. \FULL{}}, 
the participants watched another two video clips in \AUG{} and \FULL{} mode, respectively. 
Again, a training session was conducted before starting \FULL{} mode to ensure the participant were confident to use the gaze interactions.
Participants were encouraged to think aloud about their game observations when watching the videos.
% After watching each video clip, 
At the end of each video clip,
we performed a post-video interview to
collect the participants' feedback on the mode they had just experienced.
% either the embedded visualizations or the gaze interactions
% based on the specific mode they had just experienced.
At the end of each task, 
participants filled out a post-task questionnaire to rate their experiences.

\paragraph{Phase 3. Post-study Questionnaire (10mins).}
At the end of the session,
we asked participants to complete a post-study questionnaire of 
their subjective ratings on the overall system,
rank the three modes,
and provide feedback on the entire system.

\subsubsection{\textbf{Measures}}
\noindent
Similar to the formative study, 
we recorded the think-aloud for each task.
Besides, 
we collect quantitative measurements of user subjective ratings 
in the post-task 
and post-study questionnaires.
At the end of each task, 
participants were asked to rate the usefulness, engagement, and usability of the features 
they had just experienced,
i.e., the four visualizations (i.e., Player Highlight, \OffR{}, \DefS{}, and \OOOL{}) in \textbf{Task1}
and the two gaze interactions (i.e., \GFo{} and \GFi{}) in \textbf{Task2},
on a 7-point Likert scale.
In the post-study questionnaires,
we asked participants to rated the overall system on five questions regarding system usefulness and engagement~\cite{} 
and ranked the three modes. 
% We also collected and analyzed qualitative feedback from the participants in post-task and post-study interviews.

\subsection{Study Results}
We first report 
% the participants' 
the ratings of the overall system 
and the rankings of the three modes,
and then discuss the feedback on the usefulness, engagement, and usability of
individual visualizations and interactions.

\subsubsection{\textbf{The overall user experience of \system{} was predominantly positive, with \FULL{} being most preferred}}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_61_overall.pdf}
    \caption{Left: Ratings on the overall system. Right: Rankings of different conditions, 
        i.e., \RAW{} -- watch with raw footage,
        \AUG{} -- watch with embedded visualizations solely,
        \FULL{} -- watch with gaze interaction and embedded visualizations.
        }
    \label{fig:overall}
\end{figure}

\noindent
% The participants overarchingly spoke highly of \system{}.
As shown in \autoref{fig:overall} left, 
the majority rated \system{} as \quot{helpful} and \quot{fun}, 
felt \quot{in control} and \quot{encouraged} when using the system,
and were \quot{likely to use} the system for watching basketball games.
Figure~\ref{fig:overall} right presents the rankings of the three modes,
showing that 
\FULL{} was the most preferred mode by 12 participants, 
followed by \AUG{} by 4 and \RAW{} by none. 
% The rankings revealed that the gaze-moderated embedded visualizations designed by us were preferred by most of the participants.
%% P11, don't like the bluring of the audiences
%% P7 don't like the blurring due to the visual artifacts
%% p8 don't like the blurring of audience seems abnormal, and don't feel overwhelming.
Among four participants who didn't rank \FULL{} as the best,
% While there is 
% one participant simple preferred \AUG{} over \FULL{} for no reason;
they were mainly concerned about  
the blurring effect of the audience in the \GFi{}, 
stating that 
% They disliked the visual artifacts introduced by the blurring effect %of the audiences
a game video without audiences seemed abnormal.
However, all of them agreed that the filtering of open players (highlighted in green) was useful.
Such customization
can be easily achieved 
by providing a \quot{Preferences} panel to enable users to configure their preferred settings.
In summary,
while \GFi{} can be improved by providing more customization,
participants provided very positive feedback on \system{},
demonstrating that the system
can effectively improve the experience of casual fans in watching live basketball videos.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_62_vis+gaze.pdf}
    \caption{Ratings on the embedded visualizations and gaze interactions.}
    \label{fig:rate_vis}
\end{figure}


% \subsubsection{\textbf{Simple visualizations that link to immediate game actions and react to user's gaze were favored by participants}}
% \noindent
% Taken together, 
% each embedded visualization supports different game insights for audience, similar to the findings of~\cite{lin2022the}. 
% What's more interesting is that casual fans in our study preferred visualizations that can be easily noticed (e.g., Player Highlight or player name with \GFo{}) 
% and link to immediate action, 
% such as indicating shooting action with \OffR{} or \DefS{}.

\subsubsection{\textbf{Embedded visualizations are useful if they are attrative and informative}}
\noindent
Participants rated positively on the usefulness of each visualization (\autoref{fig:rate_vis}a).
Among the four embedded visualizations,
Player Highlight was considered to be the most useful
in \quot{predicting the ball receiver} at the next pass,
\quot{highlighting the open players},
and thus \quot{making the game much clearer}, 
as mentioned by the participants.

Participants also rated \OffR{} and \DefS{} as useful to understand players' in-game decisions.
For example, F8 thought that \OffR{}
can \quot{help me expect when he's gonna shoot. Otherwise, it's just like this person can shoot anytime.};
F3 commented that \DefS{} clearly showed \quot{who's able to defend} 
and explained why \quot{James can easily score on Iguodala}.
However, 
some participants found them less useful 
since the visualizations were placed on the ground,
different from the ball at hand-height,
and thus often hard to notice in a tense game.
Nevertheless, most of the participants agreed that 
\quot{it was nice to have} \OffR{} and \DefS{} in the system.

\OOOL{} was controversial in terms of usefulness. 
Some participants 
considered it helpful \quot{to follow the game and to see who was involved [in defending]} (F6)
while others felt it suffers from the same limitations 
as \OffR{} and \DefS{} (i.e., cannot be noticed)
with less useful information 
that was already \quot{clear from the video} (F1).
P13 also suggested that we could show the one-on-one relationships for more players 
other than just for the player with the ball.

\subsubsection{\textbf{Gaze interactions are useful 
as they satisfy audiences' own information and cognitive needs
}}
\noindent
Both \GFo{} and \GFi{}
received very positive ratings regarding usefulness (\autoref{fig:rate_vis}a).
% With gaze interactions, participants naturally adjusted the embedded visualizations
% to satisfy their own information needs and cognitive bandwidth.
Participants particularly enjoyed using \GFo{}
as it could help them \quot{know the name of the player [who I am looking at]} (e.g., F1 - F16).
This simple yet effective information can significantly help casual fans to \quot{follow the game and understand who is who} (F16).
\GFi{} also 
improved the game understanding of participants
as it could \quot{make the scene tidier} (F22)
and \quot{focus the information on what I'm looking [at]} (F4).

\subsubsection{\textbf{Embedded visualizations are engaging since they provide a deeper epistemic pleasure}}
\noindent
The participants felt that 
the embedded visualizations are engaging (\autoref{fig:rate_vis}b)
since they can help them \quot{understand and follow the game}.
This is also reflected 
in the positive relationship between the usefulness and engagement of the embedded visualizations -- 
the more useful, the more engaging.
For example,
F1, a novice in watching NBA games, 
commented that \quot{it is nice to know who the star players are because otherwise, they all look like regular players to me.}
F5 remarked that he \quot{always tried to predict the receiver of a pass but always failed}.
With the visualizations, he felt much more confident in predicting the receiver and 
felt quite a sense of accomplishment whenever he was correct.

\subsubsection{\textbf{Gaze interactions are engaging since they promote proactive game viewing experiences}}
\noindent
Gaze interactions are also engaging (\autoref{fig:rate_vis}b)
since they make the passive watching experience
interactive and proactive.
As F2 explained, when the video scene responded to her gaze, 
she felt that she was \quot{also a part of the game.}
F4 particularly enjoyed using the gaze interactions 
which made the videos much more \quot{responsive}
and made him \quot{almost feel like I'm there}.
% P9 feel the theater mode
% \cmo{Participants' gaze patterns also revealed that the participants would more actively look for players when using gaze interactions.}
Moreover, participants suggested that using the gaze interactions was \quot{natural} (e.g., F9, F14) 
and would not add further cognitive cost to the game watching 
since \quot{you can actively control it ... you don't have to [use it]} (F5).
Overall, 
the participants' feedback
provides a strong hint 
that the engagement of watching sports videos can be significantly improved
if video content responds to the audience's gaze.

\subsubsection{\textbf{The gaze-moderated embedded visualizations are easy to understand and use}}
\noindent
All participants confirmed the usability of the embedded visualizations and gaze interactions in \system{} (\autoref{fig:rate_vis}c).
They thought both the visualizations and gaze interactions were \quot{easy to understand} and \quot{use}
(e.g., F8, F14 - F16).
We noticed that while some participants thought that \OOOL{} was not that useful,
they still agreed that it was easy to understand.
Their ratings demonstrated that our design of \system{} 
is effective: even the games were fast and tense, 
the visualizations and interactions were still easy to understand and use
while watching the game.

\subsection{Implications for Designing Gaze-moderated Embedded Visualizations}
We now discuss the design implications we learned from the feedback and observations in the user study.

\subsubsection{\textbf{Attention to Visual Attention}}
% -- pay attention to visual attention, overwhelming, attentions,
\noindent
While we were concerned that embedded visualizations would impose additional cognitive load on watching an already fast-paced basketball game, 
most participants in our study did not find the visualizations overwhelming.
Instead, some participants even could not 
notice several embedded visualizations (e.g., \OffR{} and \DefS{}).
The participants' feedback actually reveals the Inattentional Blindness~\cite{DBLP:journals/tvcg/HealeyE12} phenomena,
in which viewers can completely fail to perceive visually salient objects or activities.
This finding implies that 
when designing embedded visualizations, % for dynamic scenarios, such as in sports,
\textbf{properly directing the user's attention sometimes can be more effective and important
than reducing the visual complexity
for avoiding overwhelming}.
Additionally,
this finding also implies that 
designer must consider users' attention in designing embedded visualizations
for effectively conveying information.
For example,
F5 discussed with us that 
we should highlight the \OffR{}, instead of players,
if we want to help the audiences efficiently identify which player has the highest EPV.
Besides, one could also highlight visualizations that link to immediate actions
to increase the information salience, 
e.g., highlight the \OffR{} when the player is about to shoot.

% -- commentaries and augmentations
\subsubsection{\textbf{The Interaction Between Seeing and Hearing}}
\noindent
F4 particularly mentioned that
he paid less attention to the commentaries in \AUG{} mode
but listened to them more carefully in \RAW{} mode,
which implied that the embedded visualizations can ``overlay'' the commentaries.
In fact, 
almost all the participants 
switch their main information source 
from the commentaries to the embedded visualizations
when watching the game in \AUG{} or \FULL{} mode.
This observation indicates that
there is an interaction between 
the participants' perception of the embedded visualizations and commentaries.
Such an interaction between human's hearing and vision system has long been identified (e.g., McGurk effect~\cite{}).
Interestingly, in \FULL{} mode,
several participants provided that they would try to search the players mentioned by the commentators by using the gaze interactions.
Thus,
it is crucial to synchronize the commentaries (hearing) 
and embedded visualizations (vision)
to achieve a consistent and convivial watching experience.
Several participants suggested that we can leverage the commentaries to create embedded visualizations.
A recent paper~\cite{chen2022sporthesia} explores this direction for racket-based sports.


%% gaze interactions open free exploration space, interfering the watching
\subsubsection{\textbf{Gaze Interactions Shift the Game from Explanatory to Exploratory}}
\noindent
In \FULL{} mode,
sometimes the participants would continuously follow the players highlighted by their gaze,
thereby missing important passes or shots.
On the other hand, in \AUG{} mode,
participants tended to follow and
focused more on the players highlighted by the system.
Such a difference suggests 
that \AUG{} mode is more explanatory
while adding gaze interactions can shift it towards exploratory.
This is not surprise as the audiences have larger space to actively explore with the gaze interactions.
As such,
when designing gaze interactions for game viewing systems or, broadly speaking, 
any situated visualizations systems that involve visual guidance,
designers must bear the ultimate goal of the systems in mind
and strike a balance between explanatory and exploratory.
Future work can extend this line to consider human-AI interaction for embedded visualizations.

% -- learn by watching
\subsubsection{\textbf{Gaze Interactions Enable Learning by Watching}}

\noindent
The gaze interactions can not only improve game watching experience 
but also help audiences progressively learn basketball tactics.
For example, 
\GFi{} only highlights empty players with green spotlight when the players are near the user's gaze.
With this feature,
F3 could verify if his hypothesis is correct.
When sometimes he thought that 
there should be open players in a corner,
he could move his gaze to the corner
and confirm his guessing if the system \quot{showed green [highlighting]} there.
Besides, F15 also elaborated that \GFo{}
helped him better recognize players
by showing the name of a player to confirm 
that he was looking at the right person.
Such a hypothesis-testing process 
made the participants feel more confident in 
interpreting the game.
We see this as an interesting opportunity 
to leverage gaze-moderated embedded visualization 
to develop long term impact 
for the users
beyond improving their watching experience within individual games.

\subsubsection{\textbf{Suggestions}}
\noindent
%% Limitations
% -- visual artifacts,  overlaps, 
While the participants generally spoken highly of \system{},
they did complain about a few limitations related to the system implementations.
For example, F8 disliked the visual artifacts introduced by the imperfect segmentation model;
some participants said that \GFo{} could not accurately highlight the target when the players crowded together.
These limitations can be resolved with more advanced models or eye trackers.
Besides,
the participants did suggest several features 
that can improve the user experience of \system{}.
% when applying it in practice.
% -- further customizability
First, the system should provide more customization 
such as supporting toggling off / on some visualizations,
visualizing other data,
and modifying the parameters of the interactions.
This can be easily implemented 
by allowing the user to configure the system in a \quot{Preference} panel.
% --  adapt to pace, information load
Second, multiple participants pointed out that
the visualizations were 
more readable in slow paced situations 
(e.g., when a player is dribbling outside the three-point line)
and harder to notice when the game is fast paced
(e.g., when a player is cutting in).
Thus, they suggested that the visualizations should also adapt to the pace of the game.
One solution is to use the average moving speed of the players as
an indicator of the pace of the game to adapt the visualizations.
% -- play by play replay
Another point worth to mention is that 
a few participant 
wished the system can generated play-by-play replays with embedded visualizations
to explain the game in details
rather than augmenting the live videos.
We see this requirement as an interesting future research direction.

==> tex/_deprecated/6-user_study_v4.tex <==
\section{User Study}
\label{sec:evaluation}

To assess the usefulness, usability, and engagement 
of using our gaze-moderated embedded visualizations in watching basketball videos,
we conducted a comparative study between three modes --
watch with raw footage (\RAW{}), 
with solely embedded visualizations (\AUG{}),
and with gaze-moderated embedded visualizations (\FULL{}).

\subsection{Study Setup}

\subsubsection{\textbf{Participants and Apparatus}}
\noindent
We recruited 16 casual fans (F1-F16; M = 10, F = 6; Age: 18 - 35) through university mailing lists and forums 
after screening for their fandom levels and basketball knowledge.
All participants
watched \quot{less than 10 games per year} 
and only \quot{know the basic rules} of basketball.
All participants had not participated in our formative study.
The study was conducted in the lab with a 24-inch monitor.
We followed the same ergonomic settings in the formative study 
but changed to use a Tobii eye tracker 5~\cite{tobii}
for more accurate gaze interactions.
The study took about one hour and each participant was compensated with a \$20 gift card.

\subsubsection{\textbf{Design and Procedure}}
\noindent
The study consisted of two tasks, namely,
\textbf{Task1 - \RAW{} vs. \AUG{}}, 
% comparing \RAW{} and \AUG{} mode, 
and \textbf{Task2 - \AUG{} vs. \FULL{}}.
Each task compared two modes.
% comparing \AUG{} and \FULL{} mode.
For each task,
we used a game video from the formative study
and evenly split it into two video clips (each lasting around 4.5 minutes)
for each mode.
The videos and the order of modes in each task
were counterbalanced across participants.
Each session included the following phases:

\paragraph{Phase 1. Introduction (10mins).}
The study started with an introduction of the research motivation, 
the purpose of the study, 
and the protocol.
After the participant signed a consent form, 
we conducted a warm-up interview about basketball game-watching experiences.

\paragraph{Phase 2. Comparative Tasks (40mins).}
% After the introduction,
We asked participants to finish two comparative tasks (each lasted 20 mins):
In \textbf{Task1 - \RAW{} vs. \AUG{}}, 
the participants watched two video clips in \RAW{} and \AUG{} modes, respectively.
    Before \AUG{} mode, we conducted a training session to
    walk the participant through the four embedded visualizations in a separate video (about 20 seconds).
    We only proceeded to the task when participants were clear and confident enough to use the embedded visualizations.
In \textbf{Task2 - \AUG{} vs. \FULL{}}, 
the participants watched another two video clips in \AUG{} and \FULL{} mode, respectively. 
Again, a training session was conducted before starting \FULL{} mode to ensure the participant were confident to use the gaze interactions.
Participants were encouraged to think aloud about their game observations when watching the videos.
% After watching each video clip, 
At the end of each video clip,
we performed a post-video interview to
collect the participants' feedback on the mode they had just experienced.
% either the embedded visualizations or the gaze interactions
% based on the specific mode they had just experienced.
At the end of each task, 
participants filled out a post-task questionnaire to rate their experiences.

\paragraph{Phase 3. Post-study Questionnaire (10mins).}
At the end of the session,
we asked participants to complete a post-study questionnaire of 
their subjective ratings on the overall system,
rank the three modes,
and provide feedback on the entire system.

\subsubsection{\textbf{Measures}}
\noindent
% Similar to the formative study, 
% we recorded the think-aloud for each task.
% Besides, 
We collect quantitative measurements of user subjective ratings 
in the post-task 
and post-study questionnaires.
At the end of each task, 
participants were asked to rate the usefulness, engagement, and usability of the features 
they had just experienced,
including the four visualizations (i.e., Player Highlight, \OffR{}, \DefS{}, and \OOOL{}) in \textbf{Task1}
and the two gaze interactions (i.e., \GFo{} and \GFi{}) in \textbf{Task2},
on a 7-point Likert scale.
In the post-study questionnaires,
we asked participants to rate the overall system on five questions about system usefulness and engagement~\cite{obrienDevelopmentEvaluationSurvey2010} 
and ranked the three modes. 
% We also collected and analyzed qualitative feedback from the participants in post-task and post-study interviews.

\subsection{Study Results}
We first report 
% the participants' 
the ratings of the overall system 
and the rankings of the three modes,
and then discuss the feedback on the usefulness, engagement, and usability of
individual visualizations and interactions.

\subsubsection{\textbf{The overall user experience of \system{} was predominantly positive, with \FULL{} being most preferred}}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/fig_61_overall.pdf}
    \caption{Left: Ratings on the overall system. Right: Rankings of different modes, 
        i.e., \RAW{} -- watch with raw footage,
        \AUG{} -- watch with embedded visualizations solely,
        \FULL{} -- watch with gaze interaction and embedded visualizations.
        }
    \label{fig:overall}
\end{figure}

\noindent
% The participants overarchingly spoke highly of \system{}.
As shown in \autoref{fig:overall} left, 
the majority rated \system{} as \quot{helpful} and \quot{fun}, 
felt \quot{in control} and \quot{encouraged} when using the system,
and were \quot{likely to use} the system for watching basketball games.
Figure~\ref{fig:overall} right presents the rankings of the three modes,
showing that 
\FULL{} was the most preferred mode by 12 participants, 
followed by \AUG{} by 4 and \RAW{} by none. 
Among four participants who didn't rank \FULL{} as the best,
they were mainly concerned about  
the blurring effect of the audience in \GFi{}, 
stating that 
a game video without audiences seemed abnormal.
However, all of them agreed that the filtering of open players (highlighted in green) was useful.
Such customization
can be easily achieved 
by providing a \quot{Preferences} panel to enable users to configure their preferred settings.
% In summary,
% while \GFi{} can be improved by providing more customization,
% participants provided very positive feedback on \system{},
% demonstrating that the system
% can effectively improve the experience of casual fans in watching live basketball videos.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/fig_62_vis+gaze.pdf}
    \caption{Ratings on the usefulness, engagement, and usability of the embedded visualizations and gaze interactions in \system{}.}
    \label{fig:rate_vis}
\end{figure}

\subsubsection{\textbf{Embedded visualizations are more useful if they are more attractive and informative}}
\noindent
Participants rated positively on the usefulness of each visualization (\autoref{fig:rate_vis}a).
Among the four embedded visualizations,
Player Highlight was considered to be the most useful
in \quot{predicting the ball receiver} at the next pass,
\quot{highlighting the open players},
and thus \quot{making the game much clearer}, 
as mentioned by the participants.

Participants also rated \OffR{} and \DefS{} as useful to understand players' in-game decisions.
For example, F8 thought that \OffR{}
could \quot{help me expect when he's gonna shoot. Otherwise, it's just like this person can shoot anytime.};
F3 commented that \DefS{} clearly showed \quot{who's able to defend} 
and explained why \quot{James can easily score on Iguodala}.
However, 
some participants found them less useful 
since the visualizations were placed on the ground,
different from the ball at hand-height,
and thus often hard to notice in a tense game.
Nevertheless, most of the participants agreed that 
\quot{it was nice to have} \OffR{} and \DefS{} in the system.

\OOOL{} was controversial in terms of usefulness. 
Some participants 
considered it helpful \quot{to follow the game and to see who was involved [in defending]} (F6)
while others felt it suffers from the same limitations 
as \OffR{} and \DefS{} (i.e., cannot be noticed)
with less useful information 
that was already \quot{clear from the video.} (F1)
F13 suggested that we could show the one-on-one relationships for more players 
other than just for the player with the ball.

\subsubsection{\textbf{Gaze interactions are useful 
as they satisfy audiences' own information and cognitive needs
}}
\noindent
Both \GFo{} and \GFi{}
received very positive ratings regarding usefulness (\autoref{fig:rate_vis}a).
% With gaze interactions, participants naturally adjusted the embedded visualizations
% to satisfy their own information needs and cognitive bandwidth.
Participants particularly enjoyed using \GFo{}
as it could help them \quot{know the name of the player [who I am looking at]} (F1 - F16).
This simple yet effective information can significantly help casual fans to \quot{follow the game and understand who is who.} (F16)
\GFi{} also 
improved the game understanding of participants
as it could \quot{make the scene tidier} (F22)
and \quot{focus the information on what I'm looking [at].} (F4)

\subsubsection{\textbf{Embedded visualizations are engaging since they provide a deeper epistemic pleasure}}
\noindent
The participants felt that 
the embedded visualizations were engaging (\autoref{fig:rate_vis}b)
since they could help them \quot{understand and follow the game}.
This is also reflected 
in the positive relationship between the usefulness and engagement of the embedded visualizations -- 
the more useful, the more engaging.
For example,
F1 %, a novice in watching NBA games, 
commented that \quot{it is nice to know who the star players are because otherwise, they all look like regular players to me.}
F5 remarked that he \quot{always tried to predict the receiver of a pass but always failed.}
With the visualizations, he felt much more confident in predicting the receiver and 
felt quite a sense of accomplishment whenever he was correct.

\subsubsection{\textbf{Gaze interactions are engaging since they promote proactive game viewing experiences}}
\noindent
Gaze interactions are also engaging (\autoref{fig:rate_vis}b)
since they make the passive watching experience
interactive and proactive.
As F2 explained, when the video scene responded to her gaze, 
she felt that she was \quot{also a part of the game.}
F4 particularly enjoyed using the gaze interactions, 
which made the videos much more \quot{responsive}
and made him \quot{almost feel like I'm there.}
Moreover, participants suggested that using the gaze interactions was \quot{natural} %(e.g., F9, F14) 
and would not add further cognitive cost to the game watching 
since \quot{you can actively control it ... you don't have to [use it]} (F5).
Overall, 
the participants' feedback
provides a strong hint 
that the engagement of watching sports videos can be significantly improved
if video content responds to the audience's gaze.

\subsubsection{\textbf{The gaze-moderated embedded visualizations are easy to understand and use}}
\noindent
All participants confirmed the usability of the embedded visualizations and gaze interactions in \system{} (\autoref{fig:rate_vis}c).
They thought both the visualizations and gaze interactions were \quot{easy to understand} and \quot{use}.
We noticed that while some participants thought that \OOOL{} was not that useful,
they still agreed that it was easy to understand.
Their ratings demonstrated that our design of \system{} 
is effective: even the games were fast and tense, 
the visualizations and interactions were still easy to understand and use
while watching the game.

\subsection{Implications for Designing Gaze-moderated Embedded Visualizations}
We now discuss the design implications we learned from the feedback and observations in the user study.

\subsubsection{\textbf{Visual Attention Matters When Designing Embedded Visualizations}}
% -- pay attention to visual attention, overwhelming, attentions,
\noindent
While we were concerned that embedded visualizations would impose additional cognitive load on watching an already fast-paced basketball game, 
most participants in our study did not find the visualizations overwhelming.
Instead, some participants even could not 
notice several embedded visualizations (e.g., \OffR{} and \DefS{}).
The participants' feedback actually reveals the Inattentional Blindness~\cite{DBLP:journals/tvcg/HealeyE12} phenomenon,
in which viewers can completely fail to perceive visually salient objects or activities.
This finding implies that 
when designing embedded visualizations, % for dynamic scenarios, such as in sports,
\textbf{properly directing the user's attention can sometimes be more effective and important
than reducing the visual complexity
for avoiding overwhelming}.
Additionally,
this finding also implies that when designing embedded visualizations,
designers must \textbf{consider users' attention for effectively conveying information}.
For instance,
F5 discussed with us that 
we should highlight the \OffR{}, instead of players,
if we want to help audiences efficiently identify the player with the highest EPV.
Besides, one can also highlight visualizations that link to immediate actions
to increase the information salience, 
e.g., highlight the \OffR{} when the player is about to shoot.

% -- commentaries and augmentations
\subsubsection{\textbf{Synchronization of Seeing and Hearing Matters When Designing Embedded Visualizations}}
\noindent
F4 particularly mentioned that
he paid less attention to the commentaries in \AUG{} mode
but listened to them more carefully in \RAW{} mode,
which implied that the embedded visualizations could ``overlay'' the commentaries.
In fact, 
almost all the participants 
switched their main information source 
from the commentaries to the embedded visualizations
when watching the game in \AUG{} or \FULL{} mode.
This observation indicates that
there is an interaction between 
the participants' perception of the embedded visualizations and commentaries.
Such an interaction between human's hearing and vision system has long been identified (e.g., McGurk effect~\cite{tiippana2014mcgurk}).
Interestingly, in \FULL{} mode,
several participants provided that they would try to search the players mentioned by the commentators by using the gaze interactions.
Thus,
it is crucial to \textbf{synchronize the commentaries (hearing) 
and embedded visualizations (vision)
to achieve a consistent and convivial watching experience}.
Several participants suggested that we can leverage the commentaries to create embedded visualizations.
A recent paper~\cite{chen2022sporthesia} explores this direction for racket-based sports.

%% gaze interactions open free exploration space, interfering the watching
\subsubsection{\textbf{Gaze Interactions Shift the Game from Explanatory to Exploratory}}
\noindent
In \FULL{} mode,
the participants spent more time using their gaze to highlight players,
% to highlight players by using their gaze,
% attempted to 
% continuously follow the players highlighted by their gaze,
% thereby missing important passes or shots.
while in \AUG{} mode,
participants tended to follow and focus more on the players highlighted by the system.
Such a difference suggests 
that \AUG{} mode is more explanatory
while adding gaze interactions can shift it towards exploratory.
This is unsurprised as the audiences have a larger space to actively explore with the gaze interactions.
As such,
when designing gaze interactions for game viewing systems or, broadly speaking, 
any situated visualizations systems that involve visual guidance,
designers must \textbf{bear the ultimate goal of the systems in mind
and strike a balance between explanatory and exploratory}.
% Future work can extend this line to consider human-AI interactions for embedded visualizations.

% -- learn by watching
\subsubsection{\textbf{Gaze Interactions Enable Active Learning in Game Watching}}
\noindent
The gaze interactions can 
% not only improve game watching experience but 
also help audiences progressively learn basketball knowledge.
For example, 
\GFi{} only highlights \cmo{open} players with green spotlights when the players are near the user's gaze.
With this feature,
F3 could verify if his hypothesis is correct.
When sometimes he thought that 
there should be open players in a corner,
he could move his gaze to the corner
and confirm his guess if the system \quot{showed green [highlighting]} there.
Besides, F15 also elaborated that \GFo{}
helped him better recognize players
by showing the name of a player to confirm 
that he was looking at the right person.
Such a hypothesis-testing process 
made the participants feel more confident in 
interpreting the game. 
We see this as an interesting opportunity 
to \textbf{leverage gaze-moderated embedded visualization 
to develop long-term impact 
for the users}
beyond improving their watching experience within individual games.

\subsubsection{\textbf{Suggestions}}
\noindent
%% Limitations
% -- visual artifacts,  overlaps, 
While the participants generally spoke highly of \system{},
they did complain about a few limitations related to the system implementations.
For example, F8 disliked the visual artifacts introduced by the imperfect segmentation model;
some participants said that \GFo{} could not accurately highlight the target when the players crowded together.
These limitations can be resolved with more advanced models or eye trackers.
Besides,
the participants suggested several features 
% that can improve the user experience of 
for \system{}.
% when applying it in practice.
% -- further customizability
First, 
the system should provide more customization via a \quot{Preference} panel,
such as supporting toggling off / on some visualizations,
visualizing other data,
and modifying the parameters of the interactions.
% This can be easily implemented 
% by allowing the user to configure the system in a \quot{Preference} panel.
% --  adapt to pace, information load
Second, 
multiple participants suggested that 
the visualizations should also adapt to the pace of the game,
e.g., showing more details in slow-paced and less in fast-paced situations.
% pointed out that
% the visualizations were 
% more readable in slow paced situations 
% (e.g., when a player is dribbling outside the three-point line)
% and harder to notice when the game is fast paced
% (e.g., when a player is cutting in).
% Thus, they suggested that 
One solution is to use the average moving speed of the players as
an indicator of the pace of the game to adapt the visualizations.
% -- play by play replay
Another point worth mentioning is that 
a few participants wished the system could generate play-by-play replays with embedded visualizations
to explain the game in detail.
% rather than augmenting the live videos.
We see this requirement as an interesting future research direction.

==> tex/_deprecated/7-discussion_v1.tex <==
\section{Discussions}

\para{Reproducible Environments For Embedded Visualizations Research.}
% - reproductive research
Compared to traditional web-based visualizations,
embedded or situated visualizations are particularly challenging to research
since the physical context where the embedded visualizations are registered in
is inherently difficult to reproduce, distribute, and benchmark.
It can be more difficult, or even impossible, to reproduce
the physical context if it is dynamic (e.g., sports scenarios).
This perhaps is the major reason why most existing research~\cite{lin2022the, yao2022visualization}
opts for using reproducible simulated environments (e.g., virtual reality) 
for exploring embedded visualizations.
In this work, 
we use videos 
% as reproducible simulated environments
to explore 
the design of interactive embedded visualizations 
% to provide information 
in dynamic, complex scenarios.
To boost the research in embedded visualizations,
we will open source~\footnote{\url{https://anonymous-github-repo.io}} our video-based environments (i.e., code and data)
for others to reproduce our system and develop their owns.

\para{Gaze Interactions for Interactive Embedded Visualizations.}
In recent years, 
eye-trackers are becoming increasingly affordable, 
opening a wide range of opportunities for interactive visualizations.
Compared to other input modalities 
such as keyboard and mouse, touch, and voice,
gaze input can realize fast, intuitive, and implicit interactions.
% In fact, more and more video games~\cite{}, 
% especially first-person shooting or driving games,
% integrate gaze interactions to provide better user experiences.
In fact,
gaze interactions are widely supported in head-mounted displays~\cite{} 
for augmented or virtual reality (AR/VR),
which are the major scenarios to employ embedded visualizations.
Our research shows that even only using simple gaze data (i.e., the 2D position of gaze point on the screen)
can significantly increase the usefulness and engagement of embedded visualizations.
Yet, 
gaze interactions have their own limitations,
such as cannot be used in multi-viewers scenarios (e.g., TV in living room).
Besides,
we still haven't explored 
leveraging advanced gaze events (e.g., fixation, saccade)
or combining gaze with other input modalities,
which we consider as promising future directions.

\para{Towards Augmenting Real-world Environments Beyond Videos.}
While watching sports games on TV and livestreams is accessible for most audiences,
many sports fans prefer watching the games in-person.
With the development of sensing techniques and Augmented Reality (AR) devices 
such as head-mounted displays,
it is gradually possible to augment 
real-world environments with digital information.
Our research provides a step-stone towards augmenting in-person game watching experiences:
the CV pipeline can be a technical base for processing live video streams from AR devices;
the gaze-moderated embedded visualizations design can also be generalized to real-world environments. 
Nonetheless, 
there are still numerous open questions that must be tackled to adapt our system to AR environments,
including the limited field of view, 
the effect of stereoscopy vision and depth perception,
and the ability to freely change viewing perspective.
We hope that the lessons learned from the present research can 
inspire and provide a firm foundation for future research in augmenting in-person game watching scenarios, 
ultimately generalizing embedded visualizations to general real-world environments.

\para{Study Limitations.}
Our study results, including the ratings and gaze distributions, 
only evaluate the system qualitative rather than quantitative,
due to the lack of quantitative metrics and benchmark tasks.
While theoretically our CV pipeline can process the video in real-time,
our current system uses it to preprocess the videos in advanced.
Besides, our system assumes a two seconds buffer time in the videos to obtain the ball receiver.
Finally, the designs of the embedded visualizations and gaze interactions in \system{}
are derived based on the 16 participants in our formative study.
Further explorations are thus suggested for different scenarios and user groups.


==> tex/_deprecated/8-discussion_v2.tex <==
\section{Discussions}

\paragraph{\textbf{Reproducible Environments For Embedded Visualizations Research.}}
% - reproductive research
Compared to traditional web-based visualizations,
embedded or situated visualizations are particularly challenging to research
since the physical context where the embedded visualizations are registered in
is inherently difficult to reproduce, distribute, and benchmark.
It can be more difficult, or even impossible, to reproduce
the physical context if it is dynamic (e.g., sports scenarios).
This perhaps is the major reason why most existing research~\cite{lin2022the, yao2022visualization}
opts for using reproducible simulated environments (e.g., virtual reality) 
for exploring embedded visualizations.
In this work, 
we use videos 
% as reproducible simulated environments
to explore 
the design of interactive embedded visualizations 
% to provide information 
in dynamic, complex scenarios.
To boost the research in embedded visualizations,
we will open source~\footnote{\url{https://anonymous-before-published.github.io}} our video-based environments (i.e., code and data)
for others to reproduce our system and develop their own.

\paragraph{\textbf{Gaze Interactions for Embedded Visualizations.}}
In recent years, 
eye-trackers are becoming increasingly affordable.
% opening a wide range of opportunities for interactive visualizations.
Compared to other input modalities 
such as keyboard, mouse, and voice,
gaze input can realize fast, intuitive, and implicit interactions.
In fact,
gaze interactions are widely supported in head-mounted displays~\cite{vive2}
for augmented or virtual reality (AR/VR),
which are the major scenarios to employ embedded visualizations.
Our research shows that even only using simple gaze data (i.e., the 2D position of the gaze point on the screen)
can significantly increase the usefulness and engagement of embedded visualizations.
Yet, 
gaze interactions have their own limitations,
such as \cmo{that they} cannot be used in multi-viewers scenarios (e.g., TV in living rooms).
Besides,
we still haven't explored 
leveraging advanced gaze events (e.g., fixation, saccade)
or combining gaze with other input modalities,
which we consider as promising future directions.

%% the technical challenges to apply to real livestreams
\paragraph{\textbf{Towards Actual Augmented Live Game Viewing.}}
\cmo{move to sec4?}
In \autoref{sec:cv_limitation}, 
we discuss the technical challenges and potential solutions to apply our system in reality.
% While our research provides a step-stone towards augmenting actual livestreams,
% there are still
% several technical challenges 
% that must be tackled to realize our system in reality,
% such as achieving
% real-time processing, 
% higher recognition accuracy, 
% and efficient access to tracking and historical data.
% These technical challenges overall can be addressed by more computational resources
% such as powerful machines,
% lightweight models, 
% and better engineering implementations.
On the other hand,
real-world applications also provide opportunities for improving the system,
including 
videos with a higher resolution and framerate,
parameters of the camera, 
and steering from human experts.
Thus, 
we believe our system can be adopted and extended 
to actual live games by the broadcasters,
or by researchers once the extra resources and information are available.

\paragraph{\textbf{Augmenting Real-world Games Beyond Videos.}}
% While watching sports games on TV and livestreams is accessible for most audiences,
% many sports fans prefer watching the games in-person.
With the development of sensing techniques and AR devices 
such as head-mounted displays,
it gradually becomes possible to augment 
real-world games with digital information.
While our research provides a step-stone towards augmenting real-world environments,
% Our gaze-moderated embedded visualizations design
% can be generalized to real-world environments,
several issues must be taken into account when adopting it to AR,
including the limited field of view, 
the effect of stereoscopy vision and depth perception,
and the ability to freely change viewing perspective.
We hope that the lessons learned from the present research can 
inspire and provide a firm foundation for future research in augmenting in-person game watching scenarios, 
ultimately generalizing embedded visualizations to general real-world environments.

\paragraph{\textbf{Study Limitations.}}
Our study results, including the ratings and gaze distributions, 
only evaluate the system qualitative rather than quantitative,
due to the lack of quantitative metrics and benchmark tasks.
% While theoretically our CV pipeline can process the video in real-time,
% our current system uses it to preprocess the videos in advanced.
% Besides, our system assumes a five seconds buffer time in the videos to obtain the ball receiver.
The designs of the embedded visualizations and gaze interactions in \system{}
are derived based on the 16 participants in our formative study.
Further explorations are thus suggested for different scenarios and user groups.

